A Multifidelity Sim-to-Real Pipeline for Verifiable and Compositional Reinforcement Learning

We propose and demonstrate a compositional framework for training and verifying reinforcement learning (RL) systems within a multifidelity sim-to-real pipeline, in order to deploy reliable and adaptable RL policies on physical hardware. By decomposing complex robotic tasks into component subtasks and defining mathematical interfaces between them, the framework allows for the independent training and testing of the corresponding subtask policies, while simultaneously providing guarantees on the overall behavior that results from their composition. By verifying the performance of these subtask policies using a multifidelity simulation pipeline, the framework not only allows for efficient RL training, but also for a refinement of the subtasks and their interfaces in response to challenges arising from discrepancies between simulation and reality. In an experimental case study we apply the framework to train and deploy a compositional RL system that successfully pilots a Warthog unmanned ground robot.

==> figures/abstract/simple_hlm2.tex <==
\begin{tikzpicture}[
    labelText/.style={font=\scriptsize, inner xsep=0.0cm, inner ysep=0.0cm},
    eqText/.style={font=\scriptsize, inner xsep=0.0cm, inner ysep=0.0cm},
    % branch/.style={fill, shape=circle, minimum size=1.5pt, inner sep=0pt},
]
    \tikzstyle{branch}=[fill, shape=circle, minimum size=3pt, inner sep=0pt]
                        
    \node (s_init) [eqText, circle, draw, line width=0.5mm, inner sep=0.0cm]  {\(\abstractInitialState\)};
    \node (start) [labelText, left=3mm of s_init.west] {start};
    
    \draw [-latex] (start.east) -- (s_init.west);

    % % Failure and goal states
    \node(s_fail) [
        eqText,
        circle, 
        right=8mm of s_init.east, 
        inner sep=0.0cm, 
        draw=red, 
        line width=0.5mm, 
        xshift=0.0mm, 
        yshift=-3mm,
    ]  {\(\abstractFailureState\)};
    
    \node (s_goal) [
        eqText,
        circle,
        right=8mm of s_init.east,
        draw=green,
        line width=0.5mm,
        xshift=0.0mm,
        yshift=3mm,
        inner sep=0.0mm,
    ] {\(\abstractSuccessState\)};

    % Controller
    \node[branch, right=2mm of s_init.east] (c) {};
    \path [draw, -] (s_init.east) -- node [font=\tiny, yshift=1.5mm, xshift=0.0mm] {\(\controller\)} (c);
    \path [draw, -latex] (c) -- node [font=\tiny, above, xshift=0.0mm, yshift=0.5mm] {\(\bernoulliProb_{\controller}\)} (s_goal);
    \path [draw, -latex] (c) -- node [font=\tiny, below, inner sep=0.0mm, xshift=-1.5mm, yshift=-0.5mm] {\(1-\bernoulliProb_{\controller}\)} (s_fail);
    
    % % Self-loops at the absorbing states
    \path (s_fail) edge [loop right, draw=red] node [eqText] {\(1\)} (s_fail);
    \path (s_goal) edge [loop right, draw=green] node [eqText] {\(1\)} (s_goal);
    \end{tikzpicture}

==> figures/experiments/hf_sim_previous_day_left_failures_data.tex <==
\addplot [rlPoliciesHighSim, line width=\trajectoryWidth]
table {%
665 62
664.556157927308 70.0546812425004
663.850010551205 82.4604684516157
663.907624255362 95.3122886953127
664.842406707621 108.144634743109
666.13060754266 121.121706716139
667.15857464435 133.903191012466
668.138148031758 152.54409941291
668.912012579658 175.073362348589
671.884786431905 187.46364744962
677.330829295374 198.706327899347
686.526169361251 209.415266834254
702.075989059875 220.501815062806
722.746974372703 231.152651808425
735.319675816444 239.115675788698
741.751254763222 244.122209792145
748.891796694514 250.810004765893
755.758915093345 258.333486138172
763.386196079275 268.752304942315
772.019121191426 283.547166800529
780.112950614793 304.28515903456
783.110659788621 320.036262873744
786.484214272269 343.139231316
789.934678798826 363.581730653469
793.570239320545 384.058120570596
797.990956799327 409.445495593822
800.301158947504 426.753282004194
790.976921115698 441.266775454108
785.77990081885 450.871090198679
776.201122723931 459.318358612065
766.650674847197 467.891960370038
759.056092360073 474.869606805347
753.331036043337 480.19666366254
747.41777321061 485.913740666774
740.097056745667 493.278057208405
732.969281681561 500.579913216515
724.618521480892 510.475320132973
713.198957728503 527.715384422276
702.180597379787 542.927729005449
693.979051486173 551.464918063873
683.521259403806 559.0088989043
669.922719115325 564.877608739546
662.676775623157 566.8515346808
650.285621531455 568.823748876006
626.585381003747 568.355209300024
612.107592904303 563.286908989524
609.267584166795 561.520897776129
607.907560884732 561.486442023406
607.848675574995 559.668200128559
605.188538048722 559.253328232542
606.385891348728 558.725826431414
611.465858279427 567.974572873211
618.985618498531 576.752506152662
624.948422677257 596.659156916555
630.073027298523 617.047212293011
636.517073789148 639.536086392876
643.014720135833 659.313211351082
646.635538995763 669.839577724034
646.775729688099 670.215492530464
646.775729688099 670.215492530464
646.775729688099 670.215492530464
646.775729688099 670.215492530464
646.775729688099 670.215492530464
};
\addplot [rlPoliciesHighSim, line width=\trajectoryWidth]
table {%
665 62
664.848350036652 65.8392145771772
664.188397601484 73.524715797999
663.651490988855 83.4182829324065
663.887150175789 96.5941736650866
665.68302868935 117.109134866581
667.211823236504 134.712457856096
668.197971407236 153.078459477754
668.3878273236 168.491328419422
672.598476009674 188.406456886607
683.39765525532 204.959724843865
699.229235975604 217.539062960354
717.925151091836 227.162717811901
728.624442201305 233.263274867491
737.047427139856 239.101242086701
746.84882271992 247.638601214817
761.717517909166 265.404559438547
772.243178600572 283.392897317095
780.531722895074 304.838481951962
783.590831148644 322.825690230063
786.534937534881 343.297714430313
788.622794071836 355.653811335954
790.758685650623 368.456347879419
794.344803135859 388.986002683403
798.078515879946 409.372242701104
800.210936488547 425.896959566318
792.802512280255 437.097300241874
789.319263801938 446.213168194314
779.400712541981 455.142602606223
769.7948469378 463.916066771056
760.617169536648 472.463562142277
751.264753846588 481.557373991004
740.480523468911 492.595360411316
726.837042514692 507.785598180318
716.354493803169 523.208212512765
706.291988201586 538.13628408173
690.6308881049 554.568618084316
677.658589041512 562.307210808531
666.155989552319 565.962052385876
649.654662198614 568.820905601413
633.570841250237 569.536119175686
619.401461398023 567.246970240195
609.764908670395 562.88977062661
609.136351790786 563.214608938665
609.012738681696 559.582901020617
605.993190707377 560.498380257131
604.837403401373 559.260526966815
609.295409619024 562.353353398845
619.326754348285 575.750101104539
626.097418359891 600.931975048865
631.878124318211 623.847862654328
637.69801882993 643.317136517404
640.917750826988 653.290082246452
644.170068869627 663.332091570151
646.609681656821 670.221814460446
646.683109001337 670.497746465588
646.683109001337 670.497746465588
646.683109001337 670.497746465588
646.683109001337 670.497746465588
};
\addplot [rlPoliciesHighSim, line width=\trajectoryWidth]
table {%
665 62
664.558707647711 69.0717464693848
663.283000634729 87.2495135814368
664.115322784367 105.266057830181
666.644974242184 130.034261957866
667.805448366996 146.494577220827
668.283737329376 170.022215329288
672.886712662906 190.716129873709
681.721049610114 204.585219306473
697.160684566985 217.594003801615
713.585056730727 225.771626607678
732.456017551221 236.679556382261
748.774217119568 250.312776361766
763.295047620906 268.337584127327
773.343155793486 286.134410965901
779.176487826643 300.742974442821
783.234931936741 321.531881560076
785.891491141473 339.463504439275
788.930794156972 357.458181309914
790.998800752386 369.809468670792
792.372794562824 377.914134611455
795.456575900997 395.483672508957
798.908225983379 415.953254874138
800.338221847747 429.124527877735
795.003906229413 438.521658750416
791.057481083889 446.711123495872
783.129788068932 453.513711586815
775.648720066392 460.729713696971
762.684212311139 472.028824046041
748.545255872093 484.984016095655
733.760599396206 499.631148733176
720.084657316983 516.672186361371
707.24928585464 536.320494741073
693.866433896597 551.622682817565
675.089262436824 563.20572140252
657.859915525429 567.642586395725
637.647003212087 569.570511938066
625.327063276737 568.366635333629
609.459842320865 562.342106104754
608.081898651676 562.104656715774
605.328241590034 559.473288797436
605.443592667087 559.432851495885
609.517900668062 562.273637688408
620.387005500322 576.941707187842
625.818114329777 596.627684717913
631.123671408768 619.52250105701
636.757894601646 639.589521575226
642.966295870576 659.045573881551
646.774773090165 670.211555971589
646.962512904614 670.554596240686
646.962512904614 670.554596240686
646.962512904614 670.554596240686
646.962512904614 670.554596240686
646.962512904614 670.554596240686
646.962512904614 670.554596240686
646.962512904614 670.554596240686
646.962512904614 670.554596240686
};
\addplot [rlPoliciesHighSim, line width=\trajectoryWidth]
table {%
665 62
664.868818993813 65.7360728106114
664.160825454447 75.4987591458202
663.885321754738 93.9573861348793
665.253148065269 112.094507357966
667.12033633045 132.646339949744
668.194726978564 153.313296655461
668.535467404636 171.128337667084
673.906599227018 190.751769066601
683.818206803049 205.313573565025
697.501613231484 216.509571068158
717.278026608579 226.646272863196
733.55001473001 236.705579620389
748.18157669963 249.060764067585
759.098009578702 261.708436377356
771.244313279133 281.662518781707
779.374944653852 302.382293470088
782.647681969071 317.778975750545
785.643678610408 338.427175714259
789.552027515316 361.419504337439
793.621835650228 384.445396680267
797.470438368857 406.195336504835
800.249634637789 425.433950102901
795.752518837055 436.439386939068
783.30489531317 453.091655873571
771.290906576732 464.755490235792
756.65241099894 479.073504556958
745.663463001833 489.870457763033
731.24302393834 504.6069443493
724.983100421576 512.131574753079
720.372477330308 518.526310190418
711.85585767544 531.434839374756
697.078165623156 549.833426411257
675.509539440693 563.60316298055
653.42207286971 568.720170085194
638.6967072585 569.378630841273
628.827634234163 568.687984272836
616.820424589417 564.892961842924
609.498420429962 560.902546181134
609.621223701339 561.053835455918
606.263222979928 559.044976928312
606.407908909583 558.059743808534
603.602186159438 557.362635511108
607.581823829266 558.705970412281
618.692998544741 574.713772522079
626.131832368313 596.888797370606
630.521775117349 616.060252192285
635.527379275626 635.018705650561
641.700434847398 654.840204933474
646.591092061331 669.615506756081
646.591092061331 669.615506756081
646.591092061331 669.615506756081
646.591092061331 669.615506756081
646.591092061331 669.615506756081
646.591092061331 669.615506756081
646.591092061331 669.615506756081
646.591092061331 669.615506756081
};
\addplot [rlPoliciesHighSim, line width=\trajectoryWidth]
table {%
665 62
664.862415912646 65.710827773401
664.013316251935 77.361144291125
663.991781280187 96.6553201067701
665.48760158301 114.79180499317
667.073600127288 132.732249998913
668.126805416561 150.84895335888
668.364783232018 167.477747614864
672.646081064953 188.561112048099
685.518310384861 207.135223067828
704.137736641869 220.139323459357
724.751054595848 230.880809529484
742.344511142501 243.410796361004
757.392697990579 259.357581265897
767.414338915453 274.50775546841
776.838311322475 294.025548493883
781.256382711947 308.097272931049
784.981797003375 332.792856992333
787.62136758178 349.341643755725
791.028201452084 369.81440875686
794.571136867741 390.270783447244
798.060597329564 410.209311344719
800.406813509889 427.065906809909
796.707378743626 437.190564695647
789.375765679584 448.200687510813
783.129007806508 453.531545139358
776.347709972969 460.469275853561
768.603845341317 467.311595627378
758.757124650157 476.242124548219
744.120376510034 490.155304350166
729.255382002133 505.586292671654
717.196180659006 522.496543150093
705.881055982532 539.069089258117
689.536597945982 555.54080463726
673.512844442425 563.961078350885
651.482729710799 568.400231540071
628.76161761784 568.716397332033
612.153875258219 563.472702406933
608.25347210504 561.806625698449
608.184433896261 558.739496489345
605.437304305437 559.665854926698
608.197895530366 560.69377685559
617.394512519183 569.987332850191
624.418437873599 591.460176537565
627.938688395131 606.826070764704
630.554769047133 617.415528618779
633.840049414816 629.974170049741
637.537548079728 642.381918363517
644.722451003591 664.571057798785
646.881248930064 670.565291748763
646.881248930064 670.565291748763
646.881248930064 670.565291748763
646.881248930064 670.565291748763
646.881248930064 670.565291748763
646.881248930064 670.565291748763
646.881248930064 670.565291748763
};

==> figures/experiments/hf_sim_rl_policies_left_data.tex <==
\addplot [rlPoliciesHighSim, line width=\trajectoryWidth]
table {%
665 62
664.122191909173 74.3737824130109
663.620958365529 94.9633314810563
665.329825284745 115.007651875355
667.22998270117 136.176940962025
668.282414286947 159.49076585049
668.391813278768 171.263710068634
670.570761636669 183.896434187379
675.226630083753 195.628386644775
679.278869953057 202.234693116111
686.129886265716 210.05615041475
693.07680731778 216.666305704454
699.608136763445 221.756175805706
712.790663851463 230.187529534246
730.672493211327 239.886972481377
744.633721715839 247.649906046265
762.185941880288 260.336884691228
776.284676125295 276.80215995533
783.628074415735 291.4615332779
788.223416662787 306.071942404364
792.541644376843 325.859318791782
795.58175500062 351.60128724507
796.575614698937 367.219511118986
796.988974325295 377.688414419014
797.388464746106 393.06632409449
797.875779373489 415.151883174118
796.191925161229 437.851678254843
789.96508032999 456.472217946341
775.065425528387 473.724287173225
758.156170326773 489.271137137136
746.663419746194 499.596157961331
731.891621534235 509.890566238564
715.464753698609 516.749196635103
697.262941354399 518.213156799468
677.277488910285 520.103480405412
658.652852622551 528.432755953674
645.663592119676 539.696764851735
636.136182357412 555.485759337682
634.207661094642 562.261135354537
634.593867483741 571.469817921302
631.759718506135 591.003123524846
630.391821494185 608.445026217336
632.29066274515 626.932979935633
636.109484550933 641.379279714178
640.55500514335 653.916499834455
645.336889863417 666.717555023634
648.897521199011 675.308859464004
648.897521199011 675.308859464004
648.897521199011 675.308859464004
648.897521199011 675.308859464004
648.897521199011 675.308859464004
648.897521199011 675.308859464004
648.897521199011 675.308859464004
648.897521199011 675.308859464004
648.897521199011 675.308859464004
};
\addplot [rlPoliciesHighSim, line width=\trajectoryWidth]
table {%
665 62
664.959551496171 63.5350569376537
664.455857479996 70.8062274711321
663.821220945419 80.9887462507724
664.116096321974 99.0547366222362
665.729533602087 116.96187276725
667.450542363565 137.928704139131
668.294720595044 156.166793232778
668.395435219439 167.97229484528
671.629892972534 185.596547607734
676.771504296475 196.839949375717
692.600614489855 214.229604142659
708.976342207375 226.153332287827
724.869299812366 235.066452028195
736.394494927949 240.944026000644
747.710352473926 247.608014468151
760.11433391841 256.550820898304
773.297059201726 270.747817088019
782.402983729644 286.324002607101
787.801513155037 302.114818657191
792.503871383246 323.961564339699
794.813722361293 341.772942699135
796.193669294044 359.827634367811
797.011770951079 383.085402295036
797.421444423657 400.530823700829
797.392109611554 419.188609097307
795.180895147216 441.593551199894
789.749486209658 456.522306490658
779.099898395773 470.30037202683
763.101903523177 483.812961108178
746.441204880331 499.663012948317
729.389099930288 511.248290022978
718.148254281234 516.079417651065
703.861669359336 518.273892902529
684.677478014693 518.873073911581
662.840691354759 526.257700460457
646.734342495982 539.159696903369
635.034400980462 561.155831807815
634.82739639597 561.996292140508
635.927424594814 574.922563820777
632.765816940424 596.911422683869
632.049903120927 619.898377650726
636.699391423251 642.67590414137
644.519995386479 664.919381260695
651.501581628338 681.933124505876
651.615755691415 682.007962858127
651.615755691415 682.007962858127
651.615755691415 682.007962858127
651.615755691415 682.007962858127
651.615755691415 682.007962858127
};
\addplot [rlPoliciesHighSim, line width=\trajectoryWidth]
table {%
665 62
664.866070885453 65.8028850371776
664.291180448354 73.4940475755239
663.764835749235 86.3848693492138
664.514195471388 104.335063026455
665.444171030729 114.148486545625
666.40223142378 124.410730900635
667.435779318623 137.319756117383
668.095915335675 150.231933162553
668.356383018781 163.768091495552
668.599018653445 171.361448913733
670.090918127918 181.016377833038
672.62708973599 188.951085546853
676.849669944865 197.231522320685
681.559881498231 203.557561848201
687.224020550207 209.545106979479
694.106261949576 216.020674410481
702.530405256391 222.123554797614
709.206023372989 226.319660848265
720.286258547156 232.695903308531
732.304584564511 238.755839193656
739.464600250388 242.628726661117
750.480249976366 249.22745064005
764.510217938406 260.336961197143
778.484729792276 278.13592947062
784.273717898783 290.666099113407
790.117713503084 311.354438305881
794.038771102141 332.54860831562
796.1244072082 353.213881008754
797.211385959951 374.01572760301
798.187155981988 397.266373647281
797.985982215544 420.538101402551
797.313682869689 430.903700861884
793.031915492291 450.842889536256
785.169307737406 464.422782627803
778.794373005993 471.299206008486
770.287603000585 478.267915326597
761.143750367444 486.850422900515
751.716129860863 495.651824900313
741.661470254713 503.569890568504
731.118596931086 510.532800425147
717.185811961883 516.406565036492
697.482850140914 518.032582387095
680.804714178118 519.448800470697
671.231730821223 522.590051555769
652.625445407796 534.494132291221
640.362883261055 549.437692428222
635.602627126739 561.664258326089
635.400579878608 563.907579021998
635.975351182112 575.445836305754
634.987174129452 586.849416389959
632.91624859349 599.476215403051
632.196130665431 612.80012999362
634.533553441868 633.144711273525
640.441065084551 652.862265361392
645.655064972203 667.128546893048
646.790848996367 669.906395691441
646.989110368487 670.27525226424
647.029733732347 670.350756956273
647.029733732347 670.350756956273
647.029733732347 670.350756956273
647.029733732347 670.350756956273
647.029733732347 670.350756956273
647.029733732347 670.350756956273
647.029733732347 670.350756956273
};
\addplot [rlPoliciesHighSim, line width=\trajectoryWidth]
table {%
666.806954797405 130.027742506693
667.846992017244 145.505666918623
668.227623826561 155.915221992071
668.390851925428 168.498089854737
671.194766139868 183.773978462193
676.226112773028 195.161298689337
684.039157831825 205.72930937461
695.219747951732 216.269612929172
707.469796574093 224.688804075522
718.631204342521 231.275942550367
728.547490666292 236.338956165834
739.484140371301 242.085764020954
753.132603019774 250.535441467262
764.521484191664 259.783710624403
771.859613656636 267.963191778863
779.74922181671 279.79878035016
784.872246502821 291.592192400928
789.039922626301 306.380363049512
791.5794302992 319.420084488643
793.848257260629 331.821516266385
795.49600121315 346.9996827826
796.268196330189 357.530833961091
797.284452476852 376.71796647543
797.599145979889 392.067986081771
797.654170532708 405.012794478476
797.442782392701 418.164408935319
796.630394179251 431.872256204933
795.006699316585 442.191666626817
789.69404498549 456.372155932281
781.822357224898 467.048912118163
770.49840413241 477.252987412461
759.12711529524 487.505996190246
741.88005351051 503.057096000166
722.104066243887 514.294950217367
704.343225582397 517.532094965014
679.599541063283 519.596259257682
659.479606264818 529.221388613156
648.660503194055 538.410712665044
641.025366462337 548.687951484914
636.777117007328 558.873398247397
636.054239027443 562.023917528599
634.402662360592 577.589407811036
631.954456379196 590.604676274954
630.700113229164 602.477895372047
630.877006024123 615.525274305542
632.815604365097 628.748749514309
636.894885047981 643.176503763223
641.183630535949 655.423274961304
646.26314667371 668.826007176136
651.121807359943 680.600277321094
651.915623280296 682.468284949074
651.915623280296 682.468284949074
651.915623280296 682.468284949074
651.915623280296 682.468284949074
651.915623280296 682.468284949074
651.915623280296 682.468284949074
651.915623280296 682.468284949074
651.915623280296 682.468284949074
651.915623280296 682.468284949074
};
\addplot [rlPoliciesHighSim, line width=\trajectoryWidth]
table {%
665 62
664.751820636878 67.3276672373165
663.828534421367 78.6198591000755
663.847066292157 97.8105954182355
665.373345896276 114.674420310973
666.798427687733 130.038481403543
668.006138856681 149.427631215079
668.347428265378 168.690735760895
671.699897082915 186.464848668298
681.946954981741 203.828146685849
698.869982680201 219.450531416209
715.208919223743 229.705890345227
730.554288600453 237.716098299635
748.569959244293 247.814881534593
762.871276884215 258.566245424283
776.085971067889 274.255763316484
783.484620338921 288.385389280297
789.383588587775 308.242787398724
793.816963156919 332.023183004681
795.777940787284 350.085627234406
796.747265780793 365.151758256631
797.271778084137 378.155993181213
797.596144229576 391.588688838668
798.146496578549 406.517459434314
797.912051424093 419.453341115408
797.01053287032 432.414567888344
794.660872962084 444.786111466958
786.67875496301 461.221397660465
773.542695812971 474.503112143132
764.748262740951 482.242827482861
751.909221658313 494.86097523444
735.570334882184 507.553261094515
725.030988563196 513.450394811207
712.727525477659 517.399546100679
699.735197136378 518.173023750973
687.270572574234 518.893310723931
676.525489775958 521.101230904278
665.226312122929 525.428754285303
654.295478483324 532.594294132126
645.212750773996 541.178925918486
638.15110235985 552.368460548638
634.946584720222 560.908887339753
634.85261524701 561.447340175225
634.151428895745 569.981820182381
632.539606840045 581.531518669772
630.956415723668 592.134961982225
630.103080098784 608.140593472859
632.711758228491 629.551446848386
637.437942714755 645.276175647102
640.309893306787 653.300398153823
644.981979069083 665.736967201388
651.869494421667 682.770993381745
651.956901708815 683.014698870938
651.956901708815 683.014698870938
651.956901708815 683.014698870938
651.956901708815 683.014698870938
651.956901708815 683.014698870938
651.956901708815 683.014698870938
651.956901708815 683.014698870938
};

==> figures/experiments/hf_sim_rl_policies_right_data.tex <==
\addplot [rlPoliciesHighSim, line width=\trajectoryWidth]
table {%
663.481377566473 94.7349699729805
664.421178984759 108.285464696764
666.752847106513 131.500257209461
668.000234494188 150.944955246722
668.295317644128 167.836902924135
664.898854179067 186.780172669943
661.209216540082 194.610033043428
657.147955483808 201.130476422407
649.81880743338 208.48131740087
639.331775937618 215.014074752067
632.772585734996 217.663199678495
624.676070345945 219.755047747343
612.846316087329 223.911395580547
594.006409773625 232.05781766374
574.08327067448 243.847341746221
560.204842908612 254.735599975649
554.429992374871 260.616091066134
548.115999449115 268.554262278114
543.481008721099 277.24496341292
539.291100829286 286.290347122187
534.997443373255 298.034929308622
531.928931759628 310.636435238998
528.721858302689 323.265607611292
524.77384598535 343.749923667541
521.76534096617 367.250646708057
519.670112931016 391.39673555729
520.937227211448 411.0859423857
522.79990349227 429.048451393829
522.190495867248 449.537672180848
520.489635820563 462.429633372
519.906761262225 475.845971042264
526.44993231605 497.665400413696
535.395851705999 509.705860758209
554.259886091627 521.168698179919
573.847070571388 527.178434729375
584.801314084598 532.721883608839
598.675327637749 543.0839356718
604.273152856077 549.196189113111
613.126199777426 561.551227618161
621.484864547214 583.739430182885
625.015577395796 599.215137618513
628.617454441909 614.257535953684
632.711326492582 628.618185666797
636.707930279073 640.990414708682
640.752436352096 653.308475999734
644.905196788162 665.513271732706
646.268098544844 669.167254770695
646.53388744907 669.617703105141
646.53388744907 669.617703105141
646.53388744907 669.617703105141
646.53388744907 669.617703105141
};
\addplot [rlPoliciesHighSim, line width=\trajectoryWidth]
table {%
663.868532234481 78.7949031618072
663.839204359527 96.0545704007568
665.355664928062 114.035098260513
666.625514264851 127.394470023264
667.705759216132 142.272854778814
668.177240684998 153.487186347002
668.342380419292 165.705214147181
666.908665161705 180.103858467242
656.615517175059 201.631456270056
636.329833362584 216.435300937287
617.028414436867 222.315738284115
593.399684699781 232.23408623869
573.507368888839 244.245058987468
555.557352261338 259.449046347808
546.686294638329 270.958663780557
540.186481723625 284.180593101241
532.647425976562 308.031993958817
526.809286054513 333.014076929591
522.581763369287 358.668729534577
520.551747645638 379.685642194576
519.196199125705 394.404819521586
521.176689876354 417.55334898264
522.342005380147 430.331612507526
522.032918924529 446.054761851779
520.649551169643 459.40469163549
519.546208799891 472.085119631553
520.355041128492 481.503519294065
524.370942771083 494.57299313905
535.764701823857 511.119408375152
555.803996928655 522.780807691579
578.483624239136 530.668915400596
595.876985925295 541.861473255327
607.425228332313 554.22888223575
616.501135498806 569.257328006784
620.632012822332 581.647922046727
623.620539192779 594.212149117474
625.927039354231 605.102437567291
630.499674768468 622.024688814309
634.520329753471 634.837448068168
638.75565137053 647.386682831848
643.407064653833 661.38208705572
646.449925846005 669.8653036779
646.622256997078 670.185150313016
646.622256997078 670.185150313016
646.622256997078 670.185150313016
646.622256997078 670.185150313016
646.622256997078 670.185150313016
646.622256997078 670.185150313016
};
\addplot [rlPoliciesHighSim, line width=\trajectoryWidth]
table {%
667.158548262189 134.670514268757
667.929336931391 147.605107435982
668.314531321031 165.761430785561
666.070307232352 182.381738078164
660.381019896411 195.250440804131
646.893336670546 209.791245098399
632.122669854202 217.077109229586
615.661981013361 221.833493002911
601.192904338816 227.145179002327
592.33044333147 231.124548050941
579.946766226098 238.030411493021
570.912655541587 244.006724309639
564.706395306704 248.887111573393
555.608251982427 257.534560402178
546.688024312834 269.452619369252
537.825328608063 287.621538139587
532.192097581847 306.989897847658
528.358108794 324.607144457852
524.658067795391 342.604257213685
521.924224044076 362.573700507232
520.485874259484 378.124821962559
519.380727562442 397.24512264186
520.945363152775 410.275752525024
522.645701944597 423.275416546873
523.050180008985 436.425273686989
522.211197404956 448.963122067191
520.138879545921 465.722045287219
520.034045059073 477.972398766434
524.995268130482 495.002229307825
537.403536373 511.281789266558
556.84805452085 521.65757494591
572.536055706194 526.518075271402
593.984049520169 538.36641493713
607.123103798691 552.104514499683
617.593306628737 570.724677702276
622.152574589537 585.861084563892
626.34716447373 604.218527899414
630.071857120635 619.37270669819
633.623916453188 631.608435448964
637.759272741773 644.209596836513
643.363969855579 661.32789982367
646.422615502816 669.866987494321
646.422615502816 669.866987494321
646.422615502816 669.866987494321
646.422615502816 669.866987494321
646.422615502816 669.866987494321
646.422615502816 669.866987494321
646.422615502816 669.866987494321
};
\addplot [rlPoliciesHighSim, line width=\trajectoryWidth]
table {%
665 62
664.86022022747 65.9099503004188
664.160083928042 75.5670102118883
663.830379083871 83.5452488826608
663.975162527678 96.6273648706428
666.014932206283 119.47615276746
667.606283009545 139.864450594972
668.333808305068 160.818147646903
667.508954433617 177.351961121043
663.708245465536 189.914221030786
654.373833972575 204.684581101326
640.343764553588 215.376010528523
620.543165832255 221.219265426529
611.316978689836 224.707866112522
601.799769602754 228.554120536905
592.626533777636 232.827412870242
583.603665008774 237.831759541793
572.694853344578 244.975797367445
562.606873840963 252.788563144062
550.123799714318 265.701268451391
540.077639783711 284.779422614601
534.689206701177 298.309386206666
529.662940252822 319.672963978127
526.109766603393 335.90464627489
522.247235652481 361.919657929631
520.198350877014 383.915084002176
519.425836602384 400.561927634405
522.180802225261 420.963863472476
522.574601880597 444.083845123757
521.763204629086 454.249231402102
519.986625008547 466.90310388933
521.663282728811 487.140920974769
533.912112212966 509.443055143753
549.94957125646 521.043284058378
570.424216881049 527.401986857943
588.006233955263 535.295590024618
602.7734573483 547.507489287878
612.177923210415 559.732600126003
619.635832951603 576.520821058342
624.183978973595 596.6749294523
629.512210155109 618.703140693163
634.977892599415 637.132428823213
642.38621786139 659.83679917827
646.50837766533 671.059633124672
646.50837766533 671.059633124672
646.50837766533 671.059633124672
646.50837766533 671.059633124672
646.50837766533 671.059633124672
646.50837766533 671.059633124672
646.50837766533 671.059633124672
646.50837766533 671.059633124672
646.50837766533 671.059633124672
646.50837766533 671.059633124672
646.50837766533 671.059633124672
646.50837766533 671.059633124672
646.50837766533 671.059633124672
646.50837766533 671.059633124672
646.50837766533 671.059633124672
};
\addplot [rlPoliciesHighSim]
table {%
665 62
664.173535577026 73.1304102542679
663.465616085109 93.5271048207629
664.686587712361 109.703875018996
666.737632257434 130.304649946879
667.656563482561 143.205130868173
668.2969013201 161.291590084185
667.148581358277 179.190497931707
659.492495907857 197.922754527969
650.779344889631 207.673969306034
636.0717471973 216.643333366579
618.527770656685 221.297977268835
597.540635676593 230.074463812947
579.634554058445 239.920069102729
563.611674162961 251.60115347508
552.001088928963 263.028051904962
542.817462633955 278.678188301486
535.976216207617 295.085902561775
532.192871600308 309.263709303004
526.962940994013 332.153955057262
523.89184128599 350.35980686848
521.996022781377 365.944230921487
520.383710216888 384.178245721512
519.495426768553 403.985532285721
521.822592014292 421.804093320688
522.240564749484 444.96299859803
520.352377527249 463.399006657201
520.353949965536 475.830025016648
523.430127014198 487.994408954955
531.128465024063 501.726202272575
548.403490158969 515.693561772568
566.394632560462 521.850739984649
581.30824049564 528.381567920452
595.634352099736 538.381517151968
605.972073745738 549.939489626369
615.26961326278 564.82812004051
620.575110434439 579.876758382401
624.139312347753 595.195764211074
627.925814766341 611.062490489812
632.627701226751 628.042225639353
638.206657384115 645.295563119641
643.008425567703 659.962912990117
646.8853849441 670.643591712715
646.8853849441 670.643591712715
646.8853849441 670.643591712715
646.8853849441 670.643591712715
};

==> figures/experiments/hf_sim_rl_policies_right_data_obstacles.tex <==
\addplot [rlPoliciesHighSim, line width=\trajectoryWidth]
table {%
663.481377566473 94.7349699729805
664.421178984759 108.285464696764
666.752847106513 131.500257209461
668.000234494188 150.944955246722
668.295317644128 167.836902924135
664.898854179067 186.780172669943
661.209216540082 194.610033043428
657.147955483808 201.130476422407
649.81880743338 208.48131740087
639.331775937618 215.014074752067
632.772585734996 217.663199678495
624.676070345945 219.755047747343
612.846316087329 223.911395580547
594.006409773625 232.05781766374
574.08327067448 243.847341746221
560.204842908612 254.735599975649
554.429992374871 260.616091066134
548.115999449115 268.554262278114
543.481008721099 277.24496341292
539.291100829286 286.290347122187
534.997443373255 298.034929308622
% 531.928931759628 310.636435238998
% 528.721858302689 323.265607611292
% 524.77384598535 343.749923667541
% 521.76534096617 367.250646708057
% 519.670112931016 391.39673555729
% 520.937227211448 411.0859423857
% 522.79990349227 429.048451393829
% 522.190495867248 449.537672180848
% 520.489635820563 462.429633372
% 519.906761262225 475.845971042264
% 526.44993231605 497.665400413696
% 535.395851705999 509.705860758209
% 554.259886091627 521.168698179919
% 573.847070571388 527.178434729375
% 584.801314084598 532.721883608839
% 598.675327637749 543.0839356718
% 604.273152856077 549.196189113111
% 613.126199777426 561.551227618161
% 621.484864547214 583.739430182885
% 625.015577395796 599.215137618513
% 628.617454441909 614.257535953684
% 632.711326492582 628.618185666797
% 636.707930279073 640.990414708682
% 640.752436352096 653.308475999734
% 644.905196788162 665.513271732706
% 646.268098544844 669.167254770695
% 646.53388744907 669.617703105141
% 646.53388744907 669.617703105141
% 646.53388744907 669.617703105141
% 646.53388744907 669.617703105141
};
\addplot [rlPoliciesHighSim, line width=\trajectoryWidth]
table {%
663.868532234481 78.7949031618072
663.839204359527 96.0545704007568
665.355664928062 114.035098260513
666.625514264851 127.394470023264
667.705759216132 142.272854778814
668.177240684998 153.487186347002
668.342380419292 165.705214147181
666.908665161705 180.103858467242
656.615517175059 201.631456270056
636.329833362584 216.435300937287
617.028414436867 222.315738284115
593.399684699781 232.23408623869
573.507368888839 244.245058987468
555.557352261338 259.449046347808
546.686294638329 270.958663780557
540.186481723625 284.180593101241
% 532.647425976562 308.031993958817
% 526.809286054513 333.014076929591
% 522.581763369287 358.668729534577
% 520.551747645638 379.685642194576
% 519.196199125705 394.404819521586
% 521.176689876354 417.55334898264
% 522.342005380147 430.331612507526
% 522.032918924529 446.054761851779
% 520.649551169643 459.40469163549
% 519.546208799891 472.085119631553
% 520.355041128492 481.503519294065
% 524.370942771083 494.57299313905
% 535.764701823857 511.119408375152
% 555.803996928655 522.780807691579
% 578.483624239136 530.668915400596
% 595.876985925295 541.861473255327
% 607.425228332313 554.22888223575
% 616.501135498806 569.257328006784
% 620.632012822332 581.647922046727
% 623.620539192779 594.212149117474
% 625.927039354231 605.102437567291
% 630.499674768468 622.024688814309
% 634.520329753471 634.837448068168
% 638.75565137053 647.386682831848
% 643.407064653833 661.38208705572
% 646.449925846005 669.8653036779
% 646.622256997078 670.185150313016
% 646.622256997078 670.185150313016
% 646.622256997078 670.185150313016
% 646.622256997078 670.185150313016
% 646.622256997078 670.185150313016
% 646.622256997078 670.185150313016
};
\addplot [rlPoliciesHighSim, line width=\trajectoryWidth]
table {%
667.158548262189 134.670514268757
667.929336931391 147.605107435982
668.314531321031 165.761430785561
666.070307232352 182.381738078164
660.381019896411 195.250440804131
646.893336670546 209.791245098399
632.122669854202 217.077109229586
615.661981013361 221.833493002911
601.192904338816 227.145179002327
592.33044333147 231.124548050941
579.946766226098 238.030411493021
570.912655541587 244.006724309639
564.706395306704 248.887111573393
555.608251982427 257.534560402178
546.688024312834 269.452619369252
537.825328608063 287.621538139587
% 532.192097581847 306.989897847658
% 528.358108794 324.607144457852
% 524.658067795391 342.604257213685
% 521.924224044076 362.573700507232
% 520.485874259484 378.124821962559
% 519.380727562442 397.24512264186
% 520.945363152775 410.275752525024
% 522.645701944597 423.275416546873
% 523.050180008985 436.425273686989
% 522.211197404956 448.963122067191
% 520.138879545921 465.722045287219
% 520.034045059073 477.972398766434
% 524.995268130482 495.002229307825
% 537.403536373 511.281789266558
% 556.84805452085 521.65757494591
% 572.536055706194 526.518075271402
% 593.984049520169 538.36641493713
% 607.123103798691 552.104514499683
% 617.593306628737 570.724677702276
% 622.152574589537 585.861084563892
% 626.34716447373 604.218527899414
% 630.071857120635 619.37270669819
% 633.623916453188 631.608435448964
% 637.759272741773 644.209596836513
% 643.363969855579 661.32789982367
% 646.422615502816 669.866987494321
% 646.422615502816 669.866987494321
% 646.422615502816 669.866987494321
% 646.422615502816 669.866987494321
% 646.422615502816 669.866987494321
% 646.422615502816 669.866987494321
% 646.422615502816 669.866987494321
};
\addplot [rlPoliciesHighSim, line width=\trajectoryWidth]
table {%
665 62
664.86022022747 65.9099503004188
664.160083928042 75.5670102118883
663.830379083871 83.5452488826608
663.975162527678 96.6273648706428
666.014932206283 119.47615276746
667.606283009545 139.864450594972
668.333808305068 160.818147646903
667.508954433617 177.351961121043
663.708245465536 189.914221030786
654.373833972575 204.684581101326
640.343764553588 215.376010528523
620.543165832255 221.219265426529
611.316978689836 224.707866112522
601.799769602754 228.554120536905
592.626533777636 232.827412870242
583.603665008774 237.831759541793
572.694853344578 244.975797367445
562.606873840963 252.788563144062
550.123799714318 265.701268451391
540.077639783711 284.779422614601
534.689206701177 298.309386206666
% 529.662940252822 319.672963978127
% 526.109766603393 335.90464627489
% 522.247235652481 361.919657929631
% 520.198350877014 383.915084002176
% 519.425836602384 400.561927634405
% 522.180802225261 420.963863472476
% 522.574601880597 444.083845123757
% 521.763204629086 454.249231402102
% 519.986625008547 466.90310388933
% 521.663282728811 487.140920974769
% 533.912112212966 509.443055143753
% 549.94957125646 521.043284058378
% 570.424216881049 527.401986857943
% 588.006233955263 535.295590024618
% 602.7734573483 547.507489287878
% 612.177923210415 559.732600126003
% 619.635832951603 576.520821058342
% 624.183978973595 596.6749294523
% 629.512210155109 618.703140693163
% 634.977892599415 637.132428823213
% 642.38621786139 659.83679917827
% 646.50837766533 671.059633124672
% 646.50837766533 671.059633124672
% 646.50837766533 671.059633124672
% 646.50837766533 671.059633124672
% 646.50837766533 671.059633124672
% 646.50837766533 671.059633124672
% 646.50837766533 671.059633124672
% 646.50837766533 671.059633124672
% 646.50837766533 671.059633124672
% 646.50837766533 671.059633124672
% 646.50837766533 671.059633124672
% 646.50837766533 671.059633124672
% 646.50837766533 671.059633124672
% 646.50837766533 671.059633124672
% 646.50837766533 671.059633124672
};
\addplot [rlPoliciesHighSim]
table {%
665 62
664.173535577026 73.1304102542679
663.465616085109 93.5271048207629
664.686587712361 109.703875018996
666.737632257434 130.304649946879
667.656563482561 143.205130868173
668.2969013201 161.291590084185
667.148581358277 179.190497931707
659.492495907857 197.922754527969
650.779344889631 207.673969306034
636.0717471973 216.643333366579
618.527770656685 221.297977268835
597.540635676593 230.074463812947
579.634554058445 239.920069102729
563.611674162961 251.60115347508
552.001088928963 263.028051904962
542.817462633955 278.678188301486
535.976216207617 295.085902561775
% 532.192871600308 309.263709303004
% 526.962940994013 332.153955057262
% 523.89184128599 350.35980686848
% 521.996022781377 365.944230921487
% 520.383710216888 384.178245721512
% 519.495426768553 403.985532285721
% 521.822592014292 421.804093320688
% 522.240564749484 444.96299859803
% 520.352377527249 463.399006657201
% 520.353949965536 475.830025016648
% 523.430127014198 487.994408954955
% 531.128465024063 501.726202272575
% 548.403490158969 515.693561772568
% 566.394632560462 521.850739984649
% 581.30824049564 528.381567920452
% 595.634352099736 538.381517151968
% 605.972073745738 549.939489626369
% 615.26961326278 564.82812004051
% 620.575110434439 579.876758382401
% 624.139312347753 595.195764211074
% 627.925814766341 611.062490489812
% 632.627701226751 628.042225639353
% 638.206657384115 645.295563119641
% 643.008425567703 659.962912990117
% 646.8853849441 670.643591712715
% 646.8853849441 670.643591712715
% 646.8853849441 670.643591712715
% 646.8853849441 670.643591712715
};

==> figures/experiments/left_waypoints.tex <==
\addplot [semithick, color=waypoint, opacity=\waypointOpacity, mark=*, mark size=\waypointSize, mark options={solid}, only marks]
table {%
669.035522123351 189.396537242853
};
\addplot [semithick, color=waypoint, opacity=\waypointOpacity, mark=*, mark size=\waypointSize, mark options={solid}, only marks]
table {%
788.195635590714 311.060009576845
};
\addplot [semithick, color=waypoint, opacity=\waypointOpacity, mark=*, mark size=\waypointSize, mark options={solid}, only marks]
table {%
794.086814857822 449.899327905537
};
\addplot [semithick, color=waypoint, opacity=\waypointOpacity, mark=*, mark size=\waypointSize, mark options={solid}, only marks]
table {%
717.994916159572 515.827667341335
};
\addplot [semithick, color=waypoint, opacity=\waypointOpacity, mark=*, mark size=\waypointSize, mark options={solid}, only marks]
table {%
617.374036354003 567.843535178276
};
\addplot [semithick, color=goal, opacity=\waypointOpacity, mark=*, mark size=\waypointSize, mark options={solid}, only marks]
table {%
654.921298946443 690.05791413337
};


==> figures/experiments/left_waypoints_failure.tex <==
\addplot [semithick, color=waypoint, opacity=\waypointOpacity, mark=*, mark size=\waypointSize, mark options={solid}, only marks]
table {%
669.035522123351 189.396537242853
};
\addplot [semithick, color=waypoint, opacity=\waypointOpacity, mark=*, mark size=\waypointSize, mark options={solid}, only marks]
table {%
788.195635590714 311.060009576845
};
\addplot [semithick, color=waypoint, opacity=\waypointOpacity, mark=*, mark size=\waypointSize, mark options={solid}, only marks]
table {%
806.51173839312 444.061263145705
};
\addplot [semithick, color=waypoint, opacity=\waypointOpacity, mark=*, mark size=\waypointSize, mark options={solid}, only marks]
table {%
717.994916159572 515.827667341335
};
\addplot [semithick, color=waypoint, opacity=\waypointOpacity, mark=*, mark size=\waypointSize, mark options={solid}, only marks]
table {%
617.374036354003 567.843535178276
};
\addplot [semithick, color=goal, opacity=\waypointOpacity, mark=*, mark size=\waypointSize, mark options={solid}, only marks]
table {%
654.921298946443 690.05791413337
};


==> figures/experiments/planner_left_data.tex <==
\addplot [planner, line width=\trajectoryWidth]
table {%
665 62.0000000000004
665 62.0000000000004
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000017
665 62.0000000000017
665 62.0000000000017
665 62.0000000000018
665 62.0000000000018
665 62.0000000000018
665 62.0000000000019
665 62.0000000000019
665 62.0000000000019
665 62.0000000000019
665 62.000000000002
665 62.000000000002
665 62.000000000002
665 62.0000000000021
665 62.0000000000021
665 62.0000000000021
665 62.0000000000021
665 62.0000000000022
665 62.0000000000022
665 62.0000000000022
665 62.0000000000023
665 62.0000000000023
665 62.0000000000023
665 62.0000000000024
665 62.0000000000024
665 62.0000000000024
665 62.0000000000024
665 62.0000000000025
665 62.0000000000025
665 62.0000000000025
665 62.0000000000026
665 62.0000000000026
665 62.0000000000026
665 62.0000000000027
665 62.0000000000027
665 62.0000000000027
665 62.0000000000027
665.000016261975 61.9972700289871
665.000008688119 62.0179101146665
664.953883044314 63.6302312529412
664.868108263989 67.4139185442265
664.69325976133 76.0461075579602
664.439677987665 82.5799385518287
663.93750716569 93.2825425591528
662.855216768053 109.119375911075
662.284917364349 120.892760431015
661.895924693602 133.637021269207
661.849669249202 143.756348622044
662.234495946266 154.707250844492
662.902850501882 161.49832932349
667.693274798107 187.294808525736
666.064553644922 182.198217870102
666.047636469387 182.145714801844
666.331675073535 182.929608420427
668.120546093744 186.914056110388
674.688233048917 198.810831856601
678.54056798692 203.725741470162
683.663811831239 209.881815165375
689.424009057135 215.786383007618
698.040819947118 224.789203649926
706.981961738353 233.031692300155
713.985697073164 239.019253076289
720.001820949865 244.198940595296
729.178006094273 252.06718776096
734.977568863124 256.85970307526
743.047905318798 263.439682660044
750.457977562365 269.168162869717
758.139407758591 275.14433564504
764.671141274616 280.563309357669
771.433133285431 285.933218283872
785.071089395907 299.147317359329
786.969013479723 302.773634326355
785.186224878605 299.28576553288
785.189333353028 299.29184066041
785.235065722426 299.385073247604
786.391260008522 302.722388069766
788.574948211964 309.73266144706
789.714976833813 316.873294608203
791.664318812214 329.099135014974
792.367379963608 339.333273928777
792.947680875539 347.230905736326
792.853178077256 361.481576794607
792.715119138426 370.686407662299
792.095835678877 381.445253575289
791.487428861045 391.047594011761
790.748018150339 400.643953967195
790.140883087156 409.356183578459
789.546078541943 420.291907922062
789.929152112902 441.65911800794
790.710195340324 448.846414063725
790.229587984118 446.769218244894
790.242780358603 446.873062736121
790.261470040351 447.033588643618
790.324220662358 450.416385797718
790.033312803931 457.34549807348
788.295061887465 463.114134230038
785.707994741419 466.623668653451
781.323667664463 471.817676644623
773.962511928541 479.411515463781
764.862933235838 487.110714547686
757.195646460017 493.4333413556
749.296564356022 499.140736993945
723.835145190476 513.257129897031
718.234453959281 515.606064395028
715.794184088313 516.617027293073
721.538891211027 514.226290830274
720.837980918837 514.459375684334
716.042539856467 516.035414993339
706.366599567603 518.808281346832
697.506880797133 521.292086495686
690.222780129311 523.392419709677
679.965431175285 526.279071195219
671.115284700768 528.940645191311
660.871791083552 532.698593253053
655.091412712027 535.30548312163
647.294218393748 539.521274897227
639.876849943252 544.213717266512
633.766450704482 548.748649841341
621.795240450318 562.804988023824
619.171116421041 567.014989001747
618.727500449684 567.732711570913
618.738514229524 567.714945212474
618.738445270765 567.714938857758
618.736234583224 567.71855803238
617.956241463836 568.99755622841
615.953553243955 573.458279340434
615.353815049262 578.412002469796
613.664489996755 583.502428729532
616.569517524657 592.450549124581
620.041389212042 600.433589502221
625.243138313206 611.4225053279
628.929953174593 618.758926090548
633.27446199074 627.025274451622
639.152833950794 638.073340015342
643.170827216452 646.098992466256
645.965200627642 652.109943008028
649.315515851725 659.569151242788
653.083546235636 668.108586990282
655.51669003857 674.843970010539
657.374387719819 682.147269184675
657.547165004819 681.047099009191
657.561306540294 681.124539563944
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
657.561928292246 681.127922347763
};
\addplot [planner, line width=\trajectoryWidth]
table {%
665 62.0000000000014
665 62.0000000000015
665 62.0000000000015
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000017
665 62.0000000000017
665 62.0000000000017
665 62.0000000000018
665 62.0000000000018
665 62.0000000000018
665 62.0000000000019
665 62.0000000000019
665 62.000000000002
665 62.000000000002
665 62.000000000002
665 62.0000000000021
665 62.0000000000021
665 62.0000000000021
665 62.0000000000022
665 62.0000000000022
665 62.0000000000022
665 62.0000000000023
665 62.0000000000023
665 62.0000000000023
665 62.0000000000024
665 62.0000000000024
665 62.0000000000024
665 62.0000000000025
665 62.0000000000025
665 62.0000000000026
665 62.0000000000026
665 62.0000000000026
665 62.0000000000027
665 62.0000000000027
665 62.0000000000027
665 62.0000000000028
665 62.0000000000028
665 62.0000000000029
665 62.0000000000029
665 62.0000000000029
665 62.000000000003
665 62.000000000003
665 62.000000000003
665 62.0000000000031
665 62.0000000000031
664.999955200929 62.0021709394215
664.996456950898 62.3730139112626
664.946149084533 64.7114744121261
664.96461959366 71.5149489886006
665.212186683059 78.8688864857614
665.528577854089 87.2933214840809
665.929052200498 96.5189850325559
666.013656750196 106.263132762914
666.387125911585 117.670352025826
666.668062199004 125.204885955722
667.095808784407 135.681655914124
667.471249919565 143.749434543589
667.934303720403 154.344826427761
668.283743625701 161.02131466778
669.631618968668 188.754751294146
669.111483994407 183.525099742357
669.117848640064 183.599589069156
670.149716399784 189.558473649285
671.608369197269 194.768786286329
673.569306675814 200.284578700169
676.210967899885 203.384988742309
680.627837872724 207.723268833209
685.45624299136 211.93695917248
692.641446779497 217.850045986096
700.515053305171 223.954543350347
711.440784334989 231.97497543039
719.902612666512 237.994515752332
726.778353988693 242.791989984478
735.668021834481 249.425253635871
744.449944133159 256.130312504863
749.831597021165 260.369430707347
758.892786418012 267.827853775511
764.276808279231 272.687160994747
771.512233028958 279.713680675526
775.581982840541 284.047931675842
786.861961841172 303.980531050488
787.583390928612 304.743098615143
787.750985406508 305.380196423559
787.756374950239 305.397099073551
787.766316137064 305.439895259197
787.964112604848 307.943171553322
787.949823654337 312.390945067353
787.885474298995 328.859758869435
787.427955138618 336.826826829806
786.615659850019 349.770184137457
785.154519366911 363.890672990978
784.694668635012 371.036115429091
783.435771270207 383.266947364292
782.635124721969 392.890195093547
782.230088278686 400.229052775109
782.016927653675 410.279592462778
782.255782002092 418.601181587102
786.19816074904 440.356291282336
787.799636083651 444.057619249136
787.552563810621 443.393457192852
787.605575149204 443.505827520298
787.590759953949 443.47458241806
787.590759953949 443.47458241806
787.594594400834 443.482842257837
788.664372908573 446.136230679796
789.932493349275 449.521317956144
793.395692079154 461.381078822734
792.941749724858 466.092822729716
791.357730082487 469.872158373136
788.66825217746 472.774132458015
784.875582378777 475.758657556134
776.585502431528 478.786057693174
765.300747567102 483.019832602997
756.990413962403 485.819439278898
748.288637726398 488.763394067585
741.497605664676 491.135538455108
724.928494801821 499.366096745196
722.817898969182 501.938909879301
723.206169650241 501.10430499529
723.214824929029 501.093052890781
722.603009201149 501.897510920744
721.033906571958 503.72569789589
718.342898929139 506.629368582069
711.727895634335 512.351935511251
707.731671562201 515.064597299527
704.01972315252 517.997627298151
696.909260946531 521.781881171396
688.676378288545 525.95764425909
675.805705441504 531.994621732985
668.492421579424 535.356587536452
659.778122001676 539.170789410063
650.718057857831 542.952670528342
642.533150673843 546.500057644588
619.508268135519 559.427781576274
614.562161154853 563.124577606061
615.426451413808 562.196730773149
615.462193829386 562.165765871913
615.387467612769 562.231070812601
614.760901142122 562.882277907958
612.412959203364 565.782465886555
610.226949284821 569.735881823332
607.877338285604 575.207640731644
608.428001404257 579.889872757866
609.539263673714 584.164154896489
614.593635164591 593.705135037898
619.450653238259 601.918710293812
627.657549815606 614.454211789464
632.982376200869 622.153257257354
639.852883185202 632.016209563977
644.761389988777 639.280734430447
648.783825838133 645.98067288784
651.81114010457 652.102934387881
655.220961764613 659.591607133773
657.903598550462 668.058702048745
659.068611403315 674.991996715483
658.571476722529 680.334451261272
657.861037562533 682.416009002199
657.566638000547 683.628368201466
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
658.460795766528 680.394975280869
};
\addplot [planner, line width=\trajectoryWidth]
table {%
665 62.0000000000003
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665.00000250904 61.9992993179805
664.999994390116 62.0006187652449
664.997266950382 62.2299250105886
664.975581927331 63.2727507831934
664.935065023517 68.6897319264338
665.097929624124 79.6509292864113
665.368302120902 89.0217134742995
665.737125515811 101.65753053505
666.02481607625 111.643717782154
666.408920781448 122.532307659906
666.784748293602 132.193823829111
667.585883935009 144.357856637867
667.95613455213 151.049829050752
668.54078704016 160.029106947102
669.776340556388 180.914930316424
670.857659661238 188.983528848858
669.954758170363 183.352426875152
669.947831761919 183.302057568889
669.950925855297 183.322105436434
670.136419494572 184.464061113217
671.713240824727 190.051179505812
673.693169371241 194.814642232032
676.783307137519 200.313094872182
681.786515274146 208.298269940678
690.380393950079 218.853421894826
696.729630927105 225.91727975945
704.021286129371 233.619108975283
712.637692729742 242.27215317246
719.329752675087 248.614437752036
727.192660288338 255.641986489821
734.417544084968 261.968069854659
740.45399615286 266.966377974781
748.628386835582 273.490949879651
755.362159727338 278.735910242145
762.968327653482 285.142326963626
766.498040653689 288.685480952711
786.133519844195 307.891449241496
790.837996632175 312.546377545953
791.809633542585 313.509194079796
791.778606235858 313.478206014404
792.673151015304 314.547993992495
794.84189411852 317.855611378231
796.235090081099 321.553131210706
799.321642282433 328.959918341703
798.914842114651 332.835181272995
797.874418548443 343.255829977559
796.217584641889 351.297871189064
793.862074947281 363.028824812738
790.529088976405 374.808449377838
788.172091672803 383.428955986641
785.603720700632 392.849564227214
784.18661532093 399.904475952098
783.264628939995 408.077926013686
783.174980424197 414.179260856106
783.840485578798 422.876235330796
788.70190944655 441.467280151975
791.55407427818 446.80982080844
792.512894637417 448.410732931263
792.512286768008 448.40968057225
792.658940479556 448.598679914836
794.850094850176 452.695724318041
797.125993180619 458.130670539331
797.822272750981 462.801059789523
797.515628737734 466.432149272388
795.348417530478 469.91799153408
793.4432652415 471.572431466433
787.66511856585 474.131831173847
778.206809537166 477.844869357086
766.918763114009 481.552954475483
759.862595882572 484.083522208049
751.118777541326 487.109766647223
744.567314912315 489.95443153502
739.068858985251 493.003942598692
723.429576120323 505.557796225273
718.475305188673 511.154072163143
718.057367151148 510.71364644464
718.076317976474 510.690586854908
718.690294424879 510.158990664843
717.414945384113 511.41996007449
711.920361085827 516.569096336494
705.658795098587 521.597429594403
697.103387738379 528.507028064219
691.14739293034 532.446467545452
685.066709131807 535.881891599443
679.955364963194 537.798133727916
675.204353901829 538.404526848256
669.462456282401 539.532777048571
658.016279840351 541.559518898043
647.158352750061 543.562679495607
640.436900149962 544.885679562026
632.163718578909 547.142911594359
616.42299338593 555.056997242124
614.831405246618 556.19557691396
614.499837392614 556.53311405291
614.545501849181 556.486841604518
616.086641386253 554.870124479212
616.013020613124 554.953838670919
615.402416382162 555.910438231056
614.808689481176 559.186153649477
613.451413907633 561.619504197788
616.205562751404 566.8620636476
620.361729410131 573.357439648106
626.415222672342 583.142737239718
631.193855831844 590.766002132222
636.318151047979 598.881626618763
639.919027768201 604.9695337424
644.722436358771 614.679273576701
646.895052273265 620.411752708258
649.841233618799 630.422849129162
651.343717154707 636.901239004327
653.365327289484 646.72769334955
655.394820423018 657.545173957197
656.732198473038 667.410645830019
657.185838115637 673.786934058911
657.639950846756 682.383012908388
658.023267462285 687.678721750022
658.012633588857 688.715614120843
658.012865381581 688.694565376194
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
658.0128632819 688.694765710427
};

==> figures/experiments/planner_right_data.tex <==
\addplot [planner, line width=\trajectoryWidth]
table {%
665 62.0000000000004
665 62.0000000000005
665 62.0000000000005
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000009
665 62.0000000000009
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.0000000000011
665 62.0000000000011
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000014
665.000020229063 62.0063127863541
665.005428073771 62.2208967116315
665.214355548769 65.6617585847529
665.421373249254 70.1088251909377
666.045028428306 79.2254390381045
667.485646791029 95.473499132888
668.206970439848 104.072507928526
669.399481502925 118.170972395344
670.219605282701 128.731643321567
670.893251378464 138.28472434533
671.629577624922 148.197703805732
671.987291998401 155.269801277516
673.452482507647 182.314956344761
673.570334553525 186.909479564059
673.602166257979 189.002485091354
673.604127498813 189.393843544687
672.772740823768 194.585764667695
670.758569324762 201.931491228036
666.625646861521 207.814116752015
663.384458407038 211.263909202428
654.014587407566 219.746956493378
647.935636356695 224.589424706239
637.284537652983 233.097763484477
628.998263330829 238.51587929266
622.410928854541 242.684245978868
611.744927002633 248.690997559955
599.966693026897 254.916672567194
591.57260621545 258.972688630545
582.304676568596 263.857128723557
572.482350048544 268.561372142638
563.509645702263 272.972930437655
555.994810681953 277.038638058195
541.503308784359 288.572456953184
537.997280696901 293.382558532782
535.879952091837 296.785328410804
535.79069348309 296.927311699579
535.795811844181 296.918871568341
535.687022554923 297.092831925145
534.794369885256 298.694570049194
531.77416336804 305.198261769249
529.619109464256 311.893507303089
526.19232586001 322.478278982096
526.330321538312 327.158183125534
526.719244199541 332.691985740084
527.276243883843 343.494730890675
528.055422735284 357.243955909242
528.470177422575 366.427704839975
528.706090630541 379.103314789504
528.815181493702 387.099450291378
527.55111138346 412.086174549565
528.323993606835 407.167822268242
528.320913680763 407.192952673314
528.267831694932 407.535528023011
527.652998107344 411.364500865939
525.114940525132 425.813661656471
523.375819615327 435.019580684475
521.163911293692 446.837804470423
519.78920595118 454.37035259668
516.479405268542 474.977145657533
515.954022301007 479.653287813343
515.691395917478 482.144123808362
516.063059726088 477.856835711265
516.063134380406 477.856199010551
516.063134380406 477.856199010551
516.0001023867 478.767464777752
516.261405171906 483.44661053462
517.651382183629 488.713916669918
520.052507074984 497.601064719584
524.035202216351 501.426561570893
527.281950299606 503.161059852259
534.046404378559 505.927859878706
544.574500456724 510.199365923627
555.952682005998 514.068933666747
563.734622438253 516.667565838618
572.386218070684 519.720741580298
580.548756943077 523.015194829428
589.1015137273 527.33459338694
595.329834987667 531.603408997427
599.476057324794 535.259535753257
604.698169502588 540.731370748405
612.953169128358 556.120104063696
613.745830256206 560.933158425971
613.979493466495 563.886207528552
613.933696193257 559.565061451914
613.936817743765 559.603286672885
613.94891102594 560.621605628932
614.106900040549 567.218628091058
614.616159427782 572.92916947386
615.190481925597 585.949736880101
617.026128132485 596.237825759465
618.889173188651 605.19584782795
621.904146920731 616.66885396899
624.536297618222 625.432223929551
629.176478479795 638.538768527019
632.14495585882 645.580910495935
637.321337362715 657.132431795913
640.645245723415 664.154433026658
646.637845734522 675.695822070726
649.869838513735 681.198086223591
652.907164566973 686.050447367426
653.69552582038 686.277636677313
653.796077465455 686.441836685293
653.788134167413 686.429125298944
653.788134167413 686.429125298944
653.788134167413 686.429125298944
653.788134167413 686.429125298944
653.788134167413 686.429125298944
653.788134167413 686.429125298944
653.788134167413 686.429125298944
653.788134167413 686.429125298944
653.788134167413 686.429125298944
653.788134167413 686.429125298944
};
\addplot [planner, line width=\trajectoryWidth]
table {%
665 62.0000000000007
665 62.0000000000008
665 62.0000000000009
665 62.0000000000009
665 62.000000000001
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000012
665 62.0000000000013
665 62.0000000000013
665 62.0000000000014
665 62.0000000000014
665 62.0000000000015
665 62.0000000000015
665 62.0000000000016
665 62.0000000000017
665 62.0000000000017
665 62.0000000000018
665 62.0000000000018
665 62.0000000000019
665 62.0000000000019
665 62.000000000002
665 62.000000000002
665 62.0000000000021
665 62.0000000000022
665 62.0000000000022
665 62.0000000000023
665 62.0000000000023
665 62.0000000000024
665 62.0000000000024
665 62.0000000000025
665 62.0000000000025
665 62.0000000000026
665 62.0000000000027
665 62.0000000000027
665 62.0000000000027
665 62.0000000000028
665 62.0000000000029
665 62.0000000000029
665 62.000000000003
665 62.000000000003
665 62.0000000000031
665 62.0000000000031
665.000000650474 61.9995925621883
665.001067741718 62.1767520915603
665.051678532216 64.907841796326
665.187308418736 70.8098706407417
665.572703352829 82.3634061731421
666.232644480456 98.1442672322865
666.714122148338 110.988402351254
667.073874955013 123.236410342459
667.541694953657 133.055945641071
668.124733554792 145.003244880022
668.666931363389 155.931746412048
670.388450534723 185.56149691865
671.064532898254 189.931252931911
671.115186329695 190.537475847973
671.114555558789 190.529945969579
671.14638209926 191.84886906068
670.482606781464 196.673603181471
668.397618337145 202.073029615766
666.985701042372 209.8972096103
660.69009037361 216.91935957467
656.03164365911 220.850598844425
650.291420549615 225.214521445859
639.555808665573 233.1379308874
631.327274356091 238.429083610049
623.225398425161 243.669634357016
614.769306586049 248.50892664926
605.468776609021 253.529251523661
598.509531924677 257.119181245589
587.066302671984 262.724387615113
578.609930112748 266.793466906406
569.618854742913 271.256071472816
563.937391638077 274.565276037182
557.487039244999 278.480571171206
552.601510858674 281.906121278254
538.391101163051 294.838023351553
536.879604893552 296.265849166708
536.90894813092 296.230863757283
536.409315646527 296.835419360281
534.900796009349 298.96075035503
530.224252731502 306.591600698687
528.415100121782 310.389695392485
525.893101522624 317.354022692188
524.127871975479 323.575947670202
521.848868490573 333.632719829818
520.350198366258 341.890362585261
518.851664860589 353.030072297876
518.048099105695 362.022409893204
517.838064797245 370.15650310094
518.098607676979 376.474462857271
518.756846641063 386.886153556257
521.487342848214 409.2644861503
521.909929682581 412.092062295372
521.166257905007 405.931651412095
521.166257905007 405.931651412095
521.166257905007 405.931651412095
521.231790888203 406.3352199352
521.968072649566 412.581686270002
522.513830717919 419.534761704072
522.923731772622 430.6064207632
523.029452936014 439.940616759917
523.057327021228 450.773111428627
522.789729497752 459.431889893279
521.890113661565 482.183741207746
521.454383384274 486.570014444536
522.116922468344 481.558035788965
522.107270607182 481.688134854581
521.867371982959 485.195234555637
521.50605986764 495.069755090318
522.164957087144 502.952186078047
523.734006805051 507.701563402832
526.13726238886 511.080810175399
528.768756799644 512.706914129033
533.225460940438 514.890634359955
541.489360081107 518.779346479789
547.107273289658 520.945787291437
558.993936975685 525.357125916936
567.326062007856 528.185405807516
579.03557079325 532.010586700533
585.508120066488 534.457046266622
590.912820745119 536.707571406351
596.836774536744 539.423407306667
603.347666173744 543.087264350094
617.776831630762 555.665590715254
620.004010910202 559.686178757685
618.491399321352 556.23826379418
618.511141772451 556.272739832156
619.341055648032 557.82473701617
622.468863223306 563.950313921807
628.350123571838 575.943543822634
634.302553961959 588.520088779769
637.719179534724 595.965317259535
642.669489812681 606.929411881799
646.762252213326 616.005640471773
651.212671174821 626.263661913296
655.657843456694 637.361081130921
658.732860390555 647.335530369093
661.066784347699 656.864224525216
662.192012893417 663.822732440811
662.141889748685 673.595237746898
661.113381095622 677.566051472317
658.563063705298 682.980449110306
656.640529175544 686.534337836311
653.97506770562 690.698156695876
653.842534276351 690.902146732445
653.837420670735 690.910067198597
653.837420670735 690.910067198597
653.837420670735 690.910067198597
653.837420670735 690.910067198597
};
\addplot [planner, line width=\trajectoryWidth]
table {%
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
664.999979170411 62.0292572102472
664.993415848306 62.8565116097683
665.115760478492 68.140760380714
665.226652242049 71.6729968853555
665.633667545815 79.097272562252
666.090923105497 86.3542282837631
667.290616650119 101.219797770858
668.026384578924 111.643088520966
669.015798114843 123.46361808975
669.421815737479 133.66020659438
669.853598867393 145.355539161679
670.251185291682 155.280049256996
670.19052838265 161.592140998337
669.93233658551 184.878185036436
670.162875271268 189.569892311471
670.162949858835 189.566626144646
670.163043367675 189.567973568109
670.173178983969 189.895184122986
670.127158115434 192.77988575613
669.079520150465 200.600915715833
666.862798246633 211.480019325815
663.080276211938 215.881442918049
658.838344375623 219.123314803348
652.35309996115 223.356667854503
643.948212508646 229.275678323211
631.510108471524 236.124825115682
622.50392548414 240.821918086588
613.868757415084 245.147359076474
601.496004618815 251.069054578634
592.927215895263 255.212539896635
583.867312704404 260.059804116061
575.708302686725 264.369849087455
567.10648528203 269.343920292687
558.736139965978 274.449732821339
553.54215865315 278.284216688569
540.54226508769 291.490360186874
538.646262442539 295.140072985826
538.321609659167 295.808465591285
538.356153177756 295.738235391839
538.298628905544 295.855665325617
537.55189212062 297.569647083877
535.419327245033 303.960729663935
530.39910750073 319.375158265666
528.079948883917 328.294230719885
524.987893963931 342.053209568931
522.993421101684 352.926365976844
522.216132365039 359.991829950207
521.554333556303 368.934064631575
521.12903972495 377.340419824976
521.308460337259 386.162438851722
523.120317007821 402.38393807405
523.306298089033 404.005074292613
523.31686066564 404.103874770693
522.892494816605 402.884550654297
522.742276692897 407.67410855802
521.672041568665 422.338828514179
520.953959674402 429.778436732641
519.632245989675 443.187023171961
518.927741141066 450.872172395946
518.174113872095 460.518884783786
517.338477955074 473.521237647995
516.628860286163 478.824195568419
516.515987712921 479.688532372533
517.181152771426 475.586108999723
517.175652399322 475.633187036929
517.14037671563 476.516398686515
517.655511988066 479.829164705953
518.815295719213 482.372828173441
523.553423172251 490.117723272719
527.531755561994 493.868963083936
533.140125843516 499.723892744731
540.295225945639 505.373846584608
552.384472325605 514.063817885065
558.89636800236 518.425008837817
570.619107790852 525.793434155581
580.206076206979 531.585392881502
587.831910845183 536.415210177325
594.71703380019 541.012784514588
603.549216504124 547.02785370307
618.205656062153 560.834636433305
619.725516955756 563.350792654289
617.77658026487 559.271724645968
617.790664839265 559.294470871853
618.39460353191 560.34928696438
621.406455037597 565.58035486407
625.550626375045 572.664087912971
635.707506575521 590.127072999175
639.638653462719 597.026538903954
645.112441281579 606.861775155778
649.930758934786 615.039075896751
656.036528147713 625.068330999637
660.041670829634 631.762150555303
664.952696775031 641.41330900686
667.549069113147 649.31980218559
668.038894991291 654.111072128246
667.244352784208 661.475106364528
667.036370313902 663.966861296494
663.312416665671 670.887802932824
660.059471675102 676.21130737502
655.401128525663 684.005995515922
653.369882744121 688.229619499706
654.478680960047 684.759753229322
654.51342313544 684.670011527776
654.51342313544 684.670011527776
654.51342313544 684.670011527776
654.51342313544 684.670011527776
654.51342313544 684.670011527776
654.51342313544 684.670011527776
654.51342313544 684.670011527776
654.51342313544 684.670011527776
654.51342313544 684.670011527776
};

==> figures/experiments/plots_vs_time/test.tex <==
\begin{tikzpicture}
    \begin{groupplot}[
      group style={group size=2 by 2},
      width=4cm, height=4cm,
    ]
    \nextgroupplot
      \addplot coordinates{(0,0) (1,2) (2,1)};
    \nextgroupplot
      \addplot coordinates{(0,0) (1,2) (2,1)};
    \nextgroupplot
      \addplot coordinates{(0,0) (1,2) (2,1)};
    \end{groupplot}
\end{tikzpicture}

==> figures/experiments/previous_day_left_failures.tex <==
\addplot [rlPolicies, line width=\trajectoryWidth]
table {%
665 61.9999999999999
665 61.9999999999999
665 61.9999999999999
665 61.9999999999998
665 61.9999999999998
665 61.9999999999998
665 61.9999999999998
665 61.9999999999998
665 61.9999999999998
665 61.9999999999998
665 61.9999999999998
665 61.9999999999998
665 61.9999999999997
665 61.9999999999997
665 61.9999999999997
665 61.9999999999997
665 61.9999999999997
665 61.9999999999997
665 61.9999999999997
665 61.9999999999997
665 61.9999999999997
665 61.9999999999997
665 61.9999999999996
665 61.9999999999996
665 61.9999999999996
665 61.9999999999996
665 61.9999999999996
665 61.9999999999996
665 61.9999999999996
665 61.9999999999996
665 61.9999999999996
665 61.9999999999996
665 61.9999999999995
665 61.9999999999995
665 61.9999999999995
665 61.9999999999995
665 61.9999999999995
665 61.9999999999995
665 61.9999999999995
665 61.9999999999995
665 61.9999999999995
665 61.9999999999994
665 61.9999999999994
665 61.9999999999994
665 61.9999999999994
665 61.9999999999994
665 61.9999999999994
665 61.9999999999994
665 61.9999999999994
665 61.9999999999994
665 61.9999999999994
665 61.9999999999994
665 61.9999999999993
665 61.9999999999993
665 61.9999999999993
665 61.9999999999993
665 61.9999999999993
665 61.9999999999993
665 61.9999999999993
665 61.9999999999993
665 61.9999999999993
665 61.9999999999993
665 61.9999999999992
665 61.9999999999992
665 61.9999999999992
665 61.9999999999992
665 61.9999999999992
665 61.9999999999992
665 61.9999999999992
665 61.9999999999992
665 61.9999999999992
665 61.9999999999992
665 61.9999999999991
665 61.9999999999991
665 61.9999999999991
665 61.9999999999991
665 61.9999999999991
665 61.9999999999991
665 61.9999999999991
665 61.9999999999991
665 61.9999999999991
665 61.9999999999991
665 61.999999999999
665 61.999999999999
665 61.999999999999
665 61.999999999999
665 61.999999999999
665 61.999999999999
665 61.999999999999
665 61.999999999999
665 61.999999999999
665 61.9999999999989
665 61.9999999999989
665 61.9999999999989
665 61.9999999999989
665 61.9999999999989
665 61.9999999999989
665 61.9999999999989
665 61.9999999999989
665 61.9999999999989
665 61.9999999999988
665 61.9999999999988
665 61.9999999999988
664.999993156354 62.0018105199637
664.999647892245 62.045383513685
664.950983664681 63.977097462642
664.652850008543 68.053232960739
662.985782462891 76.6948228819399
659.836805578675 95.211172284493
658.307276225735 107.120897285684
659.622485859604 126.798731328089
662.130862207681 138.410965901852
664.176429055089 152.8189445371
664.996672622277 164.395264032131
665.774553309685 181.331998555285
666.274695711983 195.173735611343
665.891202651939 201.013499997306
668.386429340091 202.420278392894
673.149229884312 211.52372954198
687.24794123356 223.302348501447
697.293829276109 227.129302690537
712.455195910595 234.387789529662
726.692513827949 240.289720318933
736.220307232341 246.131071165173
747.609034082673 256.062034815137
756.156980902751 265.270574857784
762.422840690368 274.612743365871
768.866532174566 287.76931367973
771.85858983241 300.754741668211
773.764022459967 307.727342322385
778.075296800209 321.364215272402
781.620741442741 333.841493610181
784.545571243311 346.756749825508
786.80472194594 357.841149964188
789.947045308264 373.537192457037
792.512901117826 385.980267461857
796.02826645165 403.842109443003
798.30195284368 416.394039286893
799.86936512341 435.428285509461
797.714385443684 445.137926181734
793.118133907646 452.08274860213
784.563889018207 459.271110346209
776.455582493721 464.672195387135
764.145622413259 471.118018444651
749.162255910553 475.896316021132
737.668325914483 477.773794332973
741.578867127149 478.013821217077
738.590135858531 478.695362818049
736.370369420581 479.213692690177
733.692046533588 479.925946307173
731.6385725181 480.567615471202
728.576073675817 481.629619711985
726.51329305291 482.489018216973
724.504728061183 483.484218697333
722.761853916614 484.651136877123
720.712736743501 486.07685208463
718.593763285487 487.761351037506
716.219556532814 491.139818977244
715.188745952023 493.836142100322
713.930136491303 498.546008352553
715.564659130775 503.478321812033
717.478705122434 508.575176348712
720.606898013601 512.809935062722
722.530003966664 514.998821834425
726.303506996093 517.76342685379
728.438824826768 519.194133638966
732.543667284209 520.322832711438
735.567847990628 520.703858925911
739.550363285846 520.166214710892
743.684916249824 519.195762616486
747.089928097504 517.440760744042
750.69845747278 515.103672393757
753.846172874422 512.576260422054
756.360589654435 510.394099969198
758.773816192278 507.634053869921
760.488466422809 505.22634749365
762.287975697092 502.340413659887
764.094160593873 499.068436697191
765.337043689725 496.19747500371
766.145366398897 494.172903332878
766.88401934605 491.828459240154
768.027735727329 487.501629669627
768.501487946564 485.254789026594
768.846203103333 482.852193497179
769.218465388133 479.970864251863
769.48466648091 477.123866540728
769.649439613547 474.312817651316
769.750077908708 471.330227856056
769.719396213142 468.219153653066
769.562633099599 465.054872720693
769.321677314028 462.179823008133
769.020499698277 460.345048445207
768.598394623049 457.248271420149
768.088897496233 454.135934955046
767.662291395593 451.641655805196
767.214439845606 449.656999563406
766.589963081773 447.094536774637
766.04195808552 444.762646796485
765.34518379109 442.327353983716
764.569319421726 439.922857702394
763.971603026553 438.114190399718
763.169313166314 435.643744807909
762.518542835046 433.887263621521
761.739341136887 431.876378464569
761.043710642984 430.186334191454
760.27555017546 428.149434335988
759.236364754317 425.831486259686
758.180218528322 423.661220682078
757.228017314789 421.704429732234
757.511806749449 422.071804435931
757.674810288002 422.354399973862
757.674810288002 422.354399973862
757.674810288002 422.354399973862
757.674810288002 422.354399973862
757.674810288002 422.354399973862
757.674810288002 422.354399973862
757.674810288002 422.354399973862
757.674810288002 422.354399973862
757.674810288002 422.354399973862
757.674810288002 422.354399973862
757.674810288002 422.354399973862
757.674810288002 422.354399973862
757.674810288002 422.354399973862
757.674810288002 422.354399973862
};
\addplot [rlPolicies, line width=\trajectoryWidth]
table {%
665 61.9999999999997
665 61.9999999999997
665 61.9999999999997
665 61.9999999999996
665 61.9999999999996
665 61.9999999999996
665 61.9999999999995
665 61.9999999999995
665 61.9999999999995
665 61.9999999999995
665 61.9999999999995
665 61.9999999999994
665 61.9999999999994
665 61.9999999999994
665 61.9999999999994
665 61.9999999999993
665 61.9999999999993
665 61.9999999999993
665 61.9999999999993
665 61.9999999999993
665 61.9999999999992
665 61.9999999999992
665 61.9999999999992
665 61.9999999999992
665 61.9999999999991
665 61.9999999999991
665 61.9999999999991
665 61.9999999999991
665 61.9999999999991
665 61.999999999999
665 61.999999999999
665 61.999999999999
665 61.999999999999
665 61.9999999999989
665 61.9999999999989
665 61.9999999999989
665 61.9999999999989
665 61.9999999999989
665 61.9999999999988
665 61.9999999999988
665 61.9999999999988
665 61.9999999999988
665 61.9999999999987
665 61.9999999999987
665 61.9999999999987
665 61.9999999999987
665 61.9999999999987
665 61.9999999999986
665 61.9999999999986
665 61.9999999999986
665 61.9999999999986
665 61.9999999999985
665 61.9999999999985
665 61.9999999999985
665 61.9999999999985
665 61.9999999999985
665 61.9999999999984
665 61.9999999999984
665 61.9999999999984
665 61.9999999999984
665 61.9999999999984
665 61.9999999999983
665 61.9999999999983
665 61.9999999999983
665 61.9999999999983
665 61.9999999999982
665 61.9999999999982
665 61.9999999999982
665 61.9999999999982
665.000001275016 61.99860213039
665.000146622637 62.0553524331606
664.634529381008 66.4523281585652
662.35998171919 75.3663369622226
658.982394666534 88.1566178519197
658.093673465837 99.4570296881397
659.524495641265 110.86540830123
662.398228993255 124.291671626107
664.173973252281 136.464012400801
665.428960145714 151.586650465581
665.952815087773 163.726724545918
666.286119726501 174.956956077388
666.422940874727 185.99132862072
665.864772444464 196.183908210687
665.715181828874 200.021620806756
667.050371257295 207.358760748531
674.78546487133 222.61475338175
683.214758089399 229.098381554919
698.147221368199 234.168918792772
710.616899182502 236.63088916717
721.632112439117 239.790983478988
730.720657905375 243.953643998144
742.110395168021 252.117629473387
749.042521844099 258.159571488889
755.57251329974 266.010002848798
760.375824633458 272.814792400492
766.896412811634 283.969301304468
770.641379164285 295.568970019475
772.941249908729 304.240461719888
775.849925932653 315.407828052733
779.52364221521 328.237671314118
782.123808537524 338.4035047825
784.668871541071 349.525987237565
787.093317026205 359.50634323202
790.164506752793 375.029553147645
792.439201575325 384.717024177593
795.004312373881 397.566975439377
797.434173224941 410.454322053751
798.777938974894 418.332318544655
799.926590300717 428.798243649758
798.130822976019 439.286349370517
793.854321913945 446.400762404615
787.025521387044 452.815798899643
779.001677983131 458.921687233372
769.118391495228 466.788308210797
759.205479461342 472.151711017097
746.870376962323 476.449902287179
736.806788380141 478.475800589028
732.275778495472 479.551688518368
738.46858333288 479.31978726029
736.806335574871 479.746237955151
734.692592887836 480.329566309407
732.68087733368 480.948118324489
730.010381179387 481.85828691281
728.037415638666 482.658854631183
726.67737660148 483.360673832851
725.087536611882 484.15149369988
723.159249588057 485.222835652861
721.830128790641 485.997539270926
719.806491286528 487.428304671464
718.043564551258 488.937216293023
716.7663302602 490.396800915217
715.481340648202 493.646825807181
714.80273885081 497.139981307298
714.595090617279 501.872134345383
716.636641711444 506.453993206602
718.277609528151 511.163388990707
720.50936723931 514.211414372602
722.162973123051 515.906816091935
725.247384314948 518.031459986903
727.831830490553 519.68679048993
731.534604898893 520.48326423035
735.792503694472 520.399351307034
738.991098976674 520.122127111819
742.584685310371 518.813427553332
745.410699640901 517.426584624355
747.777094689426 515.932210528454
750.896257184779 513.823618621153
752.836916872057 512.046498377003
755.341022295319 509.593771448593
757.551170355386 506.863931541068
758.966425202276 505.053933430619
760.459832367189 502.756322965656
761.97795309873 500.01683867155
763.652019881486 496.526231951979
764.547818247996 494.084939152005
765.602606196601 490.551363851645
766.259567744815 487.777469114991
766.755037327761 485.826795540042
767.247270824716 481.729269887364
767.411719887903 479.390514687523
767.471955321379 476.828087185902
767.482111765982 474.502547915191
767.322532055087 471.866867695019
768.532863120753 468.703747456749
768.13583273859 466.230807528526
767.77960190278 464.355400160643
767.128451867396 461.354207573432
766.561199595538 458.697250188054
766.141034921417 457.136626356095
765.506435667251 455.020398401233
764.813841722959 452.746670612255
763.98377243801 450.492709581838
763.104811323562 448.285365824234
762.111399165138 446.034326567076
760.831406217895 443.375405147966
759.661608214087 441.125184458346
758.546737964687 439.088249398527
757.057619438729 436.6317098741
755.966834860302 434.924536658613
754.385246899817 432.65508420203
753.14552264488 430.849180160659
752.890318944152 430.498107484984
753.564226020965 431.424328202617
753.564226020965 431.424328202617
753.564226020965 431.424328202617
753.564226020965 431.424328202617
753.564226020965 431.424328202617
753.564226020965 431.424328202617
};

==> figures/experiments/right_waypoints.tex <==
\addplot [semithick, color=waypoint, opacity=\waypointOpacity, mark=*, mark size=\waypointSize, mark options={solid}, only marks]
table {%
669.035522123351 189.396537242853
};
\addplot [semithick, color=waypoint, opacity=\waypointOpacity, mark=*, mark size=\waypointSize, mark options={solid}, only marks]
table {%
534.149039705691 302.312118863499
};
\addplot [semithick, color=waypoint, opacity=\waypointOpacity, mark=*, mark size=\waypointSize, mark options={solid}, only marks]
table {%
520.94391334034 411.812930117392
};
\addplot [semithick, color=waypoint, opacity=\waypointOpacity, mark=*, mark size=\waypointSize, mark options={solid}, only marks]
table {%
517.183964133093 486.288565507564
};
\addplot [semithick, color=waypoint, opacity=\waypointOpacity, mark=*, mark size=\waypointSize, mark options={solid}, only marks]
table {%
617.374036354003 567.843535178276
};
\addplot [semithick, color=goal, opacity=\waypointOpacity, mark=*, mark size=\waypointSize, mark options={solid}, only marks]
table {%
654.921298946443 690.05791413337
};

==> figures/experiments/rl_policies_left_data.tex <==
\addplot [rlPolicies, line width=\trajectoryWidth]
table {%
665 61.9999999999996
665 61.9999999999995
665 61.9999999999995
665 61.9999999999995
665 61.9999999999995
665 61.9999999999994
665 61.9999999999994
665 61.9999999999994
665 61.9999999999994
665 61.9999999999993
665 61.9999999999993
665 61.9999999999993
665 61.9999999999993
665 61.9999999999992
665 61.9999999999992
665 61.9999999999992
665 61.9999999999992
665 61.9999999999991
665 61.9999999999991
665 61.9999999999991
665 61.9999999999991
665 61.999999999999
665 61.999999999999
665 61.999999999999
665 61.999999999999
665 61.999999999999
665 61.9999999999989
665 61.9999999999989
665 61.9999999999989
665 61.9999999999989
665 61.9999999999988
665 61.9999999999988
665 61.9999999999988
665 61.9999999999988
665 61.9999999999987
665 61.9999999999987
665 61.9999999999987
665 61.9999999999987
665 61.9999999999986
665 61.9999999999986
665 61.9999999999986
665 61.9999999999986
665 61.9999999999986
665 61.9999999999985
665 61.9999999999985
665 61.9999999999985
665 61.9999999999985
665 61.9999999999984
665 61.9999999999984
665 61.9999999999984
665 61.9999999999984
665 61.9999999999983
665 61.9999999999983
665 61.9999999999983
665 61.9999999999983
665 61.9999999999983
665 61.9999999999982
665 61.9999999999982
665 61.9999999999982
665 61.9999999999982
665 61.9999999999981
665 61.9999999999981
665 61.9999999999981
665 61.9999999999981
665 61.999999999998
665 61.999999999998
665 61.999999999998
665 61.999999999998
665 61.999999999998
665 61.9999999999979
665 61.9999999999979
665 61.9999999999979
665 61.9999999999979
665 61.9999999999978
665 61.9999999999978
665 61.9999999999978
665 61.9999999999978
665 61.9999999999977
665 61.9999999999977
665 61.9999999999977
665 61.9999999999977
665 61.9999999999976
665 61.9999999999976
665 61.9999999999976
665 61.9999999999976
665 61.9999999999976
665 61.9999999999975
665 61.9999999999975
665 61.9999999999975
665 61.9999999999974
665 61.9999999999974
665 61.9999999999974
665 61.9999999999974
665 61.9999999999973
665 61.9999999999973
665 61.9999999999973
665 61.9999999999973
664.999996070248 61.9939880391531
664.988929826937 62.5247426467752
664.751133644551 65.3856113338874
663.414129901109 71.4534546572471
658.751725900413 85.9398475416605
656.297152517041 105.913437285763
657.979959683266 122.480437847617
660.882095480968 137.301038815752
663.471236276057 152.972568647609
663.200871228303 164.573998416952
664.581356312594 181.099779473332
664.974954386535 190.173831026483
664.815129469053 197.862191397135
667.112817422188 207.614968409087
671.922921373477 215.955282710041
683.032789449614 229.813199074618
692.033912337081 235.520172300364
707.609179675929 245.488279018564
716.766828530821 249.703646751765
727.913640883203 254.742264855625
735.151984175537 258.151161728729
742.369116013106 261.785002757787
751.773992776902 267.43407727807
762.017642012762 275.87682060161
768.629169256059 283.439003745411
773.734494436326 291.19991504896
779.680248438066 305.107907434092
782.428155137676 311.666477896342
785.260312359358 326.296118281651
788.3443499041 344.617659963522
790.091701218443 357.055257999006
791.319277416637 370.912066819553
792.281587631361 386.18390944739
792.541454960974 396.750280789649
792.356703732524 412.533508126712
791.348471949621 422.473162069934
787.659921980856 432.844376010045
783.319453168383 438.783169821877
779.559384156377 444.804809434407
778.075191777507 452.978033134289
773.239550947687 460.938170014881
763.449922315394 470.763631194484
756.54543201893 478.58262977059
748.348570690741 489.106588843378
740.226913209659 495.440582468027
728.389867366328 499.907628275567
721.580414114663 500.456009270508
716.605056677507 499.888958812449
709.073490760792 497.925816778534
700.802079359497 496.94838184893
687.732126300199 498.459140961518
676.79810237946 502.57201947607
668.115172662005 508.258154153823
659.735966178614 513.228339332878
651.208479487019 520.491672973042
645.367184390122 529.305421057875
641.954564158606 541.436963354137
642.55514668499 549.85066088229
645.720353744469 557.42921154911
641.919562071689 555.724531728573
642.411676670511 555.88744160539
642.713599324146 555.896533411765
641.072666184621 555.735936490819
641.184291166049 555.671072207973
641.428162224937 555.852458999708
641.47575244421 555.722480285924
641.589940295647 555.066505479851
641.160478195244 554.386646365537
638.411140312903 552.277147999567
626.699271506788 548.873427938197
619.157410754812 551.5042986718
612.54344978594 558.959786228979
611.680032824295 563.689463844203
611.899960776352 561.3764627725
614.682827253253 565.891349156051
617.146145245813 572.532070928748
621.804018902425 587.497611189271
627.574328706249 602.727108247663
630.323893172984 610.064664343251
633.99086011646 620.272274517934
638.026593794133 632.231624537915
642.237747785021 645.752464474229
645.495880394362 655.867285483285
651.003436519691 670.434310506885
655.442985087298 680.855592481343
652.580641774492 674.510680452128
652.141959550306 673.536064061237
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
652.139718471487 673.530940605037
};
\addplot [rlPolicies, line width=\trajectoryWidth]
table {%
665 62.0000000000012
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000017
665 62.0000000000017
665 62.0000000000017
665 62.0000000000017
665 62.0000000000017
665 62.0000000000018
665 62.0000000000018
665 62.0000000000018
665 62.0000000000019
665 62.0000000000019
665 62.0000000000019
665 62.0000000000019
665 62.0000000000019
665 62.000000000002
665 62.000000000002
665 62.000000000002
665 62.000000000002
665 62.000000000002
665 62.0000000000021
665 62.0000000000021
665 62.0000000000021
665 62.0000000000021
665 62.0000000000021
665 62.0000000000022
665 62.0000000000022
665 62.0000000000022
665 62.0000000000022
665 62.0000000000023
665 62.0000000000023
665 62.0000000000023
665 62.0000000000023
665 62.0000000000024
665 62.0000000000024
665 62.0000000000024
665 62.0000000000024
665 62.0000000000024
665 62.0000000000025
665 62.0000000000025
665 62.0000000000025
665 62.0000000000025
665 62.0000000000025
665 62.0000000000026
665 62.0000000000026
665 62.0000000000026
665 62.0000000000026
665 62.0000000000027
665 62.0000000000027
665 62.0000000000027
665 62.0000000000027
665 62.0000000000028
665 62.0000000000028
665 62.0000000000028
665 62.0000000000028
665 62.0000000000029
665 62.0000000000029
665 62.0000000000029
665 62.0000000000029
665 62.0000000000029
664.999915863548 62.0115272670753
664.990289828151 62.7336533422887
664.385953605411 68.0502241555778
660.587231820984 80.5761521250494
657.401339838656 98.126674882823
656.317158740549 106.708192006307
657.497934511111 126.890258367417
660.332850589369 138.790867903938
662.782039788454 157.262963604641
663.590776869986 168.19301273936
664.424772683214 180.054567885552
664.616189194543 193.34639649174
665.012804548796 199.926153536928
671.164100238923 209.195745726081
677.964864687509 217.261077713569
688.640405982405 228.667762227896
697.868372128384 233.981572629198
705.050738818043 237.582188543443
721.928483851773 245.174277071327
733.246161637224 250.361368306214
740.735745270799 254.029786423107
749.935044237066 259.295510315045
761.713717419241 268.733280130288
769.826128492823 278.848054711292
774.952129695244 286.58988084093
781.52885542316 302.937549126419
782.221200299442 305.931685141834
784.037468373478 314.588544853322
786.830697154743 327.803133480622
789.701774892172 339.752975730781
791.25683378936 352.722492471611
792.51621712795 365.818119399646
793.191881958207 381.753060897363
793.315429546594 392.433517325484
793.153831005711 405.1345278183
791.448014207346 424.12880371385
788.816623442346 431.63217072714
784.123750591428 438.551777747547
781.004249383079 443.074190563903
774.868639498004 455.839496549095
769.216961043921 464.795913306673
760.265685530944 474.080233689919
755.258950362071 480.34361294476
748.837457119675 488.828385747702
743.000198360243 494.10786015874
734.402704240787 498.74119471161
724.968503889824 500.214340146433
714.878233460949 498.632888761196
708.321633548166 496.629822690734
698.217062121911 495.784957119082
678.195026153215 499.661357996235
669.687996724522 505.150725900051
660.14332124808 510.750477051003
650.537853281586 518.960363419669
643.789867494156 530.756536692671
641.928441563995 543.524549811873
643.650921858714 551.013493894046
648.600086205805 558.035241598445
642.206190967743 553.750094330173
642.512605728365 553.786147675896
642.536018571617 553.814861579096
642.54602794319 553.754624508399
642.679566872228 553.552040720616
642.917042023115 553.5680788218
642.787759456086 553.235696675075
639.776125513165 550.69995525071
634.498516988672 549.262333360858
620.550893344899 549.412021736431
615.166527593851 553.807679557658
612.507952486239 559.707788870432
612.36920139971 562.216885182341
613.494512094848 565.982206310043
618.523968196621 578.630120773735
621.43930077719 586.327303705117
625.510972902638 597.012469992868
630.329676516406 609.647904792427
634.037242748612 619.669393814619
636.687837396335 627.206858372847
640.88264734553 639.889187083762
644.241836526307 650.106427796693
647.807344303893 659.475633454604
651.098328223618 666.832598965069
654.03918493736 673.934490871176
651.625187210245 672.283761233748
651.883636785328 672.880493821088
651.881535713272 672.877465191824
651.881535713272 672.877465191824
651.881535713272 672.877465191824
651.881535713272 672.877465191824
651.881535713272 672.877465191824
651.881535713272 672.877465191824
651.881535713272 672.877465191824
651.881535713272 672.877465191824
};
\addplot [rlPolicies, line width=\trajectoryWidth]
table {%
665 62.0000000000004
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000017
665 62.0000000000017
665 62.0000000000017
665 62.0000000000017
665 62.0000000000018
665 62.0000000000018
665 62.0000000000018
665 62.0000000000019
665 62.0000000000019
665 62.000000000002
665 62.000000000002
665 62.000000000002
665 62.0000000000021
665 62.0000000000021
665 62.0000000000021
665 62.0000000000022
665 62.0000000000022
665 62.0000000000022
665 62.0000000000023
665 62.0000000000023
665 62.0000000000023
665 62.0000000000024
664.999999249608 61.9978714397834
664.999951287478 61.9637919658749
664.872644185952 64.1534161385465
663.864355047417 69.8275358614507
660.2714422068 80.7180366603174
657.317177349974 96.7202450260787
659.982547337038 116.194037365853
661.168705720438 128.042010757978
663.741055883611 144.892364135288
664.258156631483 157.171452560856
664.983237292915 169.089687199706
665.33830873429 184.989596338061
665.049478845416 194.780588715768
667.881922751102 199.992040467169
672.724013970127 208.445462537629
682.550575024769 220.791247957093
693.159028065834 227.601540767145
706.314014717567 236.077833667106
717.977321929255 241.490918619306
732.715620680551 248.140030913474
742.056555170211 252.752317088146
753.079572822589 259.727781721092
761.416134329409 266.632253085468
767.804321322643 273.581319460957
774.276778227234 284.431155765622
779.342016944043 295.075567005989
782.832182914623 304.509404728626
784.82766703455 313.507126352567
787.412189497199 326.818954195732
790.291633905777 342.767637500076
791.788484632818 356.318773060223
792.689027280958 369.663541605478
793.040985481334 387.299312618929
792.860951206574 399.731373978673
791.804223658915 416.018924504608
788.13826395817 428.432081532362
782.626604360372 436.328105803097
779.826898475322 445.66779668645
774.502065770455 457.562023709631
765.309350958826 467.871067852998
755.043309760359 479.965075381925
746.69028726786 490.27602941685
738.077360666684 496.246527809243
728.135370186478 499.237539775263
719.697005740936 499.897639658731
706.32370419736 496.207297354874
693.047766068257 496.168521893515
683.161730448618 499.072177262564
670.196770116333 505.319533885149
659.017210505427 512.079494512601
646.865002302019 525.462940328213
642.800927752412 538.105297015346
642.841298539927 547.743523278402
647.873168343579 555.804916892607
650.021596182756 557.363998548229
650.412408487751 557.483185604529
650.606534292343 557.476007155876
650.743131219938 557.411745357538
650.696895492279 557.281023114209
650.725461035466 557.030271697055
650.416261520702 556.640903387053
647.731529430203 553.721400335199
642.001920517909 550.833169470429
632.226121792115 547.071491520373
621.359273579645 550.75193503853
613.123597145694 555.674121824695
611.711418751371 563.606131060636
610.388766453727 558.001923218365
614.353231953979 567.344087386679
619.368306678523 579.466787052997
624.260507500489 591.508986657543
628.216632038844 602.101526960511
632.600109440055 614.883269516684
637.500133322662 630.142580631237
643.011241584721 648.076467278803
647.527950749586 660.607805019123
652.003883177466 671.191538287063
651.588616607866 672.671128266308
651.897671231297 673.43145621954
651.894664272573 673.424205389122
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
651.894522949191 673.423823878167
};
\addplot [rlPolicies, line width=\trajectoryWidth]
table {%
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665.000000090635 61.9999378139933
664.999433461327 62.0648971573391
664.999225237309 62.0874921823957
664.999216941639 62.0883766525002
664.999216941639 62.0883766525002
664.999216941639 62.0883766525002
664.958938714402 62.8773358688841
664.577673179984 65.6031784009643
661.305861499638 74.8536142474648
657.370821376631 86.9898482253333
656.134438159366 108.540413084361
658.309798153799 119.620385663843
660.65815705214 136.122340904126
662.206991633839 144.285526126273
664.124188211492 157.345372677969
664.848985833018 166.016397608136
665.997126649846 181.820781050314
666.098778302841 193.975044994576
666.164494855364 200.564786715037
670.494162969157 206.931873365272
675.610250338101 214.903765232998
682.272754599067 223.503557008954
688.962677105339 228.286911693633
698.066650743438 233.783842253626
705.966366079529 239.1229266882
713.369437889378 242.708868874507
722.78640241554 247.00675987065
734.355230653307 252.559630956623
743.609065618774 257.271004014739
750.013183913758 261.30504658769
758.379343801289 267.580094686275
764.109033262636 273.132165915486
771.338153887752 282.044602233543
776.147106763521 291.695190499234
779.085754033357 299.167932903704
783.265536081908 310.620381176049
785.304659401131 320.029433428859
788.197882757151 335.901095886939
789.691771939116 346.691144428168
791.824952893053 362.220384720828
792.521715243975 372.889359273661
793.144428066405 385.532762686162
793.278698205603 396.225303762499
793.186058314601 406.806179250991
791.98364803884 422.466699483474
787.364278574785 434.497729300756
780.948360904062 442.346153539201
773.778481998392 453.026064164177
766.958823001584 466.485209988022
759.835244915952 474.460158418556
749.189719493107 486.388465564293
744.024125103208 492.49149669572
728.743473264306 501.955672816762
715.944265387355 503.424132881844
701.475788184711 499.865528062723
686.663291356116 499.466354970676
671.534198198106 504.651386931804
659.471220184803 514.376167282012
651.761705873581 518.839167743264
642.674087829908 530.604799196293
638.725938767245 549.055819855445
640.832092011483 557.86738578743
645.360919979211 563.75674714598
645.944287166022 564.073471123728
640.210972870181 560.035059825341
640.342867833151 559.990791213928
640.729127187254 559.536306225925
640.810693188121 559.405960121067
640.795175802586 559.589032739991
640.667511883522 559.268578579959
639.739284449935 557.937772814503
632.921030514212 552.918699450931
627.470836752189 551.935701908695
619.413884882288 551.539489288602
614.707881915941 556.375624345024
613.515500983407 554.185356510221
613.761771167649 556.175468106536
617.638958292823 565.312250756442
620.167304736334 574.936029842222
624.396123862988 590.680777430483
628.00961861601 603.690677567308
631.892962197185 616.535041713588
635.773519259281 629.192184296381
638.958399138094 639.466318405074
642.120957627488 649.447757378548
645.641764513242 659.701266913478
650.718113101834 671.531966300876
654.001493349883 678.757933893722
654.464437472233 679.693262489517
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593463 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
651.136609593464 671.863700625384
};

==> figures/experiments/rl_policies_right_data.tex <==
\addplot [rlPolicies, line width=\trajectoryWidth]
table {%
665 62.0000000000002
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
664.999973240563 62.0033175262721
664.993366658965 62.4978632192845
664.883484897144 65.0732317622399
664.274351381864 70.4738570687661
659.867986860508 94.6953058574928
659.185066800854 106.86562766522
661.999680792513 124.807847326866
664.218929232334 139.437499596544
664.737200883223 155.534388627594
665.323554183513 166.807162844761
665.883720455592 184.36064089775
665.323040118696 195.460421046289
663.640456852357 202.457931065476
655.856396645959 213.396747057464
641.52313952976 220.267550105762
628.69058612407 225.138828490025
615.27085426449 228.206121151394
602.709544832832 232.494251727001
590.471937885724 238.031964840658
579.562527765313 244.159585028798
564.390645305928 254.862864251814
556.799381081651 261.764711003249
550.091577462798 269.78196825459
544.471309515827 283.450102535112
543.639066438433 292.791439231733
540.59427175077 303.679413685968
535.783361811478 310.628965110182
532.240466207944 321.147374643731
530.978938648017 326.454132627822
529.226285040586 334.235524190598
527.4611022307 341.743829637753
525.351017198216 351.854956559178
523.630360977606 362.624400542535
522.554379464427 370.351124799313
521.322045895713 380.614361947688
519.790497822434 394.03952367962
518.730093994231 401.958148559991
517.597255473606 410.228908630736
518.052903733288 417.574454554259
520.298630413232 426.091672964748
521.881309136238 439.329112041432
521.572311862441 449.232521533554
519.153826031156 468.111872691405
518.06772364865 475.538476840815
519.897485225096 489.143529737933
524.250890264376 497.065791537638
532.926909193955 506.458167220334
542.639063557854 509.881606077288
554.922907248585 509.850156319221
566.031683130455 509.266486161576
574.299352381581 509.855088611565
579.9698883259 512.215470998978
588.302306529864 517.452742383825
594.232170910278 521.925929142003
599.933700541227 529.556397370706
605.777773852038 537.635735044283
613.92994540776 549.184292821165
618.196613588079 556.403033463338
622.963137476955 565.888734479073
625.021491340508 577.182781931005
624.33056596862 587.360949199613
624.139386059827 601.416757905608
625.580276096455 612.146103450721
630.509888026568 629.820746889977
633.176417899346 637.213224618273
636.054124148355 644.76523816641
639.840190209592 654.335691112509
646.55137883108 669.622936504166
650.790301612446 678.431975792711
653.933877012035 685.388353547641
651.546943887769 679.496343848736
651.543452023035 679.488859552442
651.54011834373 679.484728510466
651.54011834373 679.484728510466
651.54011834373 679.484728510466
651.54011834373 679.484728510466
651.54011834373 679.484728510466
};
\addplot [rlPolicies, line width=\trajectoryWidth]
table {%
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
664.999755328933 62.0100588131789
664.990999038144 62.3259550630084
664.398869594933 68.3321807963064
662.364870001403 76.3596421510318
657.92593750728 100.531196482111
657.646700034481 111.189596113246
658.959976127716 120.380335411796
661.123081125645 134.400120195789
663.139777697602 145.599506364887
663.894313975219 155.765625909316
664.40014389416 164.282532413471
665.30434040644 180.790392104305
665.920116634865 192.621142567543
665.512741966571 198.345357650257
663.925240637813 203.819833973585
658.949930269099 211.780780044986
648.152415731122 219.649855398789
639.365101132094 226.723397013533
624.438703885631 228.403322843959
611.582347872582 231.335328997528
603.425137511845 234.040499778537
589.433705063197 240.052166897648
578.32575993378 246.231909014339
564.858862270025 255.655311366627
557.152564337189 262.381301074506
550.007186023916 270.86971286482
545.761742088014 280.007226112435
544.006911845492 290.492907465465
540.266607872904 302.443796442432
536.949786417285 309.317794976405
533.064979926153 319.401318041458
529.531245560277 334.733436142139
527.778314217229 342.498457939005
524.571236925342 354.613286392704
522.792462049015 365.54922461842
521.23156819668 378.069803540386
520.295554285978 387.008891445065
519.164379208684 397.687311994662
518.049407457085 406.916997441802
518.146295676744 413.416415161621
520.683407865931 424.042754967262
522.10092945952 434.383643222039
521.962917706842 447.630513837957
520.698696437767 458.073874206686
518.707963076055 471.097402692141
518.079474600765 480.61091543703
519.47146332617 488.840562755213
524.655926510494 498.925241470435
531.528588871712 505.757934004969
543.503383430759 510.975535642168
551.003110782386 513.367967670603
562.159654204858 512.565191685144
571.217605034881 512.438319810029
577.477644073069 513.100772377956
588.498229056874 517.285324835969
594.466616184085 522.174392211967
601.03702329498 530.888140677137
609.28201431776 540.243680502527
616.13772257926 551.040020158112
622.574661633458 562.512006317128
626.484585155281 571.131004759511
625.650279079545 574.147918184304
624.531530187736 586.556282876264
625.305320718384 599.528999562938
626.380721846916 612.401150490637
628.466420572989 622.586230964087
631.818084614066 633.428172620903
636.530723841132 645.848233184408
640.638536816381 655.668282380801
648.732755465821 672.090465781553
652.980973837316 680.410705681264
653.718176427155 681.754301950456
653.697569502386 681.717013370602
653.698753977285 681.719203491946
653.698753977285 681.719203491946
653.698753977285 681.719203491946
653.698753977285 681.719203491946
653.698753977285 681.719203491946
653.698753977285 681.719203491946
653.698753977285 681.719203491946
653.698753977285 681.719203491946
653.698753977285 681.719203491946
};
\addplot [rlPolicies, line width=\trajectoryWidth]
table {%
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665.000092433801 61.9774759172706
664.985702647568 62.5447802881373
664.838216131225 64.8958077348719
663.128206839186 72.8763810271497
659.951586505655 82.3706213909448
656.566330283843 108.086932366507
657.819756504485 125.295327610029
662.002196986297 142.236580988837
664.268938721186 159.223093493687
665.045340329556 170.637962383958
666.150307533981 186.369486482223
666.097198022407 193.973398011455
665.706980520624 198.813456170775
664.063383639093 205.697584507581
659.17471110378 213.886825855074
643.603852288637 228.153995030845
633.343091121 229.267824454499
625.111987817291 229.93603964994
611.640174097899 235.613698319456
601.372060920144 238.783620619206
590.371761114539 243.057261703311
578.047220486013 249.331781356412
567.057540210269 256.284230986161
554.589639099611 266.644659161775
546.531359161068 277.268649951347
542.880693577439 289.67891514365
540.227481409225 299.441172119798
536.537168781355 309.235311121714
532.701224345939 321.490755856748
529.58875590064 333.925018455144
527.682853949455 342.251074400498
524.600799031904 357.941095188126
522.794660718413 370.94107278442
520.919185827367 386.961323917386
519.492725309078 399.449190714782
518.343394018473 407.398082939237
518.07020689173 414.837203514766
519.502318348228 422.951909070256
521.189468344274 433.260752021405
521.603227350766 445.97123788868
520.205940906302 459.329018457071
518.559276712989 471.945941257259
519.723548405284 482.396125572112
523.685233606639 491.158083473907
528.582171451699 497.053866337369
536.309325886096 503.518195950593
544.043205742135 505.126292496854
552.777525895331 504.891361338922
558.408029316659 507.22596319325
568.441628193089 507.755830351708
575.604222756626 509.191931261189
581.319666553919 511.464017231148
587.895539534951 515.984147638081
593.560832473797 522.338665270652
600.751401366313 531.896180430897
605.459639444219 538.513589164316
612.792535199829 549.722045600318
620.607186064506 563.517314102975
623.795728960701 571.052551834522
625.144218367127 575.061873768833
624.155825239719 579.872421253775
623.509015662781 592.090535456836
623.700711498296 600.783626366162
625.726353425919 614.373857223215
627.643722789842 621.823901962738
632.06442364874 634.884022919742
637.649036158042 649.215688424736
640.857401253627 657.257470768993
648.10986596018 671.739344163813
651.141384301997 678.704547227981
653.045570921348 682.147661685578
653.154026040597 682.348970693768
649.027913483458 673.692730550001
649.028238093758 673.693330453898
649.028238093758 673.693330453898
649.028238093758 673.693330453898
649.028238093758 673.693330453898
649.028238093758 673.693330453898
649.028238093758 673.693330453898
649.028238093758 673.693330453898
649.028238093758 673.693330453898
649.028238093758 673.693330453898
};
\addplot [rlPolicies, line width=\trajectoryWidth]
table {%
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665.000002907242 61.9986866764615
664.998007510506 62.1668058671705
664.929511319444 63.609177511408
663.460719977132 72.1417614973086
660.158739363132 86.6644062123263
657.358771244464 100.326340229655
657.152705653416 109.184661098824
659.434170108755 125.247832895472
663.018892853013 142.992597871918
664.353978264964 154.447837749363
665.376531562515 171.612092719576
666.128139759598 184.311914808589
665.428688261624 199.246685242954
665.064485728915 201.844628671239
659.995250458125 212.026932388204
652.599055430329 218.795731360384
639.870339751034 223.114915538372
631.503307613571 227.252737288649
615.871429547041 229.860673044841
605.301962645554 233.103641669814
593.331843212508 238.041876632447
585.987773351209 241.685342964412
574.810088400433 248.266956392059
566.249074626546 254.381348763198
555.868725016209 263.550729704978
550.690228226344 269.745489911213
545.926751587012 279.088473053356
543.83495367925 291.654128562097
541.529430655298 301.605214733395
534.546412593655 311.9042578938
530.904848188022 324.694242678783
527.688459479859 339.995677048368
526.031889514847 347.749605345164
523.790004462328 360.158567967058
522.124252868713 372.014234625308
520.934813294922 382.627210448026
519.707147415263 394.609768130593
518.570064266547 403.881055633262
518.18829045346 411.636445364469
519.58946126647 419.704358776551
521.305684009784 429.313272654646
521.921881975289 436.915647748767
521.771160619256 444.686580980771
520.45075220207 457.258591195705
519.259687796539 465.660161602416
517.581437897687 476.497770011119
514.712304401343 488.890730817635
514.295661010492 492.813332939122
516.222040389002 491.83231071799
518.808585033367 498.176696830387
527.922748361498 507.663140133906
536.315372989773 511.618126603838
546.903025268186 512.836360860418
557.215712553156 513.042505036334
568.215749547253 511.928578435072
579.966512070217 514.59059283031
588.533741693794 518.949919667649
593.87774012281 523.922468464225
598.163072730573 529.403106063125
606.779621118387 541.573702801882
611.243968691656 548.264181718248
615.373911603748 554.989665568869
618.998735826806 564.930620197058
620.722315571494 580.887972722653
621.683057596024 591.237201487438
622.636042273246 598.867507491271
625.28617330185 612.272188668685
628.307898413246 622.901794749745
630.762662360403 630.265055276773
634.272250525414 640.096491142107
638.028154106325 649.959033833127
641.490618316515 657.783987128407
646.28002247375 667.018517831139
652.855821090121 679.956550394532
650.297257090564 674.750839953186
649.546632657416 673.220797086716
649.547080746463 673.221728537535
649.547080746463 673.221728537535
649.547080746463 673.221728537535
649.547080746463 673.221728537535
649.547080746463 673.221728537535
649.547080746463 673.221728537535
649.547080746463 673.221728537535
};

==> figures/experiments/rl_policies_right_data_obstacles.tex <==
\addplot [rlPolicies, line width=\trajectoryWidth]
table {%
665 62.0000000000002
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
664.999973240563 62.0033175262721
664.993366658965 62.4978632192845
664.883484897144 65.0732317622399
664.274351381864 70.4738570687661
659.867986860508 94.6953058574928
659.185066800854 106.86562766522
661.999680792513 124.807847326866
664.218929232334 139.437499596544
664.737200883223 155.534388627594
665.323554183513 166.807162844761
665.883720455592 184.36064089775
665.323040118696 195.460421046289
663.640456852357 202.457931065476
655.856396645959 213.396747057464
641.52313952976 220.267550105762
628.69058612407 225.138828490025
615.27085426449 228.206121151394
602.709544832832 232.494251727001
590.471937885724 238.031964840658
579.562527765313 244.159585028798
564.390645305928 254.862864251814
556.799381081651 261.764711003249
550.091577462798 269.78196825459
544.471309515827 283.450102535112
543.639066438433 292.791439231733
540.59427175077 303.679413685968
% 535.783361811478 310.628965110182
% 532.240466207944 321.147374643731
% 530.978938648017 326.454132627822
% 529.226285040586 334.235524190598
% 527.4611022307 341.743829637753
% 525.351017198216 351.854956559178
% 523.630360977606 362.624400542535
% 522.554379464427 370.351124799313
% 521.322045895713 380.614361947688
% 519.790497822434 394.03952367962
% 518.730093994231 401.958148559991
% 517.597255473606 410.228908630736
% 518.052903733288 417.574454554259
% 520.298630413232 426.091672964748
% 521.881309136238 439.329112041432
% 521.572311862441 449.232521533554
% 519.153826031156 468.111872691405
% 518.06772364865 475.538476840815
% 519.897485225096 489.143529737933
% 524.250890264376 497.065791537638
% 532.926909193955 506.458167220334
% 542.639063557854 509.881606077288
% 554.922907248585 509.850156319221
% 566.031683130455 509.266486161576
% 574.299352381581 509.855088611565
% 579.9698883259 512.215470998978
% 588.302306529864 517.452742383825
% 594.232170910278 521.925929142003
% 599.933700541227 529.556397370706
% 605.777773852038 537.635735044283
% 613.92994540776 549.184292821165
% 618.196613588079 556.403033463338
% 622.963137476955 565.888734479073
% 625.021491340508 577.182781931005
% 624.33056596862 587.360949199613
% 624.139386059827 601.416757905608
% 625.580276096455 612.146103450721
% 630.509888026568 629.820746889977
% 633.176417899346 637.213224618273
% 636.054124148355 644.76523816641
% 639.840190209592 654.335691112509
% 646.55137883108 669.622936504166
% 650.790301612446 678.431975792711
% 653.933877012035 685.388353547641
% 651.546943887769 679.496343848736
% 651.543452023035 679.488859552442
% 651.54011834373 679.484728510466
% 651.54011834373 679.484728510466
% 651.54011834373 679.484728510466
% 651.54011834373 679.484728510466
% 651.54011834373 679.484728510466
};
\addplot [rlPolicies, line width=\trajectoryWidth]
table {%
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
665 62.0000000000001
664.999755328933 62.0100588131789
664.990999038144 62.3259550630084
664.398869594933 68.3321807963064
662.364870001403 76.3596421510318
657.92593750728 100.531196482111
657.646700034481 111.189596113246
658.959976127716 120.380335411796
661.123081125645 134.400120195789
663.139777697602 145.599506364887
663.894313975219 155.765625909316
664.40014389416 164.282532413471
665.30434040644 180.790392104305
665.920116634865 192.621142567543
665.512741966571 198.345357650257
663.925240637813 203.819833973585
658.949930269099 211.780780044986
648.152415731122 219.649855398789
639.365101132094 226.723397013533
624.438703885631 228.403322843959
611.582347872582 231.335328997528
603.425137511845 234.040499778537
589.433705063197 240.052166897648
578.32575993378 246.231909014339
564.858862270025 255.655311366627
557.152564337189 262.381301074506
550.007186023916 270.86971286482
545.761742088014 280.007226112435
544.006911845492 290.492907465465
540.266607872904 302.443796442432
% 536.949786417285 309.317794976405
% 533.064979926153 319.401318041458
% 529.531245560277 334.733436142139
% 527.778314217229 342.498457939005
% 524.571236925342 354.613286392704
% 522.792462049015 365.54922461842
% 521.23156819668 378.069803540386
% 520.295554285978 387.008891445065
% 519.164379208684 397.687311994662
% 518.049407457085 406.916997441802
% 518.146295676744 413.416415161621
% 520.683407865931 424.042754967262
% 522.10092945952 434.383643222039
% 521.962917706842 447.630513837957
% 520.698696437767 458.073874206686
% 518.707963076055 471.097402692141
% 518.079474600765 480.61091543703
% 519.47146332617 488.840562755213
% 524.655926510494 498.925241470435
% 531.528588871712 505.757934004969
% 543.503383430759 510.975535642168
% 551.003110782386 513.367967670603
% 562.159654204858 512.565191685144
% 571.217605034881 512.438319810029
% 577.477644073069 513.100772377956
% 588.498229056874 517.285324835969
% 594.466616184085 522.174392211967
% 601.03702329498 530.888140677137
% 609.28201431776 540.243680502527
% 616.13772257926 551.040020158112
% 622.574661633458 562.512006317128
% 626.484585155281 571.131004759511
% 625.650279079545 574.147918184304
% 624.531530187736 586.556282876264
% 625.305320718384 599.528999562938
% 626.380721846916 612.401150490637
% 628.466420572989 622.586230964087
% 631.818084614066 633.428172620903
% 636.530723841132 645.848233184408
% 640.638536816381 655.668282380801
% 648.732755465821 672.090465781553
% 652.980973837316 680.410705681264
% 653.718176427155 681.754301950456
% 653.697569502386 681.717013370602
% 653.698753977285 681.719203491946
% 653.698753977285 681.719203491946
% 653.698753977285 681.719203491946
% 653.698753977285 681.719203491946
% 653.698753977285 681.719203491946
% 653.698753977285 681.719203491946
% 653.698753977285 681.719203491946
% 653.698753977285 681.719203491946
% 653.698753977285 681.719203491946
};
\addplot [rlPolicies, line width=\trajectoryWidth]
table {%
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665 62.0000000000002
665.000092433801 61.9774759172706
664.985702647568 62.5447802881373
664.838216131225 64.8958077348719
663.128206839186 72.8763810271497
659.951586505655 82.3706213909448
656.566330283843 108.086932366507
657.819756504485 125.295327610029
662.002196986297 142.236580988837
664.268938721186 159.223093493687
665.045340329556 170.637962383958
666.150307533981 186.369486482223
666.097198022407 193.973398011455
665.706980520624 198.813456170775
664.063383639093 205.697584507581
659.17471110378 213.886825855074
643.603852288637 228.153995030845
633.343091121 229.267824454499
625.111987817291 229.93603964994
611.640174097899 235.613698319456
601.372060920144 238.783620619206
590.371761114539 243.057261703311
578.047220486013 249.331781356412
567.057540210269 256.284230986161
554.589639099611 266.644659161775
546.531359161068 277.268649951347
542.880693577439 289.67891514365
540.227481409225 299.441172119798
% 536.537168781355 309.235311121714
% 532.701224345939 321.490755856748
% 529.58875590064 333.925018455144
% 527.682853949455 342.251074400498
% 524.600799031904 357.941095188126
% 522.794660718413 370.94107278442
% 520.919185827367 386.961323917386
% 519.492725309078 399.449190714782
% 518.343394018473 407.398082939237
% 518.07020689173 414.837203514766
% 519.502318348228 422.951909070256
% 521.189468344274 433.260752021405
% 521.603227350766 445.97123788868
% 520.205940906302 459.329018457071
% 518.559276712989 471.945941257259
% 519.723548405284 482.396125572112
% 523.685233606639 491.158083473907
% 528.582171451699 497.053866337369
% 536.309325886096 503.518195950593
% 544.043205742135 505.126292496854
% 552.777525895331 504.891361338922
% 558.408029316659 507.22596319325
% 568.441628193089 507.755830351708
% 575.604222756626 509.191931261189
% 581.319666553919 511.464017231148
% 587.895539534951 515.984147638081
% 593.560832473797 522.338665270652
% 600.751401366313 531.896180430897
% 605.459639444219 538.513589164316
% 612.792535199829 549.722045600318
% 620.607186064506 563.517314102975
% 623.795728960701 571.052551834522
% 625.144218367127 575.061873768833
% 624.155825239719 579.872421253775
% 623.509015662781 592.090535456836
% 623.700711498296 600.783626366162
% 625.726353425919 614.373857223215
% 627.643722789842 621.823901962738
% 632.06442364874 634.884022919742
% 637.649036158042 649.215688424736
% 640.857401253627 657.257470768993
% 648.10986596018 671.739344163813
% 651.141384301997 678.704547227981
% 653.045570921348 682.147661685578
% 653.154026040597 682.348970693768
% 649.027913483458 673.692730550001
% 649.028238093758 673.693330453898
% 649.028238093758 673.693330453898
% 649.028238093758 673.693330453898
% 649.028238093758 673.693330453898
% 649.028238093758 673.693330453898
% 649.028238093758 673.693330453898
% 649.028238093758 673.693330453898
% 649.028238093758 673.693330453898
% 649.028238093758 673.693330453898
};
\addplot [rlPolicies, line width=\trajectoryWidth]
table {%
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665.000002907242 61.9986866764615
664.998007510506 62.1668058671705
664.929511319444 63.609177511408
663.460719977132 72.1417614973086
660.158739363132 86.6644062123263
657.358771244464 100.326340229655
657.152705653416 109.184661098824
659.434170108755 125.247832895472
663.018892853013 142.992597871918
664.353978264964 154.447837749363
665.376531562515 171.612092719576
666.128139759598 184.311914808589
665.428688261624 199.246685242954
665.064485728915 201.844628671239
659.995250458125 212.026932388204
652.599055430329 218.795731360384
639.870339751034 223.114915538372
631.503307613571 227.252737288649
615.871429547041 229.860673044841
605.301962645554 233.103641669814
593.331843212508 238.041876632447
585.987773351209 241.685342964412
574.810088400433 248.266956392059
566.249074626546 254.381348763198
555.868725016209 263.550729704978
550.690228226344 269.745489911213
545.926751587012 279.088473053356
543.83495367925 291.654128562097
541.529430655298 301.605214733395
% 534.546412593655 311.9042578938
% 530.904848188022 324.694242678783
% 527.688459479859 339.995677048368
% 526.031889514847 347.749605345164
% 523.790004462328 360.158567967058
% 522.124252868713 372.014234625308
% 520.934813294922 382.627210448026
% 519.707147415263 394.609768130593
% 518.570064266547 403.881055633262
% 518.18829045346 411.636445364469
% 519.58946126647 419.704358776551
% 521.305684009784 429.313272654646
% 521.921881975289 436.915647748767
% 521.771160619256 444.686580980771
% 520.45075220207 457.258591195705
% 519.259687796539 465.660161602416
% 517.581437897687 476.497770011119
% 514.712304401343 488.890730817635
% 514.295661010492 492.813332939122
% 516.222040389002 491.83231071799
% 518.808585033367 498.176696830387
% 527.922748361498 507.663140133906
% 536.315372989773 511.618126603838
% 546.903025268186 512.836360860418
% 557.215712553156 513.042505036334
% 568.215749547253 511.928578435072
% 579.966512070217 514.59059283031
% 588.533741693794 518.949919667649
% 593.87774012281 523.922468464225
% 598.163072730573 529.403106063125
% 606.779621118387 541.573702801882
% 611.243968691656 548.264181718248
% 615.373911603748 554.989665568869
% 618.998735826806 564.930620197058
% 620.722315571494 580.887972722653
% 621.683057596024 591.237201487438
% 622.636042273246 598.867507491271
% 625.28617330185 612.272188668685
% 628.307898413246 622.901794749745
% 630.762662360403 630.265055276773
% 634.272250525414 640.096491142107
% 638.028154106325 649.959033833127
% 641.490618316515 657.783987128407
% 646.28002247375 667.018517831139
% 652.855821090121 679.956550394532
% 650.297257090564 674.750839953186
% 649.546632657416 673.220797086716
% 649.547080746463 673.221728537535
% 649.547080746463 673.221728537535
% 649.547080746463 673.221728537535
% 649.547080746463 673.221728537535
% 649.547080746463 673.221728537535
% 649.547080746463 673.221728537535
% 649.547080746463 673.221728537535
};

==> figures/experiments/teleop_left_data.tex <==
\addplot [teleOp, line with=\trajectoryWidth]
table {%
665 62.0000000000002
665.000633303182 62.4216569361909
665.012474090377 65.1789860413153
665.080049498834 70.2123852177667
665.048240021357 79.0354686263167
664.828172874832 88.2058558994261
664.523373102479 98.0046687223034
664.297141454401 107.360939235283
664.630478792657 117.114922213396
666.331962434312 132.004653312357
668.788473013415 143.898496245367
671.487055078684 153.200715668246
681.774281584788 184.036052232054
684.522412831957 192.408961544921
688.015442782824 201.661208532127
690.150679199758 207.123151418722
689.350889912947 205.135118633193
689.75292082149 205.901239321082
695.452602671481 214.94943665459
698.42207183988 218.365558337744
704.177936717371 223.953213317661
712.772339163192 231.459934793456
720.06400536244 236.273727058328
728.850218672208 241.682990137374
736.982834700034 246.354722946355
744.322315385562 250.675765997997
754.768214411528 256.0192081341
763.623441167513 260.231744456472
772.060084473811 264.038256077976
780.895251203962 267.850744145924
789.21523666522 271.203358666269
797.234173723584 274.786300385897
803.848553629069 279.240703082483
806.121350926535 281.890375217461
806.823094960176 282.596824451166
804.810188499541 280.223072568495
808.269256327912 285.753758973739
812.995134000265 293.674836392433
816.711376185045 303.053754036545
820.566024016992 312.597099854673
823.569801726703 322.377823451211
826.69883651401 334.673794283631
828.709535493898 344.056953854486
831.591372066736 357.163403391188
833.619354716245 370.648186836133
834.923951212701 381.289847363265
836.284894950346 395.799303523118
836.96231059896 406.952177695834
836.857652171806 420.80273337602
836.249149458881 429.824847294108
834.469695338315 439.756597741918
831.519591552732 448.707436112809
829.375863962983 454.880844334309
831.69081796166 448.342118925278
829.550149229532 452.224997254394
823.717593029245 460.765695004667
814.929396472684 467.930160562104
807.108671463995 472.759754179612
799.400705773976 474.569199337292
787.079712070859 476.602125543188
776.607061025052 477.935720352655
763.224284999784 480.830327736337
756.596040201938 482.972397035306
748.18352570816 486.729782066279
738.819655340216 492.401881412825
732.160947974425 496.802868378675
726.579899226781 500.668032570388
726.068260581917 500.712033274519
725.302571753986 501.427512183665
722.023794058496 507.637534277253
718.200556340799 519.804838451144
715.288430627327 533.383414372837
713.625635765842 545.681736409701
712.985837626964 556.953731154229
713.070539080788 568.627422710089
714.296568572428 580.271348332121
716.141101745592 593.365741971576
717.791644015534 603.743185826243
719.194414284058 618.071720606783
719.372394913626 626.885866900434
718.662953213067 642.596330509502
717.302198863762 654.659539359357
716.461369323454 661.726784852795
715.487727337254 669.646054046799
715.134471850349 672.723293430423
715.76576856307 666.877969005606
715.765699003787 666.878572692136
715.765699003787 666.878572692136
715.765699003787 666.878572692136
715.765699003787 666.878572692136
715.765699003787 666.878572692136
715.765699003787 666.878572692136
};
\addplot [teleOp, line with=\trajectoryWidth]
table {%
665 62
665 62
665 62
665 62
665 62
665 61.9999999999999
665 61.9999999999999
665 61.9999999999999
665 61.9999999999999
665 61.9999999999999
665 61.9999999999999
665 61.9999999999999
665 61.9999999999999
665 61.9999999999999
665 61.9999999999999
665 61.9999999999999
665 61.9999999999999
665.000001948736 62.0004619267013
664.999343143625 62.4337250743992
664.965357195262 68.4440151809335
664.952433579478 83.9117752084097
664.958254692464 95.367553995454
664.81969754573 112.857555563607
664.731538324083 125.791792222902
664.651598532799 139.270039574708
664.619571998106 152.072911573592
664.737679393645 164.194374896406
673.596573705943 201.729304504309
681.147391428184 211.686218760772
690.2667780172 219.881884170549
697.366209790979 227.285630452045
709.541510128182 236.560162828499
717.312113928806 242.53130235593
728.521166836356 250.38360467405
737.13835223463 256.076929474988
750.403906048525 264.651529436312
759.023581148258 270.365870739449
770.937944145616 280.007436142885
777.112669925965 287.540414249001
783.093064446526 304.509211256828
785.003798051774 313.319245249884
784.299560518388 326.516480823052
784.241269368871 344.99090585188
783.954293699076 356.252134011701
783.586379778518 373.500153657172
784.138232951076 384.426652101784
786.496983822103 398.450319214463
789.285903036561 412.098713481341
792.396308954295 428.281821359852
792.80384493381 439.65170105633
787.803010661406 454.776583560685
780.513411410111 464.618151799127
772.54612170231 472.0336456801
763.468589700257 477.351308976018
751.484819161329 481.329773868156
737.437832041006 483.471357666009
724.637008691921 484.39974936956
705.831558222159 485.285524230458
694.374268391158 485.263370816722
676.527498235504 490.125599090438
667.114229825514 497.961804734168
661.936816264478 508.799983370795
658.978986247244 521.515824287653
658.582101689181 535.291327479353
658.900330671886 551.496651549197
659.196501883869 564.89379852094
658.851820928458 578.210073125238
658.117975248688 597.809687499833
657.285152094514 609.05015728233
653.246127665828 627.700616163114
648.983113581047 639.507642661442
644.196834040996 655.090875627877
640.654451713642 667.670513003647
638.126610219896 676.11662726587
640.177275798188 668.697721968746
640.173470148447 668.710143341999
640.173470148447 668.710143341999
640.173470148447 668.710143341999
640.173470148447 668.710143341999
640.173470148447 668.710143341999
640.173470148447 668.710143341999
640.173470148447 668.710143341999
640.173470148447 668.710143341999
640.173470148447 668.710143341999
};
\addplot [teleOp, line with=\trajectoryWidth]
table {%
665 62.0000000000005
665 62.0000000000006
665 62.0000000000006
665 62.0000000000007
665 62.0000000000007
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000009
665 62.0000000000009
664.999994029533 62.0012962028723
664.993621173836 62.5623083238208
664.910119206045 68.228051060158
664.732958932064 82.7522890909292
664.575244825263 98.7151694978964
664.300735149433 121.132069118889
663.782304725549 145.83307006056
663.756859876043 159.581997506359
670.073353150928 207.098212096905
678.24237129054 220.110591068392
689.37897074466 228.24617395291
711.497042667933 239.316305303423
727.177195550467 246.927549085356
747.100336651932 259.271193733542
759.335176677363 271.286214286441
769.219659064191 288.137890797961
774.436921982313 304.597430168164
778.859897575654 326.208826336308
780.354198091153 344.981004278159
781.379008714812 363.939930684085
782.221308076887 386.048706341477
782.531476640275 406.501813901072
782.481378303256 429.42096552485
777.226897321936 447.81044170208
763.895516678692 454.330235220992
742.513192964392 458.927275428857
722.479411174446 462.423234198313
697.832965322996 465.725039816837
675.607636935946 469.852405014036
661.613281390733 480.804064279961
648.857723389238 498.108190437385
637.580861625043 524.345691353199
631.940174376646 547.42048301196
627.767637480472 573.45709922452
624.987485284943 594.51213449547
621.009240567799 611.004243720453
609.283838167181 637.442238723507
602.312728064269 652.484027591613
596.465437318472 670.248371647134
592.912224817814 681.025841654585
592.561857900013 682.096879152529
592.569894240506 682.074471875919
592.570763572527 682.071817375128
592.570763572527 682.071817375128
592.570763572527 682.071817375128
592.570763572527 682.071817375128
592.570763572527 682.071817375128
592.570763572527 682.071817375128
592.570763572527 682.071817375128
592.570763572527 682.071817375128
};

==> figures/experiments/teleop_right_data.tex <==
\addplot [teleOp, line with=\trajectoryWidth]
table {%
665 62.0000000000002
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000005
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000006
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000007
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000008
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.0000000000009
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.000000000001
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000011
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000012
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000013
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000014
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000015
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
665 62.0000000000016
664.999999780785 62.0005624321707
664.999994353558 62.0038765100174
664.999986473774 62.005677672387
664.999938684949 62.0129983921827
664.999912452033 62.0171133164387
664.999781362145 62.0369659983152
664.999714637278 62.0512089277378
664.999357897173 62.1260745178437
664.998257539806 62.2606280793866
664.996394564522 62.4945166729286
664.994910561506 62.8244668668239
664.994755608463 63.2402326980722
664.994776906991 63.2588569717022
664.995582596267 63.7578124906554
664.995594701062 63.8054739330184
664.996178223714 64.3202966457263
664.996084451875 64.4562363064344
664.996538571118 64.9522445659634
664.996564409803 65.0123832307515
664.996362803581 65.1982324383036
664.995860855321 66.0356577989624
664.994967075942 66.940177593282
664.994005477355 67.7792374853744
664.993850415888 67.8580530972371
664.993782023811 67.8948071418455
664.992184100899 68.8196816398691
664.991977185567 68.8997931610423
664.988837317692 69.8235963398652
664.988258493314 69.9496068727071
664.984485445669 70.7752320893327
664.984003276877 70.8625806381457
664.983096799772 71.0381115589542
664.977272425251 71.9479618771491
664.975611940914 72.1777628919799
664.969072610807 72.9799613703463
664.968307349008 73.0748665616589
664.966035238204 73.3597506124252
664.958963356733 74.2364172824837
664.956326640684 74.5760247595107
664.949495630219 75.8155797318873
664.949550562785 76.6226445589755
664.950824429599 77.0746163862428
664.956637347754 78.3534523549342
664.962663674341 79.6070201157332
664.962836176992 79.6561361610441
664.965699588584 80.6678736586277
664.966299117007 80.9864497600339
664.966887866438 81.9704681476697
664.966356670572 82.3527820331744
664.9633559716 83.3083812932736
664.9612086813 83.7573511012832
664.952754799673 85.1988432148425
664.948016989067 86.6746538238229
664.950754550777 88.1873655734466
664.958063183671 89.7354530782264
665.199436528958 92.0835909779692
665.208803506754 92.1755342898159
665.215815207656 93.6667475405724
665.216172949613 93.7941344075547
665.220830696849 95.2587338375061
665.221604291787 95.394110844384
665.222071340496 95.4572049991034
665.238939613973 96.8932616258686
665.244265340182 97.1659326508268
665.281678685711 98.4230685210239
665.287232822616 98.5625834438357
665.30224816683 98.908828243235
665.375272618584 100.251389961362
665.401810958271 100.672491769372
665.491356382778 101.962526813783
665.529496341866 102.464447022333
665.633827479967 103.691564369502
665.688880826271 104.266018073652
665.813706977495 105.431494462893
665.888874310294 106.079983143818
666.108323973829 107.906718942411
666.395406946018 110.68025240469
666.597707710537 112.392021509372
666.614300548734 112.536189145501
666.820830570634 114.338668222531
666.829041432788 114.408965311577
667.018295856977 116.002075841373
667.03666270313 116.153594312327
667.054574084381 116.300960728781
667.261445682409 117.981718105862
667.289131259199 118.205411981008
667.468976313869 119.661592074979
667.487769009385 119.81442538392
667.524866496922 120.116999045002
667.716339297962 121.673632431815
667.764208596764 122.058258678673
667.931617226859 123.393340652141
667.951304011072 123.550090216024
668.009757986002 124.016200378482
668.189483698964 125.440509647424
668.259841508458 125.989571274622
668.439608012327 127.370577333935
668.520904767126 127.988737200067
668.787903591821 130.026050802871
668.946378781704 132.39763370515
669.223803496891 134.515716117512
669.512443274599 136.672658014118
669.775120032845 138.626846537469
669.807108491323 138.863372421808
670.038244376405 140.571788711761
670.062290118812 140.749094797033
670.106666407713 141.076215201909
670.353098945609 142.882514542474
670.410207822367 143.298660645679
670.622046681085 144.83746038164
670.646514334219 145.015103261272
670.716081642727 145.51940311268
670.940701212561 147.14110448726
671.02257826384 147.729352640489
671.328348265525 149.918741898661
671.526504792206 151.333558258879
671.631195710074 152.081968240728
671.927031268473 154.221353326226
672.177577765035 156.188142570618
672.184573150334 156.242721255845
672.476400988745 158.322510772387
672.761959099867 160.325735662678
672.770019042464 160.381582878171
673.022698847552 162.12560497755
673.046353039917 162.288399053416
673.066249743492 162.425373367403
673.327279628535 164.23903721056
674.276698462206 182.358045134309
674.266070285914 182.50929597246
674.26230429509 182.561229535737
674.114547038404 184.431684834147
673.970318659342 186.227986448779
673.966414276173 186.278763212592
673.850361837522 187.866210238025
673.839764450389 188.016142885567
673.830809893597 188.142822308836
673.708745973178 189.820364655878
673.693434156496 190.022572139473
673.568665499797 191.631916347707
673.546414962892 191.911853294826
673.419939211638 193.461413862728
673.389800791835 193.82072670963
673.546284684885 194.666707887298
673.594325002832 194.909188360691
673.501350670755 196.119971445413
673.490433026602 196.265900895069
673.454653462458 196.748097093848
673.365673561741 197.961917496489
673.326768156912 198.484177820648
673.201203742055 200.106208336393
673.07845296754 201.610651196121
672.974767994962 202.864005477376
672.965918538489 202.97066246838
672.962892436386 203.00711088182
672.860153549886 204.229506571151
672.852810809887 204.315063133833
672.754395354326 205.42766605242
672.742426049806 205.555951486894
672.644978559181 206.555991295079
672.628256540609 206.71876664811
672.536599953219 207.578960966007
672.516960797812 207.762101237392
672.596203033786 206.045663054651
672.605903917792 205.844719665466
672.634881934124 205.261986959905
672.5789843946 205.819741069253
672.560289036754 205.999210698792
672.513674285033 206.427277529366
672.502492830046 206.526671195855
672.475450410637 206.764298495882
672.464423465448 206.861465160448
672.443573656104 207.046021570441
672.432397077877 207.135911208373
672.413621929619 207.253126396525
672.37050966892 207.474356550481
672.368685686595 207.482926539182
672.288093454126 207.827004666145
672.279638814759 207.860034559494
672.157146649815 208.296427590934
672.143011396298 208.343182282887
672.120443061169 208.416486053525
672.09936794825 207.236658401942
672.08632790865 207.049011485634
671.809272871955 207.759412390434
671.73545478425 207.937278018182
671.440177766807 208.613031312602
671.403752806459 208.692389305885
671.295397339795 208.926510365627
670.912938298692 209.713470773402
670.761731568136 210.010930812655
670.161422474759 211.145294820284
669.738686178557 211.913960809892
669.504385169149 212.330817508285
668.792585148181 213.559380299616
668.050413985726 214.768926628999
668.02889084764 214.802973034558
667.224445460552 216.045668204402
666.399856208597 217.260086796802
666.375543465625 217.294898946891
665.541600535838 218.457482432203
665.479650470474 218.541557025326
663.905370175008 222.007750556229
663.860695363769 222.104791548354
662.928924635201 223.276904528513
662.859113746219 223.362507076681
661.81888736988 224.603524050788
661.788512614545 224.638845160444
660.727803517912 225.847828007168
660.648511048319 225.936023249417
659.674335842221 227.003545927052
659.443373929456 227.2511851654
658.573049475899 228.166217616593
658.471054640444 228.271656926768
658.17809105179 228.571861213809
657.321324995958 229.430534548889
656.855262784848 229.88415042104
655.485258768224 231.178710116825
654.090036529636 232.460879007759
652.67044656296 233.729152200792
651.266390345372 234.941304010357
651.226674814583 234.974870227755
649.803911366554 237.178057591259
649.700602436464 237.336219790024
648.376183128173 238.405079931763
648.215593565709 238.532531561926
647.051068715349 239.446263616211
646.929925813368 239.540423885617
646.705991991808 239.713845805512
645.464419418391 240.663660002356
645.176356168806 240.880606723069
643.977826216795 241.769951650364
643.620580020663 242.031279371782
642.585520692159 242.780839963464
642.029236904007 243.179118650625
640.401276491017 244.326809989975
638.784377690056 245.429806641733
638.73863534915 245.460458092727
637.15761294549 246.509885131742
637.042203681668 246.585985138619
635.642686876305 247.504529283065
635.317196991824 247.716645779714
634.351950861596 248.565055465337
633.73839138194 249.100240910046
631.971765966367 250.218252085901
630.30561942042 251.261105597741
630.18412098794 251.336680721456
628.565348457081 252.334690943453
628.368152188793 252.454878447801
626.793640474746 253.404134375006
626.518580559639 253.568134908418
624.993773432093 254.47052936991
624.637687907206 254.679436959775
623.317587472733 255.449545690704
623.164279785242 255.538532902748
622.727291796695 255.791537389624
621.31202266272 256.607049303253
620.793693529883 256.904901886336
619.445657634121 257.676728296589
618.845889616094 258.017089576595
616.88335353681 259.11192617976
614.906093169491 260.190616515047
612.927249775213 261.254617673789
610.942410537019 262.303300424394
609.007331417943 263.312914919731
608.95246704265 263.341307822715
607.084066176504 264.298740827777
606.948456969939 264.367509073478
605.144192382696 265.275340531302
604.925963661324 265.384272946306
603.184817387404 266.247859827587
602.881894711632 266.397272021448
601.206257271747 267.220327200275
600.817827775629 267.410829624564
599.378687890914 268.116555564999
599.212066952941 268.198070221393
598.737332758087 268.429805538596
597.203949112407 269.17406481964
596.644353693794 269.444223219424
595.193998145399 270.141634072821
594.550282395548 270.450557220173
592.451705415347 271.452130983741
590.348940972385 272.458022052159
588.24806597606 273.482128577802
586.142467429665 274.518567625651
584.255821979268 275.449588490476
584.086658898721 275.533032313197
584.028889864118 275.561528301012
582.056926530911 276.531621509163
581.914618870689 276.601310272503
580.027469091925 277.521373005709
579.800897848011 277.63135834687
578.171998775672 278.420970342882
578.003710708528 278.502452428896
577.695028534886 278.651677909812
575.993379464491 279.47190064709
575.601609349133 279.660240767056
574.15278054368 280.355705498301
573.985372679477 280.43570954288
573.509502523438 280.662717636277
571.971256005525 281.386083153831
571.408607248695 281.646700624115
569.95139633242 282.318592474407
569.306023502007 282.618136857027
567.936244967637 283.262424414749
567.207119332548 283.610683442687
565.119868157387 284.619780270127
563.068352236879 285.630034418385
561.052084281768 286.667235268456
559.132889150415 287.702419092183
559.079615641948 287.731885817403
557.284064386182 288.749229729614
557.156523032727 288.823306413944
555.625168396653 289.72836709221
541.277176727546 302.835025542605
541.153766722935 303.010443093996
540.286617304965 304.290183833859
540.039049806264 304.671711119705
539.268500636942 305.915462173908
538.997991615835 306.374754343585
538.322908363171 307.577107776769
538.036825871592 308.116805109397
537.552415705369 308.639455002074
536.754276279317 310.445646410997
536.04270675142 312.212541485044
536.023667900119 312.262607144972
535.410913385304 313.949891724414
535.369334710349 314.069206121884
534.880972771231 315.49777386484
534.834253735711 315.637161854136
534.773287412117 315.820209565273
534.31151125347 317.265653886718
534.238318847893 317.50745101799
533.856411066704 318.820459685772
533.775086665479 319.110329739672
533.453035746271 320.288343071914
533.364173802904 320.622255647447
533.095602797431 321.668831080609
533.00405174481 322.04057668245
532.78373208127 322.966751731398
532.691400541171 323.368829817183
532.417936819072 324.608624199782
532.190769844727 325.75267946255
532.006320331933 326.788138331435
531.855245968481 327.72836118655
531.741150311816 328.503873903089
531.72880428049 328.591646296055
531.638378058309 329.271866786965
531.624683581878 329.384163584309
531.561178256141 329.943178709471
531.539934788686 330.147237089121
531.487229309151 330.676172692173
531.464211075399 330.910844330241
531.38567313405 331.673751993207
531.303034355016 332.439437193553
531.221330138703 333.207612286113
531.356838594777 331.554059857159
531.293368722728 332.162456893212
531.291799246971 332.177388100417
531.245887944918 332.613620468756
531.242387531798 332.646741994781
531.239419995458 332.674615873859
531.203820612701 332.996690657162
531.200531742526 333.02527175251
531.180143361526 333.201072911001
531.178363491666 333.216430254048
531.176059364876 333.236386048968
531.167249390846 333.313021858118
531.165100552698 333.331700359636
531.160490341709 333.370580280148
531.159382241827 333.379573985659
531.158503065571 333.386630842775
531.15264875479 333.433106292761
531.138785406238 333.543124236032
531.111815711999 333.761148207091
531.30421422017 332.090173701176
531.23504141292 332.656328590272
531.145075892326 333.416019697536
531.143221144161 333.432136466187
531.044688306473 334.293457997813
531.034066253982 334.386332353497
531.026446695897 334.453004069577
530.910815236532 335.460681182901
530.883160181162 335.703145684484
530.756711269906 336.80866661519
530.718325864096 337.138602220172
530.594020000964 338.189191792373
530.578440701018 338.318785913535
530.527142633529 338.7421040183
530.318284936395 340.454240992566
530.115840159428 342.201285664116
530.112421885447 342.232651093271
529.947427468964 343.799597414649
529.932644530919 343.945705204838
529.922101185633 344.050556790729
529.755748101312 345.699898259628
529.737676477739 345.878179255522
529.579899016183 347.45538746776
529.555961970812 347.706203741209
529.435372322708 349.061793434157
529.397661734012 349.530921970576
529.272842693946 351.350600501198
529.211583744354 352.555979714195
529.187174000493 353.169139945685
529.138966476503 354.979811730323
529.129661483057 356.776937860406
529.166279364002 358.552341777297
529.244854065152 360.268485436965
529.246597064861 360.298242808015
529.352262825038 361.909083646508
529.359628532567 362.006133728847
529.455871510361 362.771297720834
529.466910772032 362.844914489961
529.480593202382 362.933647062457
529.613607558045 364.243286299359
529.649207483723 364.606226447641
529.774843858016 365.992611746853
529.786568199603 366.130540476388
529.800705820502 366.298359471547
529.913814150378 367.658644778241
529.946827276061 368.04257520227
530.067733352432 369.371238117982
530.111986138959 369.837305318415
530.237104496244 371.118217052778
530.29208553605 371.665768169133
530.418812231995 372.894565574082
530.485834180771 373.531147005529
530.685226770999 375.440047642698
530.87410240653 377.382635748224
531.067131048751 379.337486051363
531.205348696313 381.536999248188
531.207918220882 381.57554448218
531.426988803866 383.409234995181
531.440234262587 383.520950552626
531.64557339706 385.267442722756
531.667247601094 385.454348922411
531.856538291632 387.108132517698
531.886435482863 387.370754332479
532.06762170603 388.944173023964
534.309358452962 405.085671757749
534.322394467327 405.174065131678
534.334232394726 405.254334858655
534.336797896333 405.271730818828
534.467520244412 406.152419818201
534.474352487022 406.198267105258
534.573951855965 406.865896293159
534.583122159421 406.92725616018
534.65277713053 407.393239391939
534.659484825982 407.438264908143
534.669616960596 407.506373585986
534.720268374883 407.848010898684
534.735893849255 407.953451525872
534.787121972909 408.295373523545
534.827672490472 408.564676207352
533.949462066517 402.626495885261
533.983272775654 402.855740091256
534.023986057124 403.133080918059
534.081777744461 403.52452801376
534.156742435772 404.074336489468
534.240927848949 404.772225391479
534.242560380509 404.786401188482
534.32725472578 405.522625590017
534.336269916026 405.598803258627
534.342739466855 405.653470468697
534.44199227269 406.469272566436
534.465800158734 406.66200916384
534.57486824172 407.539856214942
534.607323668764 407.798021714467
534.725062942978 408.71564252735
534.768069095395 409.044958405423
534.946480569579 410.401032351518
535.529083782825 414.183924931868
535.831252364089 416.139073797501
536.029684289194 417.699506435067
536.219697430712 419.328784990915
536.399820362455 421.002943483845
536.552085476712 422.548598310131
536.565026908103 422.686854705938
536.567926360678 422.718056508836
536.713728439557 424.350903512075
536.722365476502 424.45171345396
536.85244120479 426.027729980701
536.866185197699 426.199545977513
536.983547012341 427.731598470164
537.00133811364 427.977461628127
537.096849535399 429.454930694242
537.11523602248 429.776882224123
537.191161978622 431.341388074861
537.200814416605 431.592484022702
537.241272322849 432.955425897316
537.244406363022 433.102819878728
537.250558634746 433.430910721672
537.266649748817 434.740057148231
537.270936988679 435.297586447734
537.277463713626 437.184411041812
537.255676528291 439.072816163899
537.198733451644 440.949621411336
537.198204232627 440.963572225319
537.117767047962 442.771941279478
537.113219755212 442.861670333887
537.014898685921 444.60041411957
537.004350846457 444.767437492764
536.887722547159 446.439841657922
536.868694315852 446.687651756242
536.74812696681 448.145704899028
536.734296125637 448.301300740767
536.704592863107 448.628966835611
536.553241805682 450.188497526348
536.511285308001 450.599554994073
536.354502002454 452.100729722726
536.302198477315 452.597018866418
536.149628683909 454.033301954639
536.080967354813 454.674256794615
535.938011991111 455.986307799733
535.863849457493 456.654758871365
535.642977786668 458.702709004092
535.456798753347 460.759028062283
535.323963777011 462.717859590139
535.31832101344 462.815143705473
535.22022080777 464.839794000864
535.21966516562 464.854642456488
535.16948919132 466.777604267504
535.168284709327 466.871652553498
535.167287290507 468.692253038071
537.67541488785 485.785833139313
537.987910495473 486.851483202116
538.028092720323 486.983894306214
538.169142118423 487.443453016173
538.692280888981 489.101953212283
539.236478437163 490.772443015239
539.79179807573 492.434746563988
540.354469810143 494.047894036196
540.910146018141 495.573936764781
541.407429257571 496.913273230982
541.425202247304 496.961149876747
541.841766002946 498.09038777885
541.872679773823 498.174604902398
542.208061967044 499.087899846203
542.246500432966 499.192055576197
542.505337686828 499.889521058219
542.545382987451 499.996845600401
542.72006185017 500.463824653198
542.738563240462 500.513199847426
542.781376031428 500.62737768351
542.933933307203 501.033076798749
542.97642794969 501.145629498212
543.101407071067 501.476160414133
543.148250224598 501.599760106935
541.733031848204 497.661140513846
541.955692718799 498.241699721379
542.253657835338 498.996440695777
542.68314666947 499.998239823054
543.161384603578 501.002684257647
543.214977358094 501.110248104788
543.267292047884 501.214405280199
543.851748903789 502.324710923308
544.014912784744 502.622215158841
544.680686889818 503.794987363132
544.753787635107 503.92026393481
544.906141638046 504.178655472648
545.705229094774 505.497455170836
545.909304201189 505.823974952058
546.722534392903 507.091061333706
546.983687608764 507.486679170257
548.127054186084 509.15192539095
551.162814191472 514.856767903978
552.269058265189 516.245625653032
552.371460800313 516.367446159315
552.419404161736 516.424072720159
553.637084549224 517.799296661552
553.741882518233 517.912995803474
554.961325931094 519.188818281124
555.12793411741 519.357185615806
556.347013907578 520.551860874166
556.578074606171 520.77148973452
557.653821010303 521.763028186036
557.774109949677 521.871211103901
558.073137296479 522.13767993261
559.248885231071 523.153452568553
559.621571230749 523.465751922287
560.769185601655 524.404091329984
561.213006201799 524.758656435511
562.310377393165 525.613488827563
562.821393073247 526.001393507908
564.374466247602 527.131233060632
564.434995146393 527.173799675639
565.504173878 528.788822795283
565.507068509933 528.792835744379
567.085070864288 529.759283661843
567.147416364336 529.795189338108
568.419262451217 530.488081974559
568.818057093574 530.68979725542
570.035457989391 531.265080657847
570.501073585168 531.468911887662
571.639589381732 531.931611744736
572.167410069632 532.129593147966
573.811559677862 532.684798984985
575.445411738885 533.159796410239
577.003342164149 533.566457816281
577.062999930001 533.581395689792
578.659428635604 533.968395289276
580.090695881129 534.305623440725
580.219293188425 534.335853707177
580.263187666731 534.346162908097
579.628936056494 534.519668608976
579.515360425864 534.546966836456
580.819432106861 534.839317893935
581.098991316837 534.900047962266
582.206019316892 535.131525268102
582.331924757848 535.156908107841
582.676140797943 535.225099793995
583.852251940678 535.446678202473
584.260055484268 535.518909083234
585.372126038781 535.702693971895
585.842072552666 535.774717696568
586.898519313904 535.921728206328
587.447828380845 535.98893661895
589.123023794987 536.156615943762
590.866558200315 536.262528185015
592.68749667677 536.302681969683
594.40986828707 536.312594673779
594.56777254315 536.312849677556
594.601940683927 536.312848626054
596.479095860693 536.307107049143
596.572052154079 536.306555638475
598.203814222198 536.346887311548
598.359487462349 536.34831262657
598.529108670517 536.349426033373
600.090030063945 536.341691543712
600.497935344891 536.338343944152
601.814302979821 536.320142660916
601.970576302303 536.317075282524
602.451435562027 536.306053742565
603.829906146453 536.264190374636
604.382291212685 536.242854608872
605.674881540119 536.184992752389
606.307509821591 536.154343635848
607.538496194414 536.092194871028
607.694298879128 536.084221041075
608.254175254567 536.055498517011
610.206324420566 535.956722055632
612.142533668063 535.855595279658
614.040389050583 535.732783227161
614.054256287529 535.731806650243
615.702331299045 535.611599350206
615.940434968728 535.593593790284
617.155294035972 535.629694085001
617.2837509536 535.632897201357
617.551267265682 535.639257921181
619.009889771679 535.518046449506
619.389873379833 535.485405354979
620.765322308049 535.364635900573
621.216947819264 535.32392990575
623.037197548458 535.15440511578
624.716046271453 534.984491767226
624.857075399256 534.96942459807
626.618339538023 534.77369921622
626.687237784549 534.76597934517
628.391551555221 534.576375630789
628.535871072883 534.56039372694
630.189714528299 534.376357210354
630.412201551416 534.351602641065
632.016781731279 534.17074782448
632.319917246055 534.135935227727
633.868224084602 533.953496549095
634.250712594257 533.907344007337
635.572877343076 533.745729124449
635.727717492784 533.726401416378
636.186610809892 533.668442077033
637.581434578143 533.486330318653
638.114750447289 533.413898919138
639.415931061556 533.230882334418
640.017184611081 533.144620440233
641.885307700235 532.874896455467
643.422622383936 532.654011272049
643.564170903056 532.633591791403
643.701085287982 532.613805211565
645.091545737066 532.408898203505
645.22812720436 532.388374128226
645.421366124855 532.359153106511
646.652571434526 532.168473339931
647.01622147002 532.111298070041
648.078423098915 531.944045476837
648.462182677167 531.884107887466
649.71944315859 531.689315745923
650.781338609138 531.523381432571
647.56625882849 532.035312041967
648.314633265669 531.914517608691
648.989378263136 531.80746362222
649.628121669812 531.715652580758
649.652895701875 531.712435984417
650.269201615193 531.641652013192
650.321405157073 531.6364704208
650.928633063508 531.585406286986
651.013079306243 531.579553115638
651.57128602057 531.549374629952
651.630697505828 531.547105365056
651.746916157699 531.543446600092
652.338216675815 531.537710754784
652.481377500296 531.540264719452
652.966784761989 531.560687116674
653.022933086704 531.564218987412
653.186874588533 531.575981758754
653.624524654272 531.617836846474
653.864264318484 531.646911921473
653.204097959451 531.583418987632
653.126085508985 531.576726828886
652.893477708571 531.558100274416
653.516801123567 531.693410635375
654.138224389289 531.872418431357
654.799768494363 532.109869715118
655.527699035384 532.420242560934
656.309404108057 532.798143580049
656.341894303932 532.81462184244
657.169450420766 533.245528489588
657.246125095128 533.286271806442
658.151839207098 533.785972635733
658.281249321696 533.861409287733
659.131387325633 534.387097027787
659.221187984581 534.445856498206
659.405184614207 534.568424309148
660.336297477146 535.234588500814
660.565289739764 535.410177186029
661.356255409858 536.060134766911
661.448563134482 536.140367535391
661.728461907037 536.390633022168
663.183936804248 537.869417235068
663.34108713572 538.036093751915
663.724040878743 538.448868206766
664.472416430433 539.289540607076
664.806672934364 539.693949622177
665.804987163719 541.010948789806
666.769825965836 542.384126270753
667.7163235142 543.792912281218
668.461113072661 544.97886527733
668.529166150657 545.092600279237
668.595172873103 545.202915270482
669.322351651201 546.473086600579
669.417759115094 546.646848906806
670.028357981289 547.795220686953
670.09124181197 547.917564613147
670.215946009109 548.163013075234
670.828048515171 549.433000709822
670.973231447086 549.751550609119
671.518718891571 551.013355525406
671.685327113185 551.420123128796
673.473756074286 552.313385533775
674.054504999764 554.028413198707
674.10083053992 554.174880607977
674.650036736143 556.014528520331
674.670522587515 556.086619306795
675.15770016553 557.883099675679
675.196786158158 558.035436634704
675.616686879722 559.783522104135
675.669056648021 560.017862115375
675.988785867821 561.547371536311
676.020513120013 561.708411147701
676.081973166665 562.027823468348
676.376985580136 563.668698083922
676.445121480871 564.076516060039
676.697333687941 565.668131445194
676.773153369284 566.168999349424
676.996460282596 567.709836364583
677.080665717658 568.309551808923
677.375890838556 570.510293765773
677.561780207772 571.985710700201
677.659558324163 572.768385506476
677.936198195968 575.065483799677
678.191855522835 577.326997879754
678.198844347694 577.390969879832
678.43782035652 579.577791319423
678.455191117838 579.735939992167
678.682836262894 581.837787443638
678.708933979525 582.091832876621
678.904697989277 584.116019659209
678.936636782317 584.466296838625
679.08937875814 586.208039193813
679.1055510685 586.398219530122
679.143251634904 586.844045145357
679.290933995021 588.684603892371
679.331862172313 589.22687586895
679.499839490098 591.61234383576
679.639192868592 593.833708743764
679.648671453655 593.993990132435
679.766135886012 596.119437035442
679.779473758286 596.375337474694
679.878550211724 598.411109514898
679.894709255877 598.768198607934
679.977577126767 600.708102734656
679.995225894573 601.157205005332
680.054582977038 602.816353505081
680.061066851482 603.008141150862
680.079242795597 603.553598819894
680.136873813394 605.308477509785
680.159688122644 605.946787853636
680.23276640211 607.594332406477
680.273382870575 608.324573963797
680.446281095972 610.706257740348
680.662482855005 613.086949778039
680.905164426728 615.454091779663
681.149485577868 617.643552350609
681.167965584468 617.801171834819
681.451535477215 620.07295738548
681.459895682503 620.13622232146
681.729722333273 622.097960020105
681.755898489007 622.279826102055
681.778324153102 622.432810562793
682.09226690424 624.453645268718
682.132380894198 624.693875796453
682.472769509832 626.596830361502
682.535162823082 626.924312263825
682.898602286322 628.718835885138
682.98662723957 629.127635013321
683.364405266163 630.80462762054
683.47971621419 631.292936473879
683.869677575469 632.850552339024
684.019316522862 633.413879496206
684.419913913679 634.853814560231
684.604220627084 635.486360811917
685.226819026979 637.512918024136
685.881707200132 639.48681481617
686.572223686213 641.426268397188
687.314174630327 643.34276947019
688.098847883475 645.186609744531
688.121866121919 645.238126615278
688.932281361108 646.988641489518
688.992470459434 647.11486032804
689.803041939172 648.787687406139
689.902671509819 648.989865071823
690.704117994922 650.59839067512
690.843487376468 650.875472339634
691.536926457963 652.248643215521
691.612691777164 652.398218581331
691.790426391419 652.748973679272
692.524555609416 654.191477439866
692.742062759864 654.615311445867
693.448125161201 655.977079742801
693.70727062691 656.472462177334
694.376524097706 657.750336048696
694.6700475777 658.313613423616
695.608334242901 660.133989143642
696.461132696634 661.801862247637
696.521601880031 661.919565233443
697.317775184018 663.456691055547
697.411844590706 663.636413509161
698.151162310384 665.042406113809
698.274260172523 665.276004803447
698.939750590664 666.536158780976
699.087976650027 666.815710745543
699.617856692026 667.813400409871
699.842668917926 668.236653956844
700.529425655457 669.531219381003
701.127183739785 670.655871155411
701.628123616145 671.59357646591
702.032701172615 672.344345136159
702.326260841973 672.888427791395
702.332806110203 672.90058269571
702.525432283344 673.2594613273
702.535810961417 673.278888316577
699.703325533263 668.637596136721
699.35530694949 668.062513234086
699.410257831895 668.165034848204
699.415062304219 668.174001489383
699.420539212868 668.184225246433
699.445756227286 668.231398970324
699.448863351302 668.237204597032
699.457549480135 668.253392075921
699.458624419939 668.255390124524
699.460502731192 668.25888227892
699.460842128692 668.25951558718
699.461438685179 668.260634033071
699.461438685179 668.260634033071
699.461438685179 668.260634033071
699.461438685179 668.260634033071
699.461438685179 668.260634033071
699.461438685179 668.260634033071
699.461438685179 668.260634033071
699.461438685179 668.260634033071
699.461438685179 668.260634033071
699.356768517326 667.780473811212
699.344440145017 667.724569235965
699.33202717796 667.668409837638
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135022
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
699.310516813696 667.571390135021
};
\addplot [teleOp, line with=\trajectoryWidth]
table {%
665.000152869578 62.2420193609231
664.97156022786 66.0686823047975
664.96476992742 66.9610559288975
664.964726212365 66.9668830218034
664.957094389038 67.921931438888
664.956711058508 67.9705084331725
664.720232882737 70.8452318943001
664.698068096466 71.1195008539769
664.692356079682 72.039403683868
664.691881257966 72.1347834325998
664.691158596247 72.285360812218
664.688091212057 73.1986045605617
664.687250707188 73.5049313726981
664.683306881247 74.774204121068
664.679011963018 75.650406630621
664.676601648672 76.0791714505804
664.669389143413 77.4061975729531
664.665623067429 78.7509645964254
664.665616050109 78.7597751828963
664.666996170762 80.1391680618179
664.666874921938 81.5438226734014
664.666850058878 81.552952076527
664.66145159452 82.8173882044128
664.66089742593 82.9351299902841
664.660591665232 83.0029218511729
664.655371190122 84.3745490444762
664.654972776507 84.5064204815716
664.655812286139 85.6117131096035
664.65636768048 85.7383164139006
664.658301126073 86.064552678828
664.667903565048 87.1398756865466
664.674053072588 87.6674858272446
664.697813672741 89.3039365732649
664.730916042276 90.9611869544247
664.73116365162 90.9720612711555
664.766068729696 92.4479546607735
664.771227486021 92.6622948676099
664.810039696375 94.2280883225188
664.81360567323 94.3766306104792
664.841349333723 95.6158962210808
664.844537041258 95.7563354164461
664.853454250636 96.11852642604
664.893116166609 97.4518127914134
664.898071463351 97.5948201922052
664.90888759967 97.8914760479144
664.969625024934 99.3201152256994
664.987797653618 99.6925696189007
665.054027391457 100.915354234556
665.062459694112 101.060565152784
665.089421678157 101.509515963382
665.314544969521 103.378914210698
665.340348363598 103.58923130005
665.40731020758 104.130749685744
665.505148579763 105.517669454817
665.53780915777 105.971490145307
665.634820058026 107.287676720677
665.675090515556 107.813449631894
665.772328620072 109.049342110362
665.820145553922 109.647660628641
665.967903707259 111.485319575065
666.104319288088 113.159516714077
666.116260521153 113.305458460309
666.117202451932 113.316957965597
666.248715865485 114.906734675609
666.267902042826 115.136272387
666.393969801615 116.645648562753
666.406002014732 116.790615889783
666.418988094794 116.947156801034
666.552221988261 118.532539746104
666.571787871612 118.761696717154
666.691374465001 120.13375378379
666.704308147673 120.279610399885
666.731179814524 120.582431821922
666.84653604706 121.890266299785
666.859441256822 122.038211534452
666.892575212079 122.419621993231
667.013550270688 123.820455145926
667.053283153268 124.281670091264
667.220263819751 126.168907384242
667.336842893475 127.453760879045
667.392678397519 128.080483005978
667.552701515741 129.925258818952
667.560505127499 130.014882703752
667.717489748672 131.800423059876
667.732473046986 131.969368372285
667.885765912283 133.688717280374
667.90799373022 133.93749129703
668.055056503665 135.587254939644
668.084480978013 135.917503831436
668.211437345442 137.3335790981
668.263391277387 137.902007962117
668.445684003306 139.877669711757
668.446835844083 139.890087663045
668.621296319379 141.786565083524
668.629715717211 141.878184745618
668.797974606612 143.694429846355
668.814048704852 143.865504411643
668.979290576018 145.602004867857
669.003518375184 145.853165485169
669.148673360574 147.354242393659
669.164119141297 147.514042970421
669.196198720379 147.845874060966
669.348670741334 149.43516407566
669.388025088783 149.848960536322
669.531062515779 151.364484735148
669.577506526562 151.859811596668
669.76779916043 153.874881489488
669.963824183636 155.895346024438
670.160447933567 157.919449245639
670.33697657026 159.765831191482
670.352283198203 159.927258622137
670.353455346963 159.939627688484
670.532523296884 161.858454193378
670.540713177265 161.949989528414
670.69398554678 163.781761040222
669.86251352391 183.348301771781
669.860736950542 183.360057412426
669.607413953538 184.053805265618
669.326247798838 185.935523284921
669.324447307066 185.947314752724
669.039775327664 187.744889877855
669.025644653183 187.83075669791
668.767430911131 189.387621094205
668.716581355987 189.695221400449
668.499617048815 191.020753510679
668.475387407316 191.169975330637
668.413040770042 191.555029055248
668.188458649787 192.96479413065
668.118746832386 193.427491411463
667.897751559232 195.30341096965
667.840788422511 196.531824033032
667.843508440457 197.108348308403
667.953881593908 198.842735245146
668.147823073891 200.504250933703
668.332403003251 202.021821526097
668.338392410438 202.075356269194
668.468596285844 203.349568771505
668.478066603527 203.45030258799
668.580856887729 204.571736097412
668.593973119132 204.714019686496
668.687043435271 205.688540022775
668.70360861611 205.856534871271
668.78346708535 206.662909538946
668.800754591833 206.838220205573
668.86186379671 207.468142437717
668.879328006608 207.650410713564
668.931174273444 208.193331663438
668.949484522527 208.385533272498
668.993351711936 208.840784290912
669.01208811827 209.03373262523
669.068321582211 209.620958803517
669.115184703326 210.215694688321
669.148068528543 210.852367761329
669.172887540984 211.542794482242
669.205670336685 212.258704612316
669.207198193695 212.286552112309
669.252740550485 213.040757253916
669.256907172407 213.106337605338
669.305707871191 213.88299928936
669.312012259085 213.987343444318
669.357203382129 214.759135502738
669.365535284425 214.905049520832
669.407815432527 215.667308733238
669.417613517898 215.858643134501
669.45260968557 216.61904399712
669.462170325777 216.86099806773
669.485081117619 217.602576125631
669.491182088759 217.884976425942
669.500546349885 218.925896592549
669.494448540418 219.612714267597
669.48604176307 220.002288553057
669.653324571164 222.809378989378
669.577428727317 223.994817715022
669.471366980967 225.16778703674
669.460782437295 225.268358064348
669.298523132666 226.597007960913
669.291401832154 226.648839642441
669.082728450657 228.016114286691
669.063055073794 228.132793967123
668.803760397157 229.523052406
668.764888581466 229.709991998898
668.479619379208 230.962700107447
668.446482896248 231.096924202098
668.3802805353 231.359094999158
668.004184770504 232.714858487664
667.90316036715 233.048968214839
667.526695923052 234.206347431636
667.480002771552 234.342109562077
667.3389614776 234.741586364758
666.877496286073 235.961920445447
666.688985914862 236.426130535983
666.169227361909 240.457819825082
665.658052735197 241.510935236834
665.366902791088 242.087497715311
664.511171365346 243.702434567594
663.606636194801 245.31165242844
662.740962942217 246.805697720745
662.668447645804 246.930152111131
661.734656919936 248.523432075904
661.6990825128 248.583689023684
660.77093916383 250.141756983595
660.692532122258 250.271936272613
659.773936296916 251.783122858438
659.651513343803 251.983276877842
658.75234027883 253.450135605104
658.583274276843 253.724688772884
657.787092605513 255.006371055959
657.698118600822 255.148391777935
657.478939876196 255.496544279744
656.614557955096 256.847148905947
656.341637039644 257.265880946968
655.788358298543 258.903500497008
655.572021330765 259.531079859668
654.740284003952 260.744668299555
654.348697802298 261.303715748015
653.08112808539 263.058242999347
651.771668729555 264.794164787743
650.432232692549 266.51685928441
649.282211882429 267.950957340545
649.17231655646 268.085864191568
649.067111698076 268.214636615424
647.951017094488 269.55756919045
647.675724929299 269.882514674834
646.592449549883 271.132196935969
646.252311707921 271.512547975858
645.195948530047 272.658218287191
644.788581659324 273.088310478629
643.770472737957 274.140790555697
643.298056802615 274.622638897223
641.802589720628 276.135640216138
640.299222650705 277.651359570102
638.83247667529 279.119220203351
638.776708227514 279.174480740443
637.348205904263 280.574488684133
637.229189461923 280.689774675712
635.841932087142 282.021174128898
635.658739882256 282.195458963972
634.320732165415 283.463319304954
634.071899977519 283.698466706368
632.795763375722 284.900211770601
632.48521829455 285.191177760064
631.398368294053 286.201434703145
631.270902702026 286.318915516107
630.89376225882 286.664602554767
629.732004312485 287.716953648191
629.287545758823 288.116012855029
628.184645776082 289.101056461339
627.67174517954 289.557797510308
626.626931205812 290.486578876802
626.046053678989 291.00224838573
624.397592667409 292.453181015278
623.281100259805 293.8863783906
621.710834762092 295.227212733395
621.579902355067 295.33811393384
619.914243742453 296.736692311757
619.850816294833 296.789399216648
618.232943501673 298.122068373481
618.098845466979 298.231839638647
616.686610791019 299.384547361152
616.546393152859 299.498866603538
616.342107826547 299.665217806877
614.864359699015 300.86136400103
614.590876645037 301.080850913675
613.181951713229 302.199069098471
612.838472092235 302.468234730787
611.497970950866 303.504391453128
611.083775371721 303.820908285256
609.81595610137 304.781705820843
609.334534243986 305.145217439518
608.145277442556 306.041044706636
607.597786030012 306.452900476857
605.870675590923 307.749110532491
604.159885323206 309.041838653281
602.46451110818 310.333309345066
600.919315228726 311.509998920872
600.792926334886 311.606332877162
599.200944126931 312.82277225568
599.141507777086 312.868166283691
597.621387605946 314.025689276843
597.495711789513 314.121062962433
596.044710585899 315.223941111392
595.855020769485 315.368577592793
594.613392503519 316.322009312854
594.483610912609 316.422368194557
594.230535414872 316.618508501947
592.927308821723 317.632995183072
592.608742965137 317.880723971271
591.365109587246 318.84672139278
590.980550289858 319.146019144656
589.808826475256 320.061963881113
589.367395052358 320.410956148276
588.286481434191 321.284334844237
587.791560267519 321.695016521672
586.240991359296 323.019979783716
584.713833568955 324.371408133767
583.216939900538 325.738712243078
581.747624866912 327.117833090208
580.475245047221 328.353889104954
580.362313907562 328.466436628013
580.3115400228 328.517286783827
579.03333785223 329.835170749585
578.930015532696 329.944859472486
577.751942955009 331.229755325971
577.599797247099 331.400228400593
576.620305124747 332.532734108969
576.520019998515 332.652861527831
576.32550743477 332.888563125789
575.359361688597 334.117588014283
575.131439860923 334.420160881159
574.653476534036 335.451204106296
574.600605117342 335.57324071685
574.448131186046 335.932321995818
573.699569360039 337.077988863795
573.434563950905 337.512771963781
572.5652928123 339.091131372159
571.844527726689 340.647507793678
571.265820634671 342.148639528485
570.845401171172 343.519131799002
570.831939171178 343.568940264458
570.521326930872 344.865678020481
570.323200604012 345.923230808199
570.308512204331 346.01398498315
570.302061581551 346.054952694764
570.169840628441 347.036617188783
570.160938177269 347.112448504744
570.064511488567 347.952582177608
570.051751181308 348.060635400828
569.964392106903 348.760730737778
569.954899081221 348.834305823534
569.936297151229 348.978193185539
569.844318590779 349.724768395664
569.82377447176 349.910199769036
569.752413768014 350.651064285955
569.733624245106 350.888066784867
569.690774163475 351.571722547475
569.672410247701 351.988266757243
569.644592329801 353.276083543523
569.663737734956 354.544244657754
569.670558165852 354.717307425832
569.764563867626 356.046873910709
569.791440132617 356.306486596282
569.95443479802 357.529300271808
569.9772978019 357.669705705387
570.034397283737 358.013602720586
570.289298642929 359.354640231538
570.377721124254 359.7708945372
570.664759742392 361.044586667504
570.776745039945 361.536530388828
571.018413133498 362.623065452293
571.049981938899 362.767628446934
571.174929173246 363.346148648877
570.863360312928 368.365615741753
571.260352558156 370.145219783898
571.641690119062 371.878539990909
571.655408580281 371.943928475265
572.01362753704 373.777443138276
572.321235991451 375.564992942714
572.332271361892 375.632289324784
572.614586736076 377.388662653721
572.638003241818 377.536552964528
572.906785305669 379.263621920078
572.94125394614 379.492564193388
573.181281781173 381.172779327767
573.223317258177 381.488486608405
573.426348879439 383.135758666365
573.473077225278 383.542754681189
573.629371334841 384.969463182719
573.647007349356 385.138321630525
573.698638401563 385.636769107614
573.849191008466 387.172035382441
573.903821697393 387.763205100609
574.032249144688 389.231544489989
574.088486989104 389.912038062791
574.261787230394 392.07609628594
574.432019076185 394.244306831592
574.6068770257 396.400227351397
574.775098675611 398.387005248898
574.789328425792 398.551793375961
574.970284330156 400.641726904977
574.977073081023 400.720712939644
575.118211968923 402.401381392685
575.132957339332 402.578399559282
575.161751941728 402.92397351151
575.299205745637 404.531628849914
575.354685828501 405.149910551237
575.568517866136 407.403832197607
575.785882101291 409.687430604738
575.990693884218 411.989519725785
576.15062332477 413.845153227321
576.190865497815 414.296748477083
576.353678189295 416.050482732417
576.405960881865 416.590100995502
576.629366966224 418.859664592347
576.834972043598 420.936879804076
576.851691506337 421.107315800865
577.040872827777 423.085781048741
577.065217448946 423.345917800174
577.224444955696 425.052995940608
577.274941995129 425.583036428142
577.434969114693 427.205209141864
577.498160013456 427.827559643505
577.65854883548 429.370707882186
577.734038704816 430.088092161288
577.972813410751 432.372597618434
578.211369316759 434.687856001535
578.442713930539 436.948315485143
578.451653402459 437.035552310989
578.698321936801 439.408086708966
578.948546315893 441.717165055469
578.958114795496 441.804832055123
579.199389718727 444.030500933428
579.219230170759 444.214036916544
579.44869912541 446.344053666385
579.478595304611 446.623669121936
579.696773099234 448.656878963034
579.737749176817 449.035056468967
579.953142870828 450.98113154742
580.007071438788 451.459932856061
580.222590617205 453.353919642653
580.286570966036 453.913188333497
580.495623714821 455.73276713635
580.572342523944 456.400868377664
580.772444161402 458.149694710167
580.861911725384 458.927806494889
581.15740253597 461.478659878273
581.460154295643 464.023590607769
581.768073570689 466.545706655159
582.058782504252 468.864931485478
582.079594005144 469.028655676726
582.376948363253 471.388219735504
582.384873831965 471.451735022796
582.660796535036 473.653046890348
582.680379781628 473.807888764686
582.941540857826 475.867856605797
582.972254670326 476.110093496234
583.195866009632 477.867134301924
583.218947995743 478.046885354202
583.261250138879 478.375485708758
583.497603731325 480.195642174893
583.551578286362 480.609906438764
583.749570549418 482.15057183068
583.77213496433 482.328319788159
583.835447483227 482.831231993275
584.039239826936 484.460706710294
584.113224013523 485.051695596945
584.309723703452 486.591227802786
584.398921929865 487.268627440209
584.599488235094 488.711219728532
584.71361322776 489.473043753864
585.064251617422 491.664328690565
585.441050159676 493.837541506738
585.821939695964 495.83772083758
585.850061176067 495.979478372803
586.272785795593 498.028475861179
586.284432380653 498.082986677541
586.709449026886 500.014510575417
586.740400087188 500.149974029442
587.130123715983 501.801222551836
587.168702172313 501.961565512008
587.220078010599 502.174781359348
587.629150637705 503.881912382771
587.698318699099 504.173921187514
588.080154477982 505.794479091513
588.166872356236 506.162443614272
588.528935165909 507.690986218964
588.634994139668 508.136964022767
588.981722754166 509.584682301434
589.108600221384 510.110692850301
589.441752580908 511.482408926538
589.59169637597 512.090481711457
590.097559054895 514.054619215322
590.654367554024 515.984499446793
591.283823625125 517.893946886824
591.950463777848 519.620761081905
592.000400350856 519.742127660944
592.756572246865 521.488676732628
592.777630872798 521.535041559029
593.564456783623 523.185479471387
593.622971712184 523.301707242533
594.451571872721 524.861465645204
594.554609244025 525.044901710595
595.325093703437 526.362413637763
595.407574809317 526.498354819802
595.559764845464 526.746544784416
596.485328254629 527.609303284838
596.70914904398 527.801320804033
597.615724275581 529.079958651127
597.888328100977 529.451847648339
598.788311861643 530.647819802207
599.123233645505 531.07996722085
600.018124754999 532.196216313689
600.424600693603 532.68614107794
601.794958875905 534.264071698564
603.238869658185 535.808385197623
604.716346138495 537.283416390005
604.757385573913 537.322806133359
605.980628789726 538.45934326739
606.346180886462 538.781684291421
607.554155530935 539.800760051216
608.000284881669 540.160191959497
609.181758116513 541.072558028225
609.708098429498 541.459404279925
611.455534885111 542.648011384791
612.800493488091 543.570763722026
614.390347289824 544.384187120305
614.531913678122 544.452139797691
614.578260208042 544.474172902343
616.219458447202 545.210095661102
616.334248179457 545.258446740137
617.732366185616 545.815319644515
617.867279783856 545.86592056489
618.046723520216 545.931734867972
619.47196786069 546.424337376628
619.712107928176 546.50155828865
620.909675529171 546.86377818007
621.038727881485 546.90043476852
621.338990002494 546.98511235253
622.46159652206 547.284993525976
622.95756889328 547.408688894188
624.588011693745 547.774371237182
626.256339894985 548.104269675283
627.972532340915 548.427901956855
628.020269467222 548.436677507866
627.788526934569 548.862865952539
627.775786114132 548.888835684928
629.355322096135 549.152596260692
629.513712251889 549.177652332163
629.72402208725 549.210605718072
631.449205389834 549.466685503728
631.750833039845 549.509272614683
633.452377749615 549.740233289352
633.846462375819 549.791424008857
635.319935897291 549.974264975674
635.491278378635 549.99435316808
635.976273263929 550.049520342493
637.408504779611 550.188797783417
638.142412950584 550.246007728479
640.322434252921 550.340855739549
642.488269322268 550.332226695045
644.628714568779 550.231628338983
646.534853658289 550.069830530848
646.701923097287 550.052469344171
646.735859333229 550.048830621236
648.671778302457 549.806985195185
648.785371961394 549.790793008609
650.507160396418 549.987400421735
650.69042521851 550.003613036109
652.418832808948 549.693883144013
652.68983101115 549.642990032151
654.158381783087 549.358964077269
654.662765174494 549.258191333129
656.046465363242 548.970836581805
656.203480507969 548.937120292717
656.626538209811 548.84480507366
658.248809319488 548.481207614571
658.598168306406 548.401654445013
660.155790153168 548.043766243874
660.587257467577 547.943429879145
662.076842054705 547.589258657663
662.592523576833 547.463439382965
664.617502663056 546.957624110117
666.64993945244 546.436509505332
668.692205655649 545.893808402412
670.547942094918 545.659030558801
670.578456628544 545.655138322813
672.526480922317 545.115318172942
672.643292445617 545.08240497586
674.521347593678 544.545791465758
674.722387187619 544.48781438858
676.528965166456 543.962341055462
676.814632437438 543.878760386795
678.54324258494 543.369644600673
678.91201378187 543.260139004853
680.558151145931 542.772474312976
681.014093719077 542.639525600699
682.589213063554 542.193198251754
683.130066011097 542.044700160099
684.611215397664 541.654827360422
685.23326489644 541.499923629014
686.628219865847 541.179069474501
687.334618665546 541.030731304206
689.426337929637 540.643205771901
691.01333063728 540.644738544411
692.954406081077 540.462309240508
693.069704130993 540.454803903582
695.084641181284 540.38249636469
695.117402962942 540.382281482616
697.046903345743 540.424759142676
697.161866150782 540.431642169037
698.830269091203 540.577508701407
698.990949448142 540.597180767
699.184306967338 540.622382772778
700.906419852551 540.919169893765
701.175270396889 540.978280075367
702.785958389741 541.411092420146
703.124848807975 541.518843203908
704.610507852107 542.068183206168
705.009144795685 542.237212064229
706.343168502266 542.879592282655
706.786256169154 543.118248973865
708.480838619369 544.145182464819
710.090672664883 545.263104025939
709.900915666027 544.420657415759
711.251938567142 545.707383900017
712.424706820742 547.018295920388
712.489925600103 547.100178319582
713.53851095175 548.558222426148
713.554570426306 548.583758448234
714.380118585744 550.069791692388
714.424195709356 550.161285593098
715.012773340636 551.560267454829
715.116286118921 551.848821751192
715.560582729008 553.258395968245
715.65974788625 553.627556109372
715.956167240123 554.833302924587
716.089912247524 555.413078073443
716.509738503615 557.246723143588
716.946193246725 559.131152975937
717.376519897533 561.028737508023
719.16116637676 560.321400609083
719.344846687887 560.241714371417
719.717183531856 561.8299573477
719.75555173696 561.99509298618
719.816143435557 562.256043258945
720.173509092929 563.815905111415
720.288751211063 564.328436278506
720.620347174499 565.835431288217
720.753314442014 566.45816727957
721.217077973814 568.683533261947
721.691588155223 570.968469092605
722.155482444103 573.281294494469
722.584790130469 575.512212591557
722.605446810574 575.620828486055
723.047120197315 577.96374593111
723.04979057705 577.978102408555
723.463575220063 580.237661247611
723.483335212044 580.34743168958
723.835372588635 582.350515440236
723.910576990333 582.745631807002
724.254257854565 584.668981969839
724.344440073011 585.174053030716
724.638178836242 586.830992314299
724.673105243376 587.030543540139
724.780651649755 587.644522759673
725.094762071963 589.437053363406
725.223778986532 590.16518232071
725.536376877081 591.890101272547
725.693767666945 592.731542286777
726.176763392467 595.213373036202
726.201143176639 595.334251586542
726.701009779484 597.731234363702
726.747103803002 597.941181393058
726.750837482659 597.958187392814
727.275758256476 600.248757631165
727.355726520109 600.579584265447
727.854069633965 602.548521275983
727.909260629444 602.756787614363
728.02435822858 603.18902662399
728.602455500714 605.244464501942
728.759986397107 605.773003675113
729.35974728109 607.690057329034
729.564077095686 608.309040443861
730.181764796929 610.089419985754
730.443407163649 610.786048340209
731.390343231355 613.182322536391
732.397524057758 615.498074476705
733.463715613749 617.709344088189
733.470526848441 617.722818462908
734.455951135632 619.598381434678
734.601860708841 619.863659766808
735.496229032793 621.421698917749
735.796813656082 621.919973494564
736.692783234445 623.343205510088
737.060480911742 623.902955809556
737.951021467766 625.198388165813
738.395346919387 625.814101305533
739.788931796004 627.678223207866
741.179510999522 629.529243040209
742.562170760603 631.403418666631
743.959684060427 633.295110642962
743.969026786643 633.307676605437
745.339276338741 635.139800491515
745.406745913968 635.229552895932
746.749580180514 637.016803223707
746.877629072447 637.18759239318
748.188834741265 638.942355007551
748.380257474816 639.199451875743
749.523403273197 640.736433547472
749.64490930919 640.899385600161
749.89831412009 641.238400822724
751.111761697131 642.84806308973
751.429118272707 643.264348961773
752.725710472323 644.946295380812
752.982852451737 645.277938533718
754.208147483479 646.861403432042
754.522709518326 647.270096761214
755.670493935568 648.758968825929
756.043529459667 649.241298823501
757.004555345546 650.482671523691
757.560751683673 651.199474683882
759.077593643741 653.145043230916
760.492726337282 655.002601996592
760.559839532227 655.093721855515
761.982176851823 657.085447346469
761.990740990717 657.097987305813
763.169155449808 658.899132535053
763.272800817098 659.065806553735
763.332123742962 659.162081617789
764.46098616472 661.087590346427
764.563965764099 661.270624289606
765.597927165418 663.12198437391
765.749151775689 663.391064551966
766.862439984422 665.333465580113
766.967852140408 665.51411289652
768.0331994598 667.319644001418
768.184738879071 667.576024516654
769.080853364305 669.101999305285
769.367691713629 669.596169721271
770.187019849941 671.017545917542
770.507093445642 671.576188512892
771.594820107687 673.480776128762
772.241771528176 674.615804115802
772.598573501224 675.239145835486
773.530816883136 676.863571957799
774.380179445958 678.335034554777
775.111079246253 679.603928585476
775.115493938173 679.611626790098
775.609831933865 680.475027794756
775.653627285835 680.55147934584
775.722797190201 680.672003199886
776.130631113275 681.378325003094
776.200969027638 681.499809699538
776.468820119068 681.963725333888
776.492682141215 682.005208085205
776.554216162996 682.112393721712
776.74276013401 682.441812472847
776.788717395934 682.522109243705
776.903410235989 682.722169605679
776.934613776062 682.776537095552
776.989140220589 682.871586726727
777.006580221771 682.901987619297
777.035915778762 682.952982059609
777.044876320938 682.970104871469
777.044891236382 682.970133459887
777.046115637424 682.972266474971
777.04626804153 682.972532857371
777.046275419782 682.972545737447
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
777.046295457633 682.972580706567
};
\addplot [teleOp, line with=\trajectoryWidth]
table {%
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000003
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665 62.0000000000004
665.00000026522 62.0001582111386
665.000028063116 62.0051208527203
665.000035216394 62.0059086615929
665.000050685474 62.0074074221896
665.000235935868 62.0202131797933
665.000338771293 62.0262810493029
665.000803969186 62.0611448430449
665.001255809649 62.1271470732673
665.001294765274 62.1307400340746
665.003180877821 62.236079083679
665.003449338966 62.2472161613308
665.003698563774 62.2572755999256
665.008400328917 62.4435200236495
665.009176134355 62.4725323659753
665.016381640649 62.762140827903
665.017934082622 62.8213222774211
665.027777548726 63.1834732591803
665.029143198224 63.2288572007029
665.032710484499 63.3412566763376
665.05368466936 63.8912340602365
665.062364855816 64.0806171051501
665.092342718075 64.6765969517814
665.096626993613 64.756906211007
665.111694144819 65.033669652768
665.158303065282 65.8258686450573
665.18279778274 66.2077034429459
665.285705942039 67.5743211559622
665.427761780741 69.1181284132055
665.61013139251 70.7732495851794
665.617317067106 70.8319647875308
665.827901835746 72.4028711517622
665.850080452564 72.5539922953377
665.871248226201 72.6959323155711
666.134432732545 74.3066490139908
666.16357023363 74.4695078257577
666.205116607986 74.700428210697
666.515581451041 76.3490437871748
666.614737967362 76.8582515868877
666.980690231912 78.7109849411824
667.068627618513 79.1606197609242
667.389706035243 80.8143092448016
667.538616329252 81.5823486080365
667.899997932633 83.4402190936159
667.940685638916 83.6483341501179
668.039440417758 84.151068844183
669.001721247654 91.8918513249605
669.442291526847 95.4183374670071
669.994317997916 98.1706472094989
670.56254003158 100.989670379245
671.126730223057 103.761403876773
671.145734022712 103.853631983655
671.738232999694 106.721534599143
672.265740927788 109.268318509534
672.333217299538 109.590459521906
672.846495038223 112.029655513652
672.939312071244 112.468437879774
673.385179291732 114.574800405008
673.553339670499 115.366875654354
674.185389555732 118.314181065162
674.840809959383 121.321607979267
675.513672354553 124.396273358094
676.183132722415 127.428052775159
676.20578776332 127.530516433553
676.85809642299 130.486147703906
676.909405564977 130.718438998215
677.601204703489 133.832338797216
677.624417822969 133.9362948365
678.296244210598 136.937808489283
678.348750754892 137.172445984564
679.038281325167 140.303367692944
679.060444635888 140.407155642559
679.67452522 143.402981049664
679.719710385793 143.636156596409
680.146581716913 145.973240664712
680.292373843373 146.843816523295
680.626750483764 149.019866891257
680.663152491075 149.271682928656
680.765242828512 150.000796730829
681.637194194604 152.916132225805
681.955209812416 155.971383033011
682.242977549488 158.943203760386
682.520142629268 161.630547602834
682.54269111231 161.839324658161
682.845259010224 164.60447208037
682.855056124581 164.695030163708
683.106885719129 167.075431863485
683.13000834741 167.298990070703
682.970066076197 193.779730216374
682.22480381895 196.434696555461
682.198092085862 196.523433134149
681.363812110238 199.211654422888
680.595820631692 201.57677213051
680.52607398313 201.791615988231
680.497659476385 201.879210446838
679.67435670076 204.411080299039
679.609961585912 204.608494791315
678.80373317155 207.05060693742
678.700176740433 207.359614547329
677.973984254556 209.486826268922
677.896843074448 209.709160755731
677.749535286899 210.132019064875
678.138844447334 211.39477397415
678.279915850746 211.87556189091
677.257986574961 214.786304590787
676.183022596268 217.704898567911
674.994073194391 220.637344620298
673.713983359157 223.535865309656
672.483552755436 226.175418358015
672.385798090205 226.378945899611
671.158148609208 228.837873554288
671.044650405305 229.056847231999
670.998080634825 229.146176111404
669.661510050048 231.63745928417
669.556416966554 231.828319765986
668.244402825891 234.15541046731
668.075692698613 234.447458849694
666.904950002937 236.429711694738
666.780995532821 236.63526002111
666.544010744798 237.025840644362
665.710784393893 239.226992028646
665.505407083761 239.744034286811
664.356130277817 241.469669882575
664.220911606327 241.669354758206
663.825847923402 242.24708959028
662.563133867749 244.042002475052
662.42210550843 244.237563968202
662.081221926084 244.705765122538
660.84066454906 246.364390174658
660.693928001518 246.555340712904
660.26670348639 247.108784088107
658.906507324153 248.817655571277
658.388199424723 249.447469028395
656.447344790589 251.723115126958
654.440852794157 253.926030042604
652.35801211295 256.030858994683
650.429382302549 257.814597255146
650.252377487917 257.971970336322
650.180326627334 258.035653549039
648.262180036709 259.668270854971
647.908170938149 259.955497909568
647.061247955572 261.01915886671
646.978663384849 261.108282879588
646.944389597802 261.144090464809
644.76216041753 262.559851049241
644.35698188155 262.80356665079
642.386545007499 263.940281989067
642.167754359747 264.062765599358
641.639953989394 264.35610382575
639.513831396342 265.509631600458
638.864947861169 265.859146574246
636.016923468486 267.380864915663
633.104405328215 268.911398419295
630.22908674099 270.388043335351
630.131914027337 270.437282527347
627.076847170381 271.969172659918
624.036771234642 273.474304770666
623.933915563118 273.524859674015
620.740860874362 275.069394545672
617.872771865701 276.429803273863
617.507965129359 276.600735769987
614.726593452357 277.891508072364
614.46297516552 278.012625794954
614.224834153956 278.122038147648
611.534599060708 279.343092870608
611.266617463819 279.463448839875
610.889608258298 279.632235530397
608.284123214933 280.783241347286
608.011058085765 280.902688631669
607.488247069125 281.130719539389
604.699605359355 282.332289427729
604.030661757631 282.617390943657
601.61714131142 283.635496722602
601.334584130702 283.753316021639
600.513156630596 284.094333113722
597.915357012047 285.156220959472
596.938974094384 285.552598699998
593.35583416976 287.036075974133
589.934628744849 288.525749520785
589.821780535108 288.575801394803
586.332936767137 290.146686070343
582.880742822936 291.72955546045
579.706861225187 293.212195006409
579.460444654985 293.329025976624
576.46781276756 294.793979076491
576.199649715462 294.92910404734
576.091682116197 294.983793264582
573.263336466058 296.452939153544
572.998059476944 296.594879915275
572.757602384563 296.724380177599
569.85052487084 298.387077909755
569.489579265744 298.607817603163
567.075079900754 300.168867725184
566.828728512344 300.337411758924
566.362627218714 300.661445306422
563.971532365118 302.452345680692
563.421085042293 302.897083379227
561.299412274726 304.730754186276
560.683771894724 305.305487492366
558.846065723711 307.155783471035
558.194058116661 307.870712439896
551.966557678202 333.741966491828
552.482406223185 336.203251038489
552.578310899186 336.662046743522
553.170406396815 339.557181694842
553.246575291133 339.940215219394
553.823259691696 342.96332294212
553.921632219905 343.519913422252
554.374037526702 346.292293630051
554.529085608806 347.340209147642
554.89529219706 350.024476961703
555.049609355155 351.252586576279
555.358472548228 353.836455757158
555.518735994257 355.253275306723
555.936982975334 359.281983806582
556.329671145879 363.183724964423
556.342590761035 363.312868134343
556.691458866221 367.019273968501
556.714636094462 367.306678659141
556.935515033497 370.469392519101
556.95568931625 370.779860424388
556.984034644787 371.21379185342
557.203930985236 374.444692570732
557.243876172938 375.020089236284
557.45781779033 378.043475636195
557.505986676785 378.758784608076
557.688003792875 381.578400914998
557.741994265666 382.426291095143
557.912416606327 385.04344222354
557.975599717937 386.015160865707
558.132789820748 388.436855952149
558.2038608748 389.525538007431
558.437379725362 392.961277585509
558.666600165645 396.339128693687
558.881842013099 399.68005286311
559.098633245972 403.03813629018
559.314917897687 406.321346621596
559.322278142657 406.431758200564
559.528379353055 409.611769327795
559.54426753904 409.860677540042
559.724083897713 412.648922633295
559.742083341741 412.925470456877
559.76740152782 413.313635073243
559.960550056321 416.255457265804
559.995266043874 416.784501134835
560.170510373592 419.586529163931
560.209638969488 420.252486711657
560.368511885627 422.905649118507
560.41891816367 423.705348072929
560.639519987808 427.140134964044
560.766213350673 429.213411380471
560.782594584442 429.485469682148
560.84711070265 430.547397180986
561.060805059085 433.923962203205
561.284846508397 437.272752054568
561.506027040891 440.487529281324
561.513225894762 440.593672280121
561.717709228546 443.647878040044
561.733095749552 443.885016032075
561.934219123335 447.043064883285
561.940883302913 447.148280332743
562.137921911215 450.153399941979
562.153749814912 450.387412890045
562.346919189606 453.249612901052
562.371040611915 453.609919022252
562.519445377192 455.824299372017
562.536940107336 456.081612219385
562.587571798359 456.828477081162
562.727637654298 458.910743445339
562.804860496347 460.042351635303
563.031417507921 463.257850344078
563.263899018195 466.473460216324
563.496998264519 469.691378081704
563.709985553264 472.815380825018
563.717039971344 472.91947014898
563.900360868669 475.666435167189
563.917574999034 475.925886126282
563.93315553525 476.160168064226
564.110257154077 478.78506981316
564.153474532319 479.409941496608
564.328229623028 481.9085243008
564.380796936298 482.66666007254
564.599061783538 485.91981350661
564.821492980253 489.167173383134
564.9688409732 491.265655150035
565.048091362387 492.405836049406
565.296842525561 495.635109528316
565.626676319564 498.833308315267
566.030566339775 501.546312072933
566.075363300135 501.802277309695
566.116558264988 502.032324397201
566.639999590108 504.643017699799
566.768091639513 505.224531999754
567.34776459826 507.693432577006
567.410860567488 507.946751606465
567.526257910286 508.39657962464
568.344998822249 511.19401952818
568.451938546399 511.505274826462
569.490173938592 514.019816873404
569.689069800996 514.424788848562
570.834515266841 516.423946684461
570.970863403027 516.632502378972
571.293676432663 517.097928716446
572.787197957835 518.953252827009
573.249547845912 519.443352797436
575.488743330466 521.388852687256
577.965048218338 522.94350645624
580.676547165575 524.15456954719
583.490861481308 525.016644286295
586.399264820845 525.635787530483
586.468306794225 525.648208467787
589.417705144089 526.12861144655
589.619590903049 526.159738229455
592.830610643136 526.658792084945
592.907728661519 526.671221812165
596.35677566748 527.239647544734
599.929127155656 527.819404358951
600.012934919621 527.832623950488
603.580976208111 528.380160924307
603.820006821475 528.415954291378
607.345803596856 528.942161224931
607.752795020196 529.002122274163
609.11317335283 533.093340216421
609.393371377354 533.734135861424
612.754502460237 534.326101091501
613.508446682446 534.458096051803
616.753593774213 535.028066730372
617.684110410717 535.191656646179
620.448041574379 535.677090829056
620.784924612386 535.735200392275
621.889954630689 535.921806684962
626.122868249426 536.619818800255
630.357929613333 537.325222884653
634.55842133787 538.028218024917
638.300205780831 538.652120454051
638.633101935375 538.706652403686
638.726171877361 538.721898255341
642.629347050686 539.34797441455
642.889103810416 539.38857952004
646.298140122664 539.906854294746
646.632073317855 539.956210583664
647.060121213298 540.019148598984
650.647326156529 540.539352479691
651.243044899452 540.626462951096
654.632738066248 541.146196688892
655.395529137655 541.259871918852
658.667667065555 541.734337594046
659.603288161145 541.868971049914
662.712334385564 542.32733311104
663.815036634749 542.50985890774
667.964573880359 543.336711413332
670.909328178953 544.146542273515
671.933614422408 544.490402312083
675.66537122245 546.123299721661
678.860794225357 548.150935376671
678.925439670598 548.200223072464
681.598372691381 550.603955148143
683.609523009323 553.175281927309
683.647818937065 553.234585908053
684.966262156375 555.616311202619
685.068975626764 555.844070263018
685.149266909479 556.022109881773
686.081803118088 558.527340234401
686.176362887892 558.813166992284
686.855988790016 561.114741513438
686.923935968783 561.357473527283
687.043844054133 561.789195715123
687.756582255888 564.344687800896
687.919854731013 564.923038407859
688.656194431607 567.464315377955
688.883892220352 568.207880881612
689.845110602508 571.063816524982
690.076955570855 571.711010336351
691.138228541146 574.572420614795
691.448557036123 575.403254277905
692.362490981882 577.844389290169
692.472986192447 578.139911280939
692.834879638961 579.110672608735
694.243403835597 582.899352238545
695.769479309227 586.744070592519
697.423881686749 590.56226304339
699.020787232135 594.002692551725
699.206968557659 594.396287188612
700.630405629563 597.432239352341
701.038009665881 598.308818127713
702.386316806247 601.235980090985
702.864108960215 602.282923145114
704.135231005131 605.082426010627
704.685365775355 606.295817368487
706.50277214013 610.298960343706
708.308475481854 614.30143905742
710.071578204208 618.212941696702
710.111654415364 618.301668589072
711.800303714227 622.054268031249
711.911824181188 622.303285769942
713.376202880007 625.580201814362
713.519218481834 625.900948887787
713.701716097355 626.310860148113
715.229994156616 629.756805202484
715.484697292511 630.33052218728
716.947747009914 633.620418135622
717.274142544551 634.354511563669
718.521244982421 637.170247121957
718.663945437145 637.493364499722
719.061186829796 638.390413378977
720.870302883899 642.388200694277
722.737495670631 646.328761787341
724.030949496949 648.883807639535
724.725558322722 650.197784237965
726.854206065142 653.960008682137
729.097019727499 657.632877562543
731.397312042948 661.302752783027
733.63866045014 664.866778263926
733.712951878184 664.985042674187
735.825520397261 668.347136206159
735.989234264695 668.607032062031
737.980276268033 671.730037269299
738.229397085396 672.117779658043
739.880987891913 674.695653730431
740.050586307826 674.960122449941
740.373434892867 675.463358643661
741.978060137061 677.965450766574
742.34650836544 678.543452496775
743.718187781843 680.697513681823
744.113302323977 681.315867849276
745.632043929016 683.672862049453
746.888571288166 685.604243149586
747.86992811875 687.111690409274
747.897360951213 687.153824146374
748.579323029233 688.201859346051
748.638444721086 688.292619921364
748.691885319915 688.374677237231
749.181223019394 689.125332428151
749.287033739582 689.287390925199
749.617758383456 689.793571779907
749.653468688375 689.848136778943
749.757058784334 690.006532916263
750.133172965229 690.583215383628
750.422102917414 691.026788729352
750.640121596527 691.361594531734
750.790349855422 691.594025216388
750.879031247356 691.731315290693
750.880247538061 691.733195738182
750.920219648605 691.795043368221
750.921423321649 691.796908621317
750.933133198596 691.815055511965
750.933829825803 691.81613250011
750.935874414832 691.819289904081
750.935919395247 691.819359297773
750.935780880753 691.819145486647
750.933674134001 691.815886796688
750.932982905514 691.814814012163
750.931033148107 691.811787651625
750.930623243974 691.811153327938
750.930623243974 691.811153327938
750.930623243974 691.811153327938
750.930623243974 691.811153327938
750.930623243974 691.811153327938
750.930623243974 691.811153327939
750.930675912367 691.811137491594
750.930681531879 691.811135801187
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
750.930688829964 691.811133605676
};

==> images/dummy_opt_problem2.tex <==
\begin{equation}
\begin{aligned}
\min_{x,p_{c}} \quad & \sum_{c\in \mathcal{C}} p_{c}\\
\textrm{s.t.} \quad & \textrm{ModelConstraints}(x, p_{c})\\
  & \textrm{TaskSpecification}(x, p_{c}) \\
\end{aligned}
\end{equation}
